Accelerated Policy Gradient: On the Convergence Rates of the Nesterov Momentum for Reinforcement Learning

Various acceleration approaches for Policy Gradient (PG) have been analyzed within the realm of Reinforcement Learning (RL). However, the theoretical understanding of the widely used momentum-based acceleration method on PG remains largely open. In response to this gap, we adapt the celebrated Nesterov's accelerated gradient (NAG) method to policy optimization in RL, termed \textit{Accelerated Policy Gradient} (APG). To demonstrate the potential of APG in achieving fast convergence, we formally prove that with the true gradient and under the softmax policy parametrization, APG converges to an optimal policy at rates: (i) $\tilde{O}(1/t^2)$ with constant step sizes; (ii) $O(e^{-ct})$ with exponentially-growing step sizes. To the best of our knowledge, this is the first characterization of the convergence rates of NAG in the context of RL. Notably, our analysis relies on one interesting finding: Regardless of the parameter initialization, APG ends up entering a locally nearly-concave regime, where APG can significantly benefit from the momentum, within finite iterations. Through numerical validation and experiments on the Atari 2600 benchmarks, we confirm that APG exhibits a $\tilde{O}(1/t^2)$ rate with constant step sizes and a linear convergence rate with exponentially-growing step sizes, significantly improving convergence over the standard PG.

==> app/11-add-adaptive-apg__.tex <==
\newpage
\section{APG With Exponentially-Growing Step Sizes}
\label{app:add-adaptive-apg}

\begingroup
\allowdisplaybreaks

%\subsection{Asymptotic Convergence of APG With Exponentially-Growing Step Sizes}
%\begin{theorem}
%    [\textbf{Asymptotic convergence under softmax parameterization}]
%    \label{theorem:global_convergence_adaptive_apg}
%    \mru{Consider a tabular softmax parameterized policy $\pi_{\theta}$. Under \hyperref[algorithm:APG]{APG} with modifying \cref{algorithm:eq1} by 
%    \begin{align*}
%        \theta^{(t)} &\leftarrow \omega^{(t-1)} + \Big[ \eta^{(t)} \nabla_{\theta}{V^{\pi_{\theta}}(\mu)} \Big\rvert_{\theta = \omega^{(t-1)}} \Big]^{+K},
%    \end{align*}
%    where $\eta^{(t)} = \beta^t \cdot \frac{(1-\gamma)^3}{8}$ for any $\beta > 1$, $\mu$ initialized uniformly at random, and $K > \ln2 + 2\ln\beta$, 
%    we have $V^{\pi_{\theta}^{(t)}}(s) \rightarrow V^{*}(s)$ as $t\rightarrow \infty$, for all $s\in\cS$.}
%\end{theorem}
%\cpcomment{It looks like in \Cref{lemma:max Is0} we actually need the
%stepsizes to be upper bounded.
%Please double check this issue.
%If indeed that condition is needed, then asymptotic convergence
%doesn't hold as claimed here for exponentially-growing stepsizes.}
%\begin{proof}[Proof of \Cref{theorem:global_convergence_adaptive_apg}]
%Using the similar arguments of \Cref{theorem:convergeoptimal} and \Cref{lemma: convergence to stationarity}-\ref{lemma:compare pi(a+) and pi(a-)}, we have
%the results. 
%Please note that after clipping, it is invalid to apply \Cref{lemma:sum conservation} in \Cref{lemma:Is- negative infinity} anymore, but it could be relaxed by showing that $\sum_{a \in \cA} \theta_{s,a}^{(t)} \le \sum_{a \in \cA} \theta_{s,a}^{(0)}$ for all $t \ge 0$, $s \in \cS$, and $a \in \cA$.
% 
%% Upon meticulous examination, it becomes apparent that the
%% step sizes $\eta^{(t)}$ can be modified to $\beta^{t} \cdot
%% \frac{(1-\gamma^3)}{8}$ while retaining the validity of all the proofs
%% in \Cref{lemma: convergence to stationarity}-\ref{lemma:compare pi(a+)
%% and pi(a-)}.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence Rate of APG With Exponentially-Growing Step Sizes}

%\begin{restatable}{lemma}{stationarylemma2}
%\label{lemma: adaptive apg enter local concavity}
%    Consider a tabular softmax parameterized policy $\pi_{\theta}$. Under \hyperref[algorithm:APG]{APG} {$\eta^{(t)} = \beta^t \cdot \frac{(1-\gamma^3)}{8}$ for any $\beta > 1$}, given any $M > 0$, there exists a finite time T such that for all $t \ge T$, $s\in\cS$, and $a \neq a^*(s)$, we have, (i) $\theta_{s, a^*(s)} - \theta_{s, a} > M$, (ii) $V^{\pi_{\theta}^{(t)}}(s) > Q^*(s, a_2(s))$, (iii) $\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s, a^*(s)}}\right\rvert_{\theta = \omega^{(t)}} > 0 > \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s, a}}\right\rvert_{\theta = \omega^{(t)}}$, (iv) $\omega_{s, a^*(s)}^{(t)} - \theta_{s, a^*(s)}^{(t)} \ge \omega_{s, a}^{(t)} - \theta_{s, a}^{(t)}$.
%\end{restatable}
%\begin{proof}[Proof of \Cref{lemma: adaptive apg enter local concavity}]
%Using the similar arguments of \Cref{lemma: enter local concavity}, we have the results.
%\end{proof}

% \begin{theorem}[\textbf{Convergence Rate of APG with adaptive learning rate}]
% \label{theorem: adaptive apg convergence rate}
%     Consider a tabular softmax parameterized policy $\pi_{\theta}$. Under \hyperref[algorithm:APG]{APG} with {$\eta^{(t)} = \beta^t \cdot \frac{(1-\gamma)^3}{8}$ for any $\beta > 1$}, there exists a finite time $T$ such that for all $t \ge T$, we have
%     \begin{align}
%         V^{*}(\rho) - V^{{\pi_\theta^{(t)}}}(\rho) = O(e^{-ct}),
%     \end{align}
%     for some constant $c > 0$.
% \end{theorem}
\adaptiveapg*

%\cpcomment{If you decided to use the clipped version, related
%	statements in the main paper is also needed, and then
%	applicability of \Cref{lemma: enter local concavity} is surely
%needed, or you can revert to the old setting of a separate lemma.
%Also, since in the proof you actually have some requirement for $K$,
%you should also state it.}
\begin{proof}[Proof of \Cref{theorem: adaptive apg convergence rate}]

By \Cref{lemma:perf_diff}, we have
\begin{align*}
    V^{*}(\mu) - V^{\pi_{\theta}^{(t)}}(\mu) &= \frac{1}{1 - \gamma} \sum_{s, a} d_{\mu}^{\pi^*}(s) \pi^*(a|s) A^{\pi_{\theta}^{(t)}}(s, a) \\
    &= \frac{1}{1 - \gamma} \sum_{s, a} d_{\mu}^{\pi^*}(s) (\pi^*(a|s) - \pi_{\theta}^{(t)}(a|s)) A^{\pi_{\theta}^{(t)}}(s, a) \\
    &\le \frac{1}{1 - \gamma} \sum_{s, a} \Bigg | d_{\mu}^{\pi^*}(s) (\pi^*(a|s) - \pi_{\theta}^{(t)}(a|s)) A^{\pi_{\theta}^{(t)}}(s, a) \Bigg | \\
    &\le \frac{2}{(1 - \gamma)^2} \left\lVert {d_{\mu}^{\pi^*}} \right\rVert_{\infty} \sum_{s, a} \Bigg | \pi^*(a|s) - \pi_{\theta}^{(t)}(a|s) \Bigg | \\
    &= \frac{2}{(1 - \gamma)^2} \left\lVert {d_{\mu}^{\pi^*}} \right\rVert_{\infty} \sum_{s} \Bigg( \Bigg | \pi^*(a^*|s) - \pi_{\theta}^{(t)}(a^*|s) \Bigg | + \sum_{a \neq a^*} \Bigg | \pi^*(a|s) - \pi_{\theta}^{(t)}(a|s) \Bigg | \Bigg) \\ 
    &= \frac{2}{(1 - \gamma)^2} \left\lVert {d_{\mu}^{\pi^*}} \right\rVert_{\infty} \sum_{s} 2(1-\pi_\theta^{(t)}(a^*|s)).
\end{align*}

To obtain the desired outcome, it is sufficient to show that there
exist $\bar{c}, \tilde{c} > 0$ such that
$1 - \pi_{\theta}^{(t)}(a^*(s) | s) \le \tilde{c} e^{-\bar{c}t}$ for
all $s \in \cS$ and all $t \ge T$.
We prove this result by contradiction.
Selecting $T$ from \Cref{lemma: enter local concavity}, we assume that after time-step $T$, for any $\bar{c}, \tilde{c} > 0$, there exists one state $s'$ and an infinite time sequence $\{ t_i\}_{i=1}^{\infty}$ such that we have $1 - \pi_{\theta}^{(t)}(a^*(s') | s') > \tilde{c} e^{-\bar{c}t}$ for all $t \in \{ t_i\}_{i=1}^{\infty}$.

We then define
\begin{align*}
    C \coloneqq \inf_{s' \in \cS, t \ge T} \Big\{ \frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*(s')|s') \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))) \Big\},
\end{align*}
then we have $C > 0$ since $d^{\pi_\omega^{(t)}}_{\mu}(s') \ge
(1-\gamma)\mu(s')$ by
\Cref{lemma:lower_bound_of_state_visitation_distribution},
$\pi_\omega^{(t)}(a^*(s')|s') > \frac{1}{|\cA|}$ since $\theta_{s',
a^*(s')} > \theta_{s', a}$ for all $a \neq a^*(s')$ by property (i) of
\Cref{lemma: enter local concavity}, and $Q^{\pi_{\theta}^{(t)}}(s',
a^*(s')) \ge V^{\pi_\theta^{(t)}}(s') > Q^{*}(s', a^*(s'))) > \max_{a
	\neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))$ by property
	(ii) of \Cref{lemma: enter local concavity}, \Cref{lemma: Q^*
	a_2}, and \cref{eq:pos}.

By choosing $\tilde{c} = \frac{K}{C}$ and
$\bar{c} = \beta$ and the corresponding $s'$ and $\{t_i\}$, we have
\begin{align}
    A^{\pi_{\theta}^{(t)}}(s', a^*(s'))
    &= Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - V^{\pi_{\theta}^{(t)}}(s') \nonumber \\
    &= Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \sum_{a \in \cA} \pi_{\theta}^{(t)}(a(s')|s') Q^{\pi_{\theta}^{(t)}}(s', a) \nonumber \\
    &= (1-\pi_{\theta}^{(t)}(a^*(s')|s')) Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \sum_{a \neq a^*(s')} \pi_{\theta}^{(t)}(a|s') {Q^{\pi_{\theta}^{(t)}}(s', a)} \nonumber \\
    &\ge (1-\pi_{\theta}^{(t)}(a^*(s')|s')) Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \sum_{a \neq a^*(s')} \pi_{\theta}^{(t)}(a|s') \cdot \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a) \nonumber \\
    &= (1-\pi_{\theta}^{(t)}(a^*(s')|s')) Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - (1-\pi_{\theta}^{(t)}(a^*|s')) \cdot \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a) \nonumber \\
    &= (1-\pi_{\theta}^{(t)}(a^*(s')|s')) \underbrace{(Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a))}_{\text{bounded away from 0}} \nonumber \\
    &> \frac{K}{C\beta^t} \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a)). \label{eq:adaptive_apg_2}
\end{align}

% But the policy parameter $\theta_{s', a^*(s')}$ follows that
Following (\ref{eq:adaptive_apg_2}), for all $t \in \{ t_i\}_{i=1}^{\infty}$, we have
\begin{align}
    &~\theta_{s', a^*(s')}^{(t+1)} - \theta_{s', a^*(s')}^{(t)} \nonumber \\
    =&~ \underbrace{(\theta_{s', a^*(s')}^{(t+1)} - \omega_{s', a^*(s')}^{(t)})}_{\text{gradient}} + \underbrace{(\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)})}_{\text{momentum}} \nonumber \\
    =&~ \min \Big\{K, \eta^{(t)} \nabla_{\theta}{V^{\pi_{\theta}}(\mu)} \Big\rvert_{\theta = \omega^{(t)}} \Big\} + (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)}) \nonumber \\
    =&~ \min \Big\{K, \eta^{(t)} \cdot \frac{1}{1-\gamma} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}({a^*}|s') \cdot A^{\pi_\omega^{(t)}}(s',{a^*}) \Big\} + (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)}) \nonumber \\
    =&~ K + \max_{a \neq a^*(s')} \Big\{ \omega_{s', a}^{(t)} - \theta_{s', a}^{(t)} \Big\} \label{eq:adaptive_apg_3},
    % &> \min \Big\{ K, \beta^t \cdot \frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*|s') \cdot e^{-\bar{c}t} \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))) \Big\} \nonumber \\
    % &= \min \Big\{ K, \big(\underbrace{\frac{\beta}{\beta_0}}_{>1}\big)^t \cdot \underbrace{\frac{(1-\gamma)^3}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*|s') \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s')))}_{\text{bounded away from 0}} \Big\}, \label{eq:adaptive_apg_3} 
\end{align}
where \cref{eq:adaptive_apg_3} holds by \Cref{lemma: enter local concavity} and the fact that
\begin{align*}
    &~\eta^{(t)} \cdot \frac{1}{1-\gamma} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}({a^*}|s') \cdot A^{\pi_\omega^{(t)}}(s',{a^*}) \\
    >&~ \beta^t \cdot \frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*|s') \cdot \frac{K}{C\beta^t} \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))) \\
    =&~ \frac{\frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*(s')|s') \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s')))}{C} \cdot K \\
    \ge&~ K.
\end{align*}

Now we discuss two possible cases:
\begin{itemize}
    \item The infinite time sequences $\{ t_i\}_{i=1}^{\infty}$ contains all $t > T$. (i.e., $\{ t_i\}_{i=1}^{\infty} = \{ T+1, T+2, T+3, \cdots \}$): \\
    In this case, by \cref{eq:adaptive_apg_3} and \Cref{lemma: enter local concavity}, we have that
    \begin{align*}
        \theta_{s', a^*(s')}^{(t+1)} - \theta_{s', a^*(s')}^{(t)} 
        &\ge K + \max_{a \neq a^*(s')} \Big\{ \omega_{s', a}^{(t)} - \theta_{s', a}^{(t)} \Big\} \\
        &> K + \max_{a \neq a^*(s')} \Big\{ \underbrace{(\theta_{s', a}^{(t+1)} - \omega_{s', a}^{(t)})}_{\text{gradient} < 0} \Big\} + \max_{a \neq a^*(s')} \Big\{ \underbrace{(\omega_{s', a}^{(t)} - \theta_{s', a}^{(t)})}_{\text{momentum}} \Big\} \\
        &\ge K + \max_{a \neq a^*(s')} \Big\{ \theta_{s', a}^{(t+1)} -
		\theta_{s', a}^{(t)} \Big\}.
    \end{align*}
    This indicates a constant growth of the policy parameter
	$\theta_{s' ,a^*(s')}$. Consequently, by softmax parameterization,
	it follows that $1 - \pi_\theta^{(t)}(a^* | s') =
	O(e^{-\bar{c}t})$,  thereby completing our contradiction.

    \item There exists at least one $(t_i-1) > T$ such that $(t_i-1) \notin \{ t_i\}_{i=1}^{\infty}$ (i.e., $1 - \pi_{\theta}^{(t_i-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t_i-1}}$):\\
    In this case, we set $K = \frac{1}{6\sqrt{|\cA|}} + 2\ln \beta$ to ensure that the one step improvement $\pi_{\theta}^{(t_i+1)}(a^*(s) | s') - \pi_{\theta}^{(t_i)}(a^*(s) | s')$ is sufficiently large once we follow the update $\theta_{s', a^*(s')}^{(t_i+1)} = \omega_{s', a^*(s')}^{(t_i)} + K$.\cpfn{This is not theupdate rule for the
	parameters unless you have a proof that it is always clipped (so
	that you will need that the gradient is not decreasing too fast,
	which I doubt if you would really get).
	Note that this update rule is indeed used in below (labeled in red).}
    By \Cref{lemma: enter local concavity}, we have:
    \begin{align}
        &~\pi_{\theta}^{(t+1)}(a^*(s) | s') \nonumber \\
        =&~ \frac{\exp(\theta_{s', a^*(s')}^{(t+1)})}{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t+1)})} \nonumber \\
        =&~ \frac{\exp(\theta_{s', a^*(s')}^{(t)} + (\theta_{s', a^*(s')}^{(t+1)} - \omega_{s', a^*(s')}^{(t)}) + (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)}))}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t)} + (\theta_{s', a}^{(t+1)} - \omega_{s', a}^{(t)}) + (\omega_{s', a}^{(t)} - \theta_{s', a}^{(t)}))} \nonumber \\
        =&~ \frac{\exp(\theta_{s', a^*(s')}^{(t)})}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t)} + \underbrace{(\theta_{s', a}^{(t+1)} - \omega_{s', a}^{(t)}) + (\omega_{s', a}^{(t)} - \theta_{s', a}^{(t)}) - (\theta_{s', a^*(s')}^{(t+1)} - \omega_{s', a^*(s')}^{(t)}) - (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)})}_{\le 0})} \nonumber \\
        \geq&~ \frac{\exp(\theta_{s', a^*(s')}^{(t)})}{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t)})} \nonumber \\
        =&~ \pi_{\theta}^{(t)}(a^*(s) | s'). \label{eq:adaptive_apg_3-1}
    \end{align}
    Following \cref{eq:adaptive_apg_3-1}, since $\pi_{\theta}^{(t)}(a^*(s) | s')$ is increasing for all $t > T$, we have
    \begin{align}
        \sum_{a \neq a^*(s')} \pi_{\theta}^{(t_i)}(a| s') = 1 - \pi_{\theta}^{(t_i)}(a^*(s) | s') < 1 - \pi_{\theta}^{(t_i-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t_i-1}}.
        \label{eq:adaptive_apg_4}
    \end{align}
    Moreover, by \Cref{lemma: enter local concavity}, we have
	\cpfn{Not seeing how the 1st ineq is obtained.}
    \begin{align}
        \frac{\sum_{a \neq a^*(s')} \exp (\theta_{s',
		a}^{(t_i)})}{\color{red}{2 \exp (\theta_{s',
		a^*(s')}^{(t_i)})}} \le \sum_{a \neq a^*(s')} \pi_{\theta}^{(t_i)}(a| s') \le \frac{K}{C \beta^{t_i-1}}. 
        \frac{\sum_{a \neq a^*(s')} \exp (\theta_{s', a}^{(t_i)})}{\exp(\frac{1}{6\sqrt{|\cA|}}) \exp (\theta_{s', a^*(s')}^{(t_i)})} \le \sum_{a \neq a^*(s')} \pi_{\theta}^{(t_i)}(a| s') \le \frac{K}{C \beta^{t_i-1}}. \label{eq:adaptive_apg_5}
    \end{align}
    Combining \cref{eq:adaptive_apg_3,eq:adaptive_apg_4,eq:adaptive_apg_5}, we get
    \begin{align}
        1 - \pi_{\theta}^{(t_i+1)}(a^*(s) | s')
        &= \sum_{a \neq a^*(s')} \pi_{\theta}^{(t_i+1)}(a| s') \nonumber\\
        &= \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \theta_{s', a}^{(t_i)}))}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \theta_{s', a}^{(t_i)}))} \nonumber\\
        &= \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)} + \overbrace{(\theta_{s', a}^{(t_i+1)} - \omega_{s', a}^{(t_i)})}^{<0} + \overbrace{(\omega_{s', a}^{(t_i)} - \theta_{s', a}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)})}^{\le0})}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \omega_{s', a}^{(t_i)}) + (\omega_{s', a}^{(t_i)} - \theta_{s', a}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        % &\le \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)})}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \omega_{s', a}^{(t_i)}) + (\omega_{s', a}^{(t_i)} - \theta_{s', a}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        &\le \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)})}{\exp(\theta_{s', a^*(s')}^{(t_i)} + (\theta_{s', a^*(s')}^{(t_i+1)} - \omega_{s', a}^{(t_i)}) + (\omega_{s', a^*(s')}^{(t_i)} - \theta_{a^*(s')}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        &\le \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)}))}{ \exp(\theta_{s', a^*(s')}^{(t_i)} + (\theta_{s', a^*(s')}^{(t_i+1)} - \omega_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        &= \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)})}{
			\exp(\theta_{s', a^*(s')}^{(t_i)})} \cdot
			{\color{red}{\exp(-K)}} \nonumber\\
        &\le \frac{2K}{C \beta^{t_i-1}} \cdot \exp(-K) \nonumber\\
        &= \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)})}{ \exp(\theta_{s', a^*(s')}^{(t_i)})} \cdot \exp(-K) \nonumber\\
        &\le \frac{\exp(\frac{1}{6\sqrt{|\cA|}})K}{C \beta^{t_i-1}} \cdot \exp(-K) \nonumber\\
        &\le \frac{K}{C \beta^{t_i+1}}, \label{eq:adaptive_apg_6}
    \end{align}
    where \cref{eq:adaptive_apg_6} holds by setting $K = \frac{1}{6\sqrt{|\cA|}} + 2\ln \beta$.
    
	{\color{red}{
    Hence we get that once $1 - \pi_{\theta}^{(t)}(a^*(s) | s') > \frac{K}{C \beta^{t}}$ occurs for any $t \in \{ t_i\}_{i=1}^{\infty}$, we could ensure that $1 - \pi_{\theta}^{(t+1)}(a^*(s) | s') \le \frac{K}{C \beta^{t+1}}$ (i.e., $(t_i+1) \notin \{ t_i\}_{i=1}^{\infty}$ for all $t_i \in  \{ t_i\}_{i=1}^{\infty}$),
    In other words, for all $t \in  \{ t_i\}_{i=1}^{\infty}$, we have $t-1 \notin  \{ t_i\}_{i=1}^{\infty}$ and hence $1 - \pi_{\theta}^{(t-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t-1}}$.
    Combining with the monotonicity of $1 -\pi_{\theta}^{(t-1)}(a^*(s) | s')$ in \cref{eq:adaptive_apg_3-1}, we get $1 -\pi_{\theta}^{(t)}(a^*(s) | s') \le 1 -\pi_{\theta}^{(t-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t-1}}$.
    Finally, we could conclude that $1 - \pi_{\theta}^{(t)}(a^*(s) |
	s') \le \frac{K}{C \beta^{t-1}}$ for all $t > T$, which also
complete our contradiction.}}\cpfn{Not understanding this paragraph.
	What you have tried to show was that $t_j-1 \notin \{t_i\}$ for some
	$j$ implies that $t_j + 1 \notin \{t_i\}$.
	In this case, I am not seeing what has been proven that could give
you a contradiction.}
	\qedhere
\end{itemize}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This indicates a constant growth of the policy parameter $\theta_{s ,a^*}$. Consequently, it follows that $1 - \pi_\theta^{(t)}(a^* | s') = O(e^{-\bar{c}t})$ for some $\bar{c} > 0$, thereby completing our contradiction.

% Following \cref{eq:adaptive_apg_3}, we then show that $1 - \pi_{\theta}^{(t)}(a^* | s') \le \big(\frac{1}{
% \beta_0
% }\big)^{t-1}$ for all large enough $t \in \{ t_i\}_{i=1}^{\infty}$ by contradiction. Assume $1 - \pi_{\theta}^{(t_i-1)}(a^* | s') > \big(\frac{1}{
% \beta_0
% }\big)^{t_i-1}$ for some $i \in \mathbb{N}_+$, then we have
% \begin{align*}
%     &\theta_{s', a^*(s')}^{(t_i)} \\
%     &= \theta_{s', a^*(s')}^{(t_i-1)} + (\theta_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i-1)}) \\
%     &> \underbrace{\theta_{s', a^*(s')}^{(t_i-1)}}_{\text{bounded below}} + \underbrace{\big(\frac{\beta}{\beta_0}\big)^{t_i-1}}_{\rightarrow \infty \text{, exponentially}} \cdot \underbrace{\frac{(1-\gamma)^3}{8} \cdot d^{\pi_\omega^{(t_i-1)}}_{\mu}(s') \cdot \pi_\omega^{(t_i-1)}(a^*|s') \cdot (Q^{\pi_{\theta}^{(t_i-1)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t_i-1)}}(s', a^*(s')))}_{\text{bounded away from 0}} \\
%     &\ge \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} + \ln (2|\cA|) + t \ln \beta_0.
% \end{align*}
% And so we have
% \begin{align}
%     &1- \pi_\theta^{(t_i)} \\ 
%     &= 1 - \frac{\exp (\theta_{s', a^*(s')}^{(t_i)})}{\exp (\theta_{s', a^*(s')}^{(t_i)}) + \sum_{a \neq a^*(s')} \exp (\theta_{s', a}^{(t_i)})} \\
%     & = 1 - \frac{\exp (\theta_{s', a^*(s')}^{(t_i)} - \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} - \ln (2|\cA|))}{\exp (\theta_{s', a^*(s')}^{(t_i)} - \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} - \ln (2|\cA|)) + \sum_{a \neq a^*(s')} \exp (\theta_{s', a}^{(t_i)} - \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} - \ln (2|\cA|))} \\
%     &\le 1 - \frac{\exp (t_i \ln \beta_0)}{\exp (t_i \ln \beta_0) + (|\cA|-1) \exp(-\ln (2|\cA|))} \\
%     &\le 1 - \frac{\exp (t_i\ln \beta_0)}{\exp (t_i\ln \beta_0) + 1/2} \\
%     &\le 1 - \frac{\beta_0^{t_i}}{\beta_0^{t_i} + \frac{\beta_0^{t_i}}{\beta_0^{t_i}-1}} \\
%     &= \big(\frac{1}{\beta_0}\big)^{t_i},
% \end{align}
% which contradict to $1 - \pi_{\theta}^{(t)}(a^* | s') > \big(\frac{1}{\beta_0}\big)^t$ for all $t \in \{ t_i\}_{i=1}^{\infty}$.

% Combining with the fact that $1 - \pi_{\theta}^{(t)}(a^* | s')$ is non-increasing, we have $1 - \pi_{\theta}^{(t)}(a^* | s') \le \big(\frac{1}{\beta_0}\big)^{t-1}$ for all large enough $t \in \mathbb{N}$ and hence we complete the proof.
%
\end{proof}


% \newpage
% \subsection{Table to put at introduction}
% \begin{table}[!ht]
% \color{blue}
% \caption{Convergence Rates with Exact Gradients for the Tabular Case}
% \label{table:rate}
% \vskip 0.11in
% \begin{center}
%     \begin{small}
%     \begin{sc}
%         \begin{tabular}{cccc}
%         \toprule
%                    & \textbf{APG (Ours)}               & NPG          & GNPG         \\
%         \midrule
%         Constant step sizes & \boldsymbol{$\tilde{O}({1} / {t^2})$} (\Cref{theorem: MDP convergence rate}) & $O({1} / {t})$ \citep{agarwal2021theory, xiao2022convergence} & N/A          \\
%         Adaptive step sizes & \boldsymbol{$O(e^{-ct})$} (\Cref{theorem: adaptive apg convergence rate})             & $O(e^{-ct})$ \citeauthor{khodadadian2021linear, xiao2022convergence}& $O(e^{-ct})$ \citep{mei2021leveraging} \\
%         \bottomru

le
% \end{tabular}
%     \end{sc}
%     \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

\subsection{Numerical Validation of the Linear Convergence Rate}
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
  % \vspace{-\intextsep}
  % \vspace{-\intextsep}
  \includegraphics[width=0.35\textwidth]{img_icml/adaptive-apg.png}
  \hspace{-5mm}
  \caption{The sub-optimality gap of APG with exponentially-growing
  step sizes under an MDP of five states and five actions with uniform initialization.}
  % \vspace{-\intextsep}
  \label{exp:adaptiveapg}
\end{wrapfigure}

In this subsection, we empirically validate the convergence rate of
APG with an exponentially-growing step size scheduling by conducting
experiments on an MDP with five states and five actions. This MDP is identical to the one discussed in \Cref{sec:disc:exp}, and detailed configuration information is provided in \Cref{app:experiment}.
The figure illustrating the logarithmic sub-optimality gap of APG with
an exponentially-growing step size shceduling under uniform
initialization is presented in \Cref{exp:adaptiveapg}.
It is evident that after ten iterations, the curve tends to form a
linear pattern.
This behavior aligns with the linear convergence rate demonstrated in \Cref{theorem: adaptive apg convergence rate}.

\endgroup


==> app/12-gnpg-apg.tex <==
\newpage
\section{APG With Geometry-Aware Normalized Step Sizes}
\label{app:gnpg-apg}

\begingroup
\allowdisplaybreaks

\subsection{Asymptotic Convergence of APG With Geometry-Aware Normalized Step Sizes}

\begin{theorem}
   [\textbf{Asymptotic Convergence Under Softmax Parameterization}]
   \label{theorem:global_convergence_gnpg_apg}
   \mru{Consider a tabular softmax parameterized policy $\pi_{\theta}$. For \hyperref[algorithm:APG]{APG} {$\eta^{(t)} = \frac{1-\gamma}{6 \cdot (1-\gamma) + 8 \cdot (C_\infty - (1-\gamma))} \cdot \frac{1}{\sqrt{|\cS|}} \cdot \lVert \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}}\rVert_2^{-1}$}  where $C_\infty \coloneqq \max_{\pi} \lVert \frac{d^{\pi}_\mu}{\mu} \rVert_\infty \le \frac{1}{\min_s \mu(s)} < \infty$ {and $\mu$ initialized uniformly at random}, the following holds almost surely:
   \begin{equation*}
       \lim_{t\rightarrow \infty}V^{\pi_{\theta}^{(t)}}(s) = V^{*}(s), \forall s\in\cS.
   \end{equation*}}
\end{theorem}

\begin{proof}[Proof of \Cref{theorem:global_convergence_gnpg_apg}]
    \mru{Similar to the proof of \Cref{theorem:global_convergence_adaptive_apg}, we have to show that APG has the following properties under the geometry-aware normalized step sizes:
    \begin{equation*}
        \lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega^{(t)}} \big\rVert =0,\quad
        \lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\theta^{(t)}} \big\rVert =0.
    \end{equation*}
    Note that we can leverage the same argument in the proof of \Cref{lemma: convergence to stationarity clipping} to show that $\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega^{(t)}} \big\rVert =0$.
    Regarding $\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\theta^{(t)}} \big\rVert =0$, it suffices to show that $\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\theta^{(t)}} - \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega^{(t)}} \big\rVert =0$. By \Cref{definition: non-uniform smoothness in mei,lemma: smoothness equivalence,lemma:NS1,lemma: NS2-apg}, we have
    \begin{equation*}
        \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\theta^{(t)}} - \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega^{(t-1)}} \big\rVert \le \Big[ 3 + \frac{4 \cdot (C_\infty - (1-\gamma))}{1-\gamma} \sqrt{|\cS|}  \Big]\cdot 2 \cdot \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega^{(t-1)}} \big\rVert \cdot \big\lVert \theta^{(t)} - \omega^{(t-1)}\big\rVert.
    \end{equation*}
    Note that the norm of $\big\lVert \theta^{(t)} - \omega^{(t-1)}\big\rVert$ is always bounded due to the geometry-aware normalized step sizes. Thus, by $\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega^{(t)}} \big\rVert =0$ and triangle inequality, we have $\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\theta^{(t)}} \big\rVert =0$.}

    \mru{After obtaining the results, we directly have the results from \Cref{lemma: monotone limits exist}-\Cref{lemma:compare pi(a+) and pi(a-)} and \Cref{theorem:convergeoptimal} under the geoemtry-aware normalized step sizes since those arguments are step size independent. Hence, we obtain the asymptotic convergence result.}
\end{proof}


\subsection{Convergence Rate of APG With Geometry-Aware Normalized Step Sizes}

\mru{We assume that \Cref{assump:unique_optimal} holds in this subsection. We introduce the following lemma for facilitating the proof of \Cref{theorem: gnpg apg convergence rate}.}

\begin{lemma}
\label{lemma: inf pi a* > 0}
    Consideer a tabular softmax paramterized policy $\pi_{\theta}$. By using APG with geometry-aware normalized step sizes, we have $\inf_{s \in \cS, t \ge 1} \pi_\omega^{(t)} (a^*(s)|s) > 0$.
\end{lemma}
\begin{proof}[Proof of \Cref{lemma: inf pi a* > 0}]
    Since we have \Cref{theorem:global_convergence_gnpg_apg}, by the same argument of \Cref{cor:policy convergence}, we have $\lim_{t\rightarrow \infty} \pi_{\omega}(a^*(s) | s) = 1$ for all $s\in\cS$. By the definition of limit and the positiveness of the softmax parameterization policy, we obtain the result.
\end{proof}

\gnpgapg*

\begin{proof}[Proof of \Cref{theorem: gnpg apg convergence rate}]

Define $\omega_{\zeta^{(t)}} \coloneqq \omega^{(t)} + \zeta^{(t)} \cdot (\theta^{(t+1)} - \omega^{(t)})$ with some $\zeta^{(t)} \in [0, 1]$.
By \Cref{lemma:NS1,lemma:NS2}, we have
\begin{align}
    &\Big| V^{\pi_\theta^{(t+1)}}(\mu) - V^{\pi_\omega^{(t)}}(\mu) - \Big\langle \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}}, \theta^{(t+1)}-\omega^{(t)} \Big\rangle \Big| \nonumber \\
    &\le \frac{4 C_\infty - (1-\gamma)}{2(1-\gamma)} \cdot \sqrt{|\cS|} \cdot \Big\lVert \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega_{\zeta^{(t)}}} \Big\rVert_2 \cdot \lVert \theta^{(t+1)} - \omega^{(t)} \rVert_2^2 \nonumber \\
    &\le \frac{4 C_\infty - (1-\gamma)}{1-\gamma} \cdot \sqrt{|\cS|} \cdot \Big\lVert \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}} \Big\rVert_2 \cdot \lVert \theta^{(t+1)} - \omega^{(t)} \rVert_2^2 \label{eq:gnpg-apg-eq1}
\end{align}
Following \cref{eq:gnpg-apg-eq1} and defining $\delta^{(t)} \coloneqq V^*(\mu) - V^{\pi_\theta^{(t)}}(\mu)$, we have.
\begin{align}
    \delta^{(t+1)} - \delta^{(t)}
    &= V^{\pi_\theta^{(t)}}(\mu) - V^{\pi_\theta^{(t+1)}}(\mu) \nonumber \\
    &= (V^{\pi_\theta^{(t)}}(\mu) - V^{\pi_\omega^{(t)}}(\mu)) + (V^{\pi_\omega^{(t)}}(\mu) - V^{\pi_\theta^{(t+1)}}(\mu)) \nonumber \\
    &\le V^{\pi_\omega^{(t)}}(\mu) - V^{\pi_\theta^{(t+1)}}(\mu) \label{eq:gnpg-apg-eq2} \\
    &\le -\Big\langle \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}}, \theta^{(t+1)}-\omega^{(t)} \Big\rangle + \frac{4 C_\infty - (1-\gamma)}{1-\gamma} \cdot \sqrt{|\cS|} \cdot \Big\lVert \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}} \Big\rVert_2 \cdot \lVert \theta^{(t+1)} - \omega^{(t)} \rVert_2^2 \nonumber \\
    &=-\frac{1-\gamma}{8C_\infty - 2(1-\gamma)} \cdot \frac{1}{\sqrt{|\cS|}} \cdot \Big\lVert \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}} \Big\rVert_2 \nonumber\\
    &\quad + \frac{4 C_\infty - (1-\gamma)}{1-\gamma} \cdot \sqrt{|\cS|} \cdot \Big\lVert \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}} \Big\rVert_2 \cdot \Big( \frac{1-\gamma}{8C_\infty - 2(1-\gamma)} \cdot \frac{1}{\sqrt{|\cS|}} \Big)^2 \nonumber \\
    &= -\frac{1-\gamma}{16C_\infty - 4(1-\gamma)} \cdot \frac{1}{\sqrt{|\cS|}} \cdot \Big\lVert \nabla_\theta V^{\pi_\theta} \rvert_{\theta = \omega^{(t)}} \Big\rVert_2 \nonumber\\
    &\le -\frac{1-\gamma}{16C_\infty - 4(1-\gamma)} \cdot \frac{1}{|\cS|} \cdot \Big\lVert \frac{d^{\pi^*}_\mu}{\mu} \Big\rVert_\infty^{-1} \cdot \underbrace{\inf_{s \in \cS, t \ge 1} \pi_\omega^{(t)} (a^*(s)|s)}_{>0 \text{  by \Cref{lemma: inf pi a* > 0}}} \cdot \delta^{(t)} \label{eq:gnpg-apg-eq3}
\end{align}
where \cref{eq:gnpg-apg-eq2} holds by the update rule \cref{algorithm:eq3} of APG and \cref{eq:gnpg-apg-eq3} holds by \Cref{lemma:non-uniform L}.
By rearranging \cref{eq:gnpg-apg-eq3}, we have
\begin{align}
    V^{\pi^*}(\mu) - V^{\pi_\theta^{(t)}}(\mu)
    &\le \Big( 1 - \frac{1-\gamma}{16C_\infty - 4(1-\gamma)} \cdot \frac{1}{|\cS|} \cdot \Big\lVert \frac{d^{\pi^*}_\mu}{\mu} \Big\rVert_\infty^{-1} \cdot \inf_{s \in \cS, t \ge 1} \pi_\omega^{(t)} (a^*(s)|s) \Big) \cdot (V^{\pi^*}(\mu) - V^{\pi_\theta^{(t-1)}}(\mu)) \nonumber \\
    &\le \exp \Big( \frac{1-\gamma}{16C_\infty - 4(1-\gamma)} \cdot \frac{1}{|\cS|} \cdot \Big\lVert \frac{d^{\pi^*}_\mu}{\mu} \Big\rVert_\infty^{-1} \cdot \inf_{s \in \cS, t \ge 1} \pi_\omega^{(t)} (a^*(s)|s) \Big) \cdot (V^{\pi^*}(\mu) - V^{\pi_\theta^{(t-1)}}(\mu)) \\
    &\le \exp \Big( t \cdot \frac{1-\gamma}{16C_\infty - 4(1-\gamma)} \cdot \frac{1}{|\cS|} \cdot \Big\lVert \frac{d^{\pi^*}_\mu}{\mu} \Big\rVert_\infty^{-1} \cdot \inf_{s \in \cS, t \ge 1} \pi_\omega^{(t)} (a^*(s)|s) \Big) \cdot (V^{\pi^*}(\mu) - V^{\pi_\theta^{(0)}}(\mu))
\end{align}
Finally, by \Cref{lemma:performance_difference_in_rho}, we reach our desired result:
\begin{align*}
    &V^{*}(\rho) - V^{{\pi}}(\rho) \\ 
    &\le \frac{1}{1-\gamma} \cdot \Big \| \frac{{d^{\pi^*}_{\rho}}}{\mu} \Big \|_{\infty} \cdot \left ( V^{*}(\mu) - V^{{\pi}}(\mu) \right ) \\
    &\le \frac{1}{1-\gamma} \cdot \Big \| \frac{{d^{\pi^*}_{\rho}}}{\mu} \Big \|_{\infty} \cdot \exp \Big( t \cdot \frac{1-\gamma}{16C_\infty - 4(1-\gamma)} \cdot \frac{1}{|\cS|} \cdot \Big\lVert \frac{d^{\pi^*}_\mu}{\mu} \Big\rVert_\infty^{-1} \cdot \inf_{s \in \cS, t \ge 1} \pi_\omega^{(t)} (a^*(s)|s) \Big) \cdot (V^{\pi^*}(\mu) - V^{\pi_\theta^{(0)}}(\mu)).
\end{align*}

\end{proof}



\subsection{Numerical Validation of the Linear Convergence Rate}
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
  % \vspace{-\intextsep}
  % \vspace{-\intextsep}
  \includegraphics[width=0.35\textwidth]{img_icml/apg-gnpg.png}
  \hspace{-5mm}
  \caption{The sub-optimality gap of APG with geometry-aware normalized
  step sizes under an MDP of five states and five actions with uniform initialization.}
  % \vspace{-\intextsep}
  \label{exp:apggnpg}
\end{wrapfigure}

In this subsection, we empirically validate the convergence rate of
APG with an geometry-aware normalized step size scheduling by conducting
experiments on an MDP with five states and five actions. This MDP is identical to the one discussed in \Cref{sec:disc:exp}, and detailed configuration information is provided in \Cref{app:experiment}.
The figure illustrating the logarithmic sub-optimality gap of APG with
an exponentially-growing step size scheduling under uniform
initialization is presented in \Cref{exp:apggnpg}.
It is evident that after ten iterations, the curve tends to form a
linear pattern.
This behavior aligns with the linear convergence rate demonstrated in \Cref{theorem: gnpg apg convergence rate}.

\endgroup

==> app/4-bandit.tex <==
\newpage
% \section*{Appendix}
% \appendix
% \label{section:Appendix}
% \vspace{-2mm}
%\section{Convergence Rate: The Instructive Bandit Case}
\section{Convergence Rates of APG: The Multi-Action Bandit Case}
\label{app:bandit}

\begingroup
\allowdisplaybreaks

\subsection{$\tilde{O}(1/t^2)$ Convergence Rate of APG}
\label{app:bandit:upper}
% \subsection{Supporting Algorithm}
% \label{app:bandit:algo}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Supporting Lemmas}
% \label{app:bandit:lemmas}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Convergence Rate}
% \label{app:bandit:rate}
%
% \begin{theorem}
% \label{theorem:bandit_convergence_rate}
% Consider a tabular softmax parameterized policy $\pi_\theta$. Under \hyperref[algorithm:APG]{APG} with $\eta = \frac{1}{5}$, there exists a finite time
% \begin{align}
% T = \textbf{\mru{TBD}},
% \end{align}
% such that for all $t > T$, we have:
% \begin{align}
% \left ( \pi^{*} - \pi_{\theta_{t}} \right )^{\top} r = O(\frac{1}{t^2}). \text{\mru{TODO: add pre-constant}}
% \end{align}
% \end{theorem}
\banditratethm*

\begin{proof}[Proof of \Cref{theorem:bandit_convergence_rate}]  
\phantom{}

% (Original thoughts) The proof can be summarized as follows:
% \begin{enumerate}
% \itemsep0em
%   \item  We first show that there exists a finite time $T_1$ such that $\pi_{\theta_{T}}^{\top} r > r(a_2)$.
%   %
%   \item We then construct a harder case and show that the convergence rate of the original case must be lower bounded by the one of the harder case (\Cref{lemma:bandit_hard_ease_case}).
%   %
%   \item Finally, we show that the harder case enjoy the convergence rate of $O(\frac{1}{t^2})$ after finite time $T_2$ (\Cref{lemma:bandit_sigmoid_concave}) and hence we get the desired result with $T = T_1 + T_2$.
% \end{enumerate}

\begin{claim}
    The proof can be completed by making the following claims:

    \textbf{a)} By \Cref{lemma:local concavity}, the function $\theta \to \pi_{\theta}^{\top} r$ is concave if $\theta_{a^{*}} - \theta_{a} > \delta$ for all $a \neq a^{*}$ where $\delta = \ln \frac{r(a_2)(|\cA|-1)}{r(a^*)-r(a_2)} + \ln (1 + \binom{|\cA|-1}{2}) - \ln(d(a^*) - d(a_i))$. %$\theta_{a^{*}} - \theta_{a} > \ln 4(|\cA|-1)$ for all $a \neq a^{*}$.

    \textbf{b)} By \Cref{lemma:bandit enters local concavity}, given such  $\delta$, there exists a finite time $T$ such that $\theta^{(t)}_{a^{*}} - \theta^{(t)}_{a} > \delta$ holds for all $t > T$, $a \neq a^{*}$.

    \textbf{c)} APG enjoys the convergence rate of $\tilde{O}(\frac{1}{t^2})$ after time $T$.
    %
    % \textbf{d)}
\end{claim}

% The proof can be summarized as follows:
%
% \begin{enumerate}
% \itemsep0em
%   \item  We first show that there exists a delta $\delta$ such that the function $\theta \to \pi_{\theta}(a^{*}) \cdot r(a^{*})$ is concave while $\theta_{a^{*}} - \theta_{a} > \delta$ for all $a \neq a^{*}$.
%   %
%   \item We then state that given any $\delta > 0$, there exists a finite time $T$ such that $\theta^{(t)}_{a^{*}} - \theta^{(t)}_{a} > \delta$ holds for all $t > T$, $a \neq a^{*}$.
%   %
%   \item Finally, we complete the proof by showing that APG enjoys the convergence rate of $O(\frac{1}{t^2})$ under a different initialized learning rate \mru{TBD} after time $T$. \mru{We also have to argue it approach $\theta^*$ where $\theta^*$ is closed to $\infty.$ Also, we have to argue $\pi(a^{*}) \cdot r(a^{*})$ is the lower bdd of the objective.}
% \end{enumerate}
%
% \textbf{Claim a).} By \Cref{lemma:composition_function_concave}, we can seperate our proof into 2 steps:
% To show that there exists a delta $\delta$ such that the function $\theta \to \pi_{\theta}(a^{*}) \cdot r(a^{*})$ is concave while $\theta_{a^{*}} - \theta_{a} > \delta$ for all $a \neq a^{*}$, we leverage \Cref{lemma:composition_function_concave} and hence it remains to show that:

% \begin{itemize}
%     \item The function $\theta \to \pi(a^*)$ is concave while $\theta_{a^{*}} - \theta_a > \delta$ for some $\delta > 0$, for all $a \neq a^{*}$: \\
%     By \Cref{lemma:local concavity}, we've shown the concavity holds for $\delta = \ln 4(n-1)$.
%     %
%     \item The function $\pi(a^*) \to \pi(a^*) \cdot r(a^*)$ is concave and non-decreasing: \\
%     This property directly hold since $\pi(a^*) \cdot r(a^*)$ is a linear function of $\pi(a^*)$ with $\frac{\partial \pi(a^*) \cdot r(a^*)}{\partial \pi(a^*)} = r(a^*) > 0$ and $\frac{\partial^2 \pi(a^*) \cdot r(a^*)}{\partial \pi(a^*)^2} = 0$.
%     %
% \end{itemize}

% \textbf{Claim b).} Part (i): We first show that $\inf_{t \ge 0, \pi_{\omega}^{(t)\top} r \in [0, r(a_2)]} \left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \omega^{(t)}} \right \| \ge \inf_{t\ge 0} \pi^{(t)}_{\omega}(a^*) \cdot (r(a^*) - r(a_2)) > 0$ by leveraging \Cref{lemma:inf-bandit optimal}:

% \begin{align}
%     \left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \omega^{(t)}} \right \|
%     &= \sqrt{\sum_{a \in \cA} \pi^{(t)}_{\omega}(a)^2 \cdot (r(a) - \pi_{\omega}^{(t)\top} r)^2} \label{eq:bandint_conv_rate_1} \\
%     &\ge \sqrt{ \pi^{(t)}_{\omega}(a^*)^2 \cdot (r(a^*) - \pi_{\omega}^{(t)\top} r)^2} \label{eq:bandint_conv_rate_2} \\
%     &= \pi^{(t)}_{\omega}(a^*) \cdot (r(a^*) - \pi_{\omega}^{(t)\top} r) \label{eq:bandint_conv_rate_3} \\
%     &\ge \inf_{t\ge 0} \pi^{(t)}_{\omega}(a^*) \cdot (r(a^*) - r(a_2)) > 0, \quad \text{for all } \pi_{\omega}^{(t)\top} r \in [0, r(a_2)], \label{eq:bandint_conv_rate_4}
% \end{align}
% where (\ref{eq:bandint_conv_rate_1}) is followed by \Cref{lemma:softmax_pg} and (\ref{eq:bandint_conv_rate_4}) is by \Cref{lemma:inf-bandit optimal}. We finish the proof of Part (i).

% Part (ii): Since APG will converge to stationary point (last-iterate) \mru{ref converge to stationary point Lemma}, given a sufficiently small $\epsilon$, we can reach our desired result. 

\textbf{Claim c).}
As the objective $\pi_\theta^{\top}r$ enters a locally concave region after time $T$, it is necessary to account for a shift in the initial learning rate due to the passage of time $T$. In other words, if we divide the update process into two phases based on time $T$, the latter phase will commence with a modified learning rate. Hence, by \Cref{cor:ghadimi_cor1} and \Cref{lemma:bandit_smoothness} with $c = T$ and $\theta^{**} = \theta^{(t)**}$, we have that for all $t > T$:
\begin{align}
    \label{eq:bandit_surrogate_1}{\pi_{\theta^{**}}^{(t)}}^{\top} r - {\pi_{\theta}^{(t)}}^{\top} r 
    & \le \frac{4L (2+T) \left \| \theta^{(0)} - \theta^{(t)**} \right \|^2 }{(t+T+1)(t+T)} \\
    &= \frac{10 (2+T) \left \| \theta^{(T)} - \theta^{(t)**} \right \|^2 }{(t+T+1)(t+T)} \\
    &= \frac{10 (2+T) \left(  \left \| \theta^{(T)} \right \| + 2 \ln(t-T) \right)^2 }{(t+T+1)(t+T)},
\end{align}
where $\theta^{(t)**} \coloneqq [2\ln(t-T), 0, 0, \cdots, 0]$ is a chosen surrogate optimal solution at time $t$.
Additionally, we have the sup-optimality gap between the original optimal solution and the surrogate optimal solution can be bounded as:
\begin{align}
    {\pi^*}^{\top} r - {\pi_{\theta^{**}}^{(t)}}^{\top} r
    &= r(a^*) - {\pi_{\theta^{**}}^{(t)}}^{\top} r \\
    &\le r(a^*) \left( 1 - \pi_{\theta^{**}}^{(t)}(a^*) \right) \label{eq:bandit_surrogate_2}\\
    &= r(a^*) \left( 1 - \frac{\exp(2\ln(t-T))}{\exp(2\ln(t-T)) + \exp(0) \cdot (|\cA| - 1)} \right) \\
    &= r(a^*) \left( \frac{|\cA| - 1}{(t-T)^2 + |\cA| - 1} \right) \\
    &\le \frac{|\cA| - 1}{(t-T)^2 + |\cA| - 1}, \label{eq:bandit_surrogate_3}
\end{align}
where (\ref{eq:bandit_surrogate_2}) holds since we ignore the terms $\pi_{\theta^{**}}^{(t)}(a) \cdot r(a) \ge 0$ for every $a \neq a^*$ .Combining (\ref{eq:bandit_surrogate_1}-\ref{eq:bandit_surrogate_3}), we get our desired result.

\begin{remark}
\normalfont \mru{It is crucial to highlight that we consider the surrogate optimal solution $\theta^{(t)**}$ instead of the original optimal solution $\theta^{*}$ due to the unbounded optimal solution of softmax parameterization.} 
\end{remark}

% Part (ii): increasing optimal solution $\bar{\theta^*}$
% 
% After that, By \Cref{prop:lower_bdd_gradient}, we have $\inf_{t \ge 1, \pi_{\theta_t}^{\top} r \in [0, r(a_2)]} \left \| \frac{\partial \pi_{\theta_t}^{\top} r}{\partial \theta} \right \| > 0$ under APG. And hence by \Cref{lemma:stationary_point}, we show that $\theta_t(a^{*}) - \theta_t(a_i) > \delta$ will holds after time $T = \text{\mru{TBD}}$ \mru{(still have to argue for all time)} for all $i = 2, 3, \cdots, n$.
% 
% So far, we've shown that after a finite time $T$, the objective we aim to optimize will turn into a concave function. Hence, the remaining thing to show is that under \mru{Algorithm 1?} with a shifting learning rate, APG could still reach the convergence rate of $O(\frac{1}{t^2})$, which we've shown in \mru{Lemma ???}.

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}[Local Concavity]
% \label{lemma:local concavity}
% The function $\theta \to \pi(a^*)$ is concave while $\theta_{a^{*}} - \theta_{a_i} > \delta$ for some $\delta > 0$, for all $a \neq a^{*}$.
% \end{lemma}
% \localconcavelemma*

% \begin{proof}[Proof of \Cref{lemma:local concavity}]  
% \phantom{}

% \begin{claim}
%     The proof can be completed by making the following claims:
    
%     \textbf{a)} The function $\theta \to \pi_{\theta}(a^{*})$ is concave and the functions $\theta \to \pi_{\theta}(a)$ are convex if $\theta_{a^{*}} - \theta_{a} > \delta$ for all $a \neq a^{*}$ where $\delta = \ln \frac{r(a_2)(|\cA|-1)}{r(a^*)-r(a_2)} + \ln (1 + \binom{|\cA|-1}{2}) - \ln(d(a^*) - d(a_i))$.
    
%     \textbf{b)} The function $\theta \to \pi_{\theta}^{\top} r'$ is concave if $\theta_{a^{*}} - \theta_{a} > \delta$ for all $a \neq a^{*}$, where $r' = [ r(a^*) - r(a_2), r(a_2) - r(a_2), \cdots, r(a_{|\mathcal{A}|}) - r(a_2) ]$ is the \textit{shifted reward function}.
    
%     \textbf{c)} The update of the objective $\pi_{\theta}^{\top} r$ under the original reward $r$ is equivalent to the update of the objective $\pi_{\theta}^{\top} r'$ under any shifted reward function $r' = \left[ r(a^*) - c, r(a_2) - c, \cdots, r(a_{|\mathcal{A}|}) - c \right]$, where $c \in \mathbb{R}$ is a constant.
    
%     \textbf{d)} Combining \textbf{(a)-(c)},we can conclude that the objective function $\pi_{\theta}^{\top} r$ will undergo an update identical to that of the concave function $\pi_{\theta}^{\top} r'$ if $\theta_{a^{}} - \theta_{a} > \delta$ for all $a \neq a^{}$.
%     %
%     % \textbf{d)}
% \end{claim}


% % \textbf{Claim a).}
% % We show the function $\theta \to \pi_{\theta}(a^{*})$ is concave if $\theta_{a^{*}} - \theta_{a} > \ln 4(n-1)$ for all $a \neq a^{*}$. The proof can be easily extend to reach the convexity of the functions $\theta \to \pi_{\theta}(a)$ for all $a \neq a^{*}$. Since the concavity is determined by the behavior of a function on arbitrary line on its domain, it is sufficient to show that the following function is concave (i.e. the second derivative is non-positive) when $k \to 0$:
% % \begin{align}
% %     f(k)
% %     &= \frac{e^{\theta_{a^*} + k \cdot d_1}}{e^{\theta_{a^*} + k \cdot d_1} + e^{\theta_{a_2} + k \cdot d_2} + \cdots + e^{\theta_{a_{|\mathcal{A}|}} + k \cdot d_{|\cA|}}} \\
% %     &= \frac{1}{1 + e^{(\theta_{a_2} - \theta_{a^*}) + k \cdot (d_2 - d_1)} + \cdots + e^{(\theta_{a_{|\mathcal{A}|}} - \theta_{a^*}) + k \cdot (d_{|\cA|} - d_1)}}
% % \end{align}

% % where $d = [d_1, d_2, \cdots, d_{|\cA|}]$ is any unit vector.

% % Let:
% % \begin{align}
% %     m(k)
% %     &= e^{(\theta_{a_2} - \theta_{a^*}) + k \cdot (d_2 - d_1)} + \cdots + e^{(\theta_{a_{|\mathcal{A}|}} - \theta_{a^*}) + k \cdot (d_{|\cA|} - d_1)} \\
% %     &= \sum_{i=2}^{|\cA|} e^{(\theta_{a_i} - \theta_{a^*}) + k \cdot (d_i - d_1)}
% % \end{align}

% % Since the Taylor expansion of the sigmoid function could be written as:
% % \begin{align}
% %     \ell (x) \coloneqq \frac{1}{1+x} = 1-x+\frac{1}{2} \ell^{''}(z)\cdot x^2, \quad \text{where } z \in [0, x]
% % \end{align}

% % We have:
% % \begin{align}
% %     f(k)
% %     &= \frac{1}{1 + m(k)}\\
% %     &= 1 - m(k) + \frac{1}{2} \ell^{''}(z) \cdot m(k)^2, \quad \text{where } z \in [0, m(k)]
% % \end{align}

% % Hence, the second derivative of $f(k)$ is:
% % \begin{align}
% %     f^{''}(k) 
% %     &= -m^{''}(k) + \frac{1}{2} \ell^{''}(z) \cdot (m(k)^2)^{''} \\
% %     &= -m^{''}(k) + \frac{1}{2} \ell^{''}(z) \cdot \left[ 2 \left( m^{'}(k) \right)^2 + 2 m(k) \cdot m^{''}(k) \right] \\
% %     &= -\sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot e^{(\theta_{a_i} - \theta_{a^*}) + k \cdot (d_i - d_1)} \\
% %     & \quad + \ell^{''}(z) \left( \sum_{i=2}^{|\cA|} (d_i - d_1) \cdot e^{(\theta_{a_i} - \theta_{a^*}) + k \cdot (d_i - d_1)} \right)^2 \\
% %     & \quad + \ell^{''}(z)\sum_{i=2}^{|\cA|} e^{(\theta_{a_i} - \theta_{a^*}) + k \cdot (d_i - d_1)} \cdot \sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot e^{(\theta_{a_i} - \theta_{a^*}) + k \cdot (d_i - d_1)} 
% % \end{align}

% % And so, we have the second derivative of f(k) when $k \to 0$ is:
% % \begin{align}
% %     f^{''}(0)
% %     &= -\sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot e^{(\theta_{a_i} - \theta_{a^*})} \\
% %     & \quad + \ell^{''}(z) \left( \sum_{i=2}^{|\cA|} (d_i - d_1) \cdot e^{(\theta_{a_i} - \theta_{a^*})} \right)^2 \\
% %     & \quad + \ell^{''}(z) \left( \sum_{i=2}^{|\cA|} e^{(\theta_{a_i} - \theta_{a^*})} \right)  \left( \sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot e^{(\theta_{a_i} - \theta_{a^*})} \right) \\
% %     &\le -\sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot e^{(\theta_{a_i} - \theta_{a^*})} \label{eq:bandit_local_cocavity_1}\\
% %     & \quad + \ell^{''}(z)  \left( (|\cA|-1) \cdot \sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot e^{2 \cdot (\theta_{a_i} - \theta_{a^*})} \right) \\
% %     & \quad + \ell^{''}(z) \left(\sum_{i=2}^{|\cA|} e^{(\theta_{a_i} - \theta_{a^*})}\right) \left(\sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot e^{(\theta_{a_i} - \theta_{a^*})}\right) \\
% %     &= \left\{ \sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot  e^{(\theta_{a_i} - \theta_{a^*})} \right. \\
% %     & \quad \left. \cdot \left[ -1 + \ell^{''}(z)  (|\cA|-1) \cdot \left(e^{(\theta_{a_i} - \theta_{a^*})} \right) + \ell^{''}(z) \sum_{i=2}^{|\cA|} e^{(\theta_{a_i} - \theta_{a^*})} \right] \right\} \\
% %     & \le \left\{ \sum_{i=2}^{|\cA|} (d_i - d_1)^2 \cdot  e^{(\theta_{a_i} - \theta_{a^*})} \right. \label{eq:bandit_local_cocavity_2}\\
% %     & \quad \left. \cdot \left[ -1 + 2 \cdot (|\cA|-1) \cdot \left(e^{(\theta_{a_i} - \theta_{a^*})} \right) + 2 \cdot \sum_{i=2}^{|\cA|} e^{(\theta_{a_i} - \theta_{a^*})} \right] \right\} \label{eq:bandit_local_cocavity_3}
% % \end{align}

% % where (\ref{eq:bandit_local_cocavity_1}) holds by Cauchy-Schwarz, and (\ref{eq:bandit_local_cocavity_2}) holds since $m(k) \ge 0$ and $\frac{d^2}{d x^2} (\frac{1}{1+x})  = \frac{2}{(1+x)^3} \le 2$ for all $x \ge 0$.

% % Since the first two terms in \ref{eq:bandit_local_cocavity_2} is non-negative, we have $f^{''}(0) \le 0$ once:

% % \begin{align}
% %     -1 + 2 \cdot (|\cA|-1) \cdot \left(e^{(\theta_{a_i} - \theta_{a^*})} \right) + 2 \cdot \sum_{i=2}^{|\cA|} e^{(\theta_{a_i} - \theta_{a^*})} \le 0 \label{eq:bandit_local_cocavity_4}
% % \end{align}

% % One could easily find that (\ref{eq:bandit_local_cocavity_4}) holds while $\theta_{a^{*}} - \theta_{a_i} > \delta$ where $\delta = \ln 4(|\cA|-1) > 0$.

% \textbf{Claim a).}
% We establish the convexity of the function $\theta \to \pi_{\theta}(a)$ for all $a \neq a^{*}$ by demonstrating that if $\theta_{a^{*}} - \theta_{a} > \ln \frac{r(a_2)(|\cA|-1)}{r(a^*)-r(a_2)} + \ln (1 + \binom{|\cA|-1}{2}) - \ln(d(a^*) - d(a_i))$ for all $a \neq a^{*}$, then the function is convex. Following that, since $\pi_{\theta}(a^*) = 1 - \sum_{a \neq a^*} \pi_{\theta}(a)$ can be viewed as a summation of concave functions, it follows that $\theta \to \pi_{\theta}(a^*)$ is concave.

% Given an action $a_i \neq a^*$, since the concavity is determined by the behavior of a function on arbitrary line on its domain, it is sufficient to show that the following function is concave (i.e. the second derivative is non-positive) when $k \to 0$:
% \begin{align}
%     f(k)
%     &= \frac{e^{\theta_{a_i} + k \cdot d_i}}{e^{\theta_{a^*} + k \cdot d_1} + e^{\theta_{a_2} + k \cdot d_2} + \cdots + e^{\theta_{a_{|\mathcal{A}|}} + k \cdot d_{|\cA|}}} \\
%     &= \frac{1}{e^{(\theta_{a^*} - \theta_{a_i}) + k \cdot (d_1 - d_i)} + e^{(\theta_{a_2} - \theta_{a_i}) + k \cdot (d_2 - d_i)} + \cdots + e^{(\theta_{a_{|\mathcal{A}|}} - \theta_{a_i}) + k \cdot (d_{|\cA|} - d_i)}} \\
%     & \coloneqq \frac{1}{m(k)},
% \end{align}

% where $d = [d_1, d_2, \cdots, d_{|\cA|}]$ is any unit vector on the domain. 

% By taking the second derivative of $f(k)$, we have:
% \begin{align}
%     f^{''}(k) 
%     &= \frac{2 (m^{'}(k))^2}{m(k)^3} - \frac{m^{''}(k)}{m(k)^2}.
% \end{align}

% And so, we have the second derivative of $f(k)$ when $k \to 0$ is:
% \begin{align}
%     f^{''}(0)
%     &= \frac{1}{m(0)^2} \left( \frac{2 (m^{'}(0))^2}{m(0)} - m^{''}(0) \right). \label{eq:bandit_local_cocavity_1}
% \end{align}

% Note that since $m(k) \ge 0$ for all $k$, we have that $f^{''}(0) > 0$ (convex) if and only if:
% \begin{align}
%     2 (m^{'}(0))^2 - m^{''} (0) \cdot m(0) > 0, \label{eq:bandit_local_cocavity_2}
% \end{align}
% where $m'(0) = \sum_{a \neq a_i} (d(a) - d(a_i)) \exp(\theta_{a} - \theta_{a_i})$ and $m''(0) = \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(\theta_{a} - \theta_{a_i})$.
% % \begin{align}
% %     m'(0) = \sum_{a \neq a_i} (d(a) - d(a_i)) \exp(\theta_{a} - \theta_{a_i}) \label{eq:bandit_local_cocavity_3} \\
% %     m''(0) = \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(\theta_{a} - \theta_{a_i}) \label{eq:bandit_local_cocavity_4}
% % \end{align}

% By plugging $m(0), m'(0), m''(0)$ into (\ref{eq:bandit_local_cocavity_2}) we have:
% % \begin{align}
% %     (m'(0))^2 
% %     & = \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(2\theta_{a} - 2\theta_{a_i}) \\
% %     & \quad + \sum_{a, a' \neq a_i, a \neq a'} 2(d(a) - d(a_i)) (d(a') - d(a_i)) \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i}) \\
% %     m^{''} (0) \cdot m(0)
% %     &= \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(2\theta_{a} - 2\theta_{a_i}) \\
% %     & \quad + \sum_{a, a' \neq a_i, a \neq a'} \left( (d(a) - d(a_i))^2 + (d(a') - d(a_i))^2 \right) \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i})
% % \end{align}

% \begin{align}
%     2(m'(0))^2 - m^{''} (0) \cdot m(0)
%     & = 2 \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(2\theta_{a} - 2\theta_{a_i}) \\
%     & \quad + 2 \sum_{a, a' \neq a_i, a \neq a'} 2(d(a) - d(a_i)) (d(a') - d(a_i)) \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i}) \\
%     & \quad - \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(2\theta_{a} - 2\theta_{a_i}) \\
%     & \quad - \sum_{a, a' \neq a_i, a \neq a'} \left( (d(a) - d(a_i))^2 + (d(a') - d(a_i))^2 \right) \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i}) \\
%     & \quad - \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(\theta_{a} - \theta_{a_i}) \\
%     & = \sum_{a \neq a_i} (d(a) - d(a_i))^2 \left( \exp(2\theta_{a} - 2\theta_{a_i}) - \exp(\theta_{a} - \theta_{a_i}) \right)\\
%     & \quad + \sum_{a, a' \neq a_i, a \neq a'} 2 (d(a) - d(a_i)) (d(a') - d(a_i)) \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i}) \\
%     & \quad - \sum_{a, a' \neq a_i, a \neq a'} (d(a)^2 + d(a')^2) \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i}) \\
%     % & \quad - \sum_{a \neq a_i} (d(a) - d(a_i))^2 \exp(\theta_{a} - \theta_{a_i}) \\
%     & \ge (d(a^*) - d(a_i)) \left( \exp(2\theta_{a^*} - 2\theta_{a_i}) - \exp(\theta_{a^*} - \theta_{a_i}) \right) \\
%     & \quad -  \sum_{a, a' \neq a_i, a \neq a'} (d(a)^2 + d(a')^2) \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i}) \\
%     & \ge (d(a^*) - d(a_i))  \exp(2\theta_{a^*} - 2\theta_{a_i}) \\
%     & \quad - \left( 1 + \binom{|\cA|-1}{2} \right) \max_{a, a' \neq a_i, a \neq a'} \exp(\theta_{a} + \theta_{a'} - 2\theta_{a_i}) \\
%     &> 0, \text{if } \theta_{a^*} - \theta_{a} > \ln (1 + \binom{|\cA|-1}{2}) - \ln(d(a^*) - d(a_i)) \text{ for all } a \neq a^*.
% \end{align}

% To ensure $-\ln(d(a^*) - d(a_i))$ is bounded, we can introduce a tighter bound by considering $\delta = \ln \frac{r(a_2)(|\cA|-1)}{r(a^*)-r(a_2)} + \ln (1 + \binom{|\cA|-1}{2}) - \ln(d(a^*) - d(a_i))$. This choice of $\delta$ ensures that $\pi_\theta^\top r > r(a_2)$, which guarantees that the domain for $d_1$ is positive, while the domains for the other $d_i$ values, where $i = 2, 3, \dots, |\mathcal{A}|$, are negative.


% \textbf{Claim b)}
% Since the sum of several concave functions is itself concave, we separate our proof into 2 steps and leverages \Cref{lemma:composition_function_concave} to show that the function $\theta \to \pi_\theta(a) (r(a) - r(a_2))$ is concave for all $a \in \cA$ if $\theta_{a^{*}} - \theta_a > \delta$, for all $a \neq a^{*}$:

% \begin{itemize}
%     \item The function $\theta \to \pi_{\theta}(a^*) (r(a^*) - r(a_2))$ is concave if $\theta_{a^{*}} - \theta_a > \delta$, for all $a \neq a^{*}$: \\
%     Since we've already shown the concavity of the function $\theta \to \pi_{\theta}(a^*)$, it remains to show the concavity and the non-decrease of the function $\pi_{\theta}(a^*) \to \pi_{\theta}(a^*) \cdot (r(a^*) - r(a_2))$.
%     And this property directly hold since $\pi_{\theta}(a^*) \cdot (r(a^*) - r(a_2))$ is a linear function of $\pi_{\theta}(a^*)$ with $\frac{\partial \pi_{\theta}(a^*) \cdot (r(a^*) - r(a_2))}{\partial \pi_{\theta}(a^*)} = r(a^*) - r(a_2) > 0$ and $\frac{\partial^2 \pi_{\theta}(a^*) \cdot (r(a^*) - r(a_2))}{\partial \pi(a^*)^2} = 0$.
%     %
%     \item  The function $\theta \to \pi_{\theta}(a_i) (r(a_i) - r(a_2))$ is concave for all $i = 2, 3, \cdots, |\cA|$, if $\theta_{a^{*}} - \theta_a > \delta$, for all $a \neq a^{*}$: \\
%     %
%     Since $r(a_i) - r(a_2) \le 0$ for all $i = 2, 3, \cdots, |\cA|$, we have $\theta \to \pi_{\theta}(a_i) (r(a_i) - r(a_2)) = - \pi_{\theta}(a_i) \cdot | r(a_i) - r(a_2) |$. Also by the convexity of the function $\theta \to \pi_{\theta}(a)$, we have the function $\theta \to -\pi_{\theta}(a)$ is concave.
%     And it remains to show the concavity and the non-decrease of the function $\pi_{\theta}(a_i) \to \pi_{\theta}(a^*) \cdot | r(a_i) - r(a_2) |$.
%     This property directly hold since $\pi_{\theta}(a_i) \cdot | r(a_i) - r(a_2) |$ is a linear function of $\pi_{\theta}(a^*)$ with $\frac{\partial \pi_{\theta}(a_i) \cdot | r(a_i) - r(a_2) |}{\partial \pi_\theta(a_i)} = | r(a_i) - r(a_2) | \ge 0$ and $\frac{\partial^2 \pi_{\theta}(a_i) \cdot | r(a_i) - r(a_2) |}{\partial \pi_\theta(a_i)^2} = 0$.
%     %
% \end{itemize}

% \textbf{Claim c)}
% To reach the equivalent update result, it is sufficient to show that the gradient of the original objective $\pi_{\theta}^{\top} r$ is equal to the shifted objective $\pi_{\theta}^{\top} r'$ under all $\theta$. By \Cref{lemma:softmax_pg}, we have for all $a \in \cA$:
% \begin{align}
%     \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right|_{\theta = \theta} = \pi_\theta(a) \cdot (r(a) - \pi_{\theta}^\top r) = \pi_\theta(a) \cdot ((r(a)-c) - (\pi_{\theta}^\top r-c)) = \left.\frac{\partial \pi_{\theta}^\top r'}{\partial\theta_{a}}\right|_{\theta = \theta},
% \end{align}
% which complete our proof.

% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\banditstationarylemma*
\begin{proof}[Proof of \Cref{lemma:bandit enters local concavity}]

\begin{claim}
    The proof can be completed by making the following claims:

    \textbf{a)} Under \hyperref[algorithm:APG]{APG}, the gradient norm will not converge at the sub-optimal policy, i.e. we have $\inf_{t \ge 0, \pi_{\theta}^{(t)\top} r \in [0, r(a_2)]} \left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \theta^{(t)}} \right \| \ge \inf_{t\ge 0} \pi^{(t)}_{\theta}(a^*) \cdot (r(a^*) - r(a_2)) > 0$.

    \textbf{b)} Given any $\delta > 0$, there exist an $\epsilon > 0$ such that if $\left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \theta^{(t)}} \right \| < \epsilon$, then $\theta_{a^*} - \theta_{a} > \delta$ for all $a \ne a^*$.

    \textbf{c)} Given any $\epsilon > 0$, there exist a finite time $T$ such that $\left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \theta^{(T)}} \right \| < \epsilon$, leading to the fact that $\theta_{a^*}^{(T)} - \theta_{a}^{(T)} > \delta$ for all $a \ne a^*$ at time $T$.


    \textbf{d)} We have $\theta_{a*}^{(t)} - \theta_{a}^{(t)} > \delta$ for all $a \ne a^*, t \ge T$.
    
    % \textbf{d)} Given any $\delta > \exp(\frac{r(a_2)(|\cA|-1|)}{r(a^*)-r(a_2)})$, if $\theta_{a*}^{(t)} - \theta_{a}^{(t)} > \delta$, then $\theta_{a*}^{(t+1)} - \theta_{a}^{(t+1)} > \delta$ for all $a \ne a^*$.
    %
\end{claim}

\textbf{Claim a)}
To reach the desired result, we leverage \Cref{lemma:inf-bandit optimal} to ensure the gradient norm is bounded away from $0$ before achieving optimal policy:
\begin{align}
    \left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \theta^{(t)}} \right \|
    &= \sqrt{\sum_{a \in \cA} \pi^{(t)}_{\theta}(a)^2 \cdot (r(a) - \pi_{\theta}^{(t)\top} r)^2} \label{eq:bandit enters local concavity 1} \\
    &\ge \sqrt{ \pi^{(t)}_{\theta}(a^*)^2 \cdot (r(a^*) - \pi_{\theta}^{(t)\top} r)^2} \label{eq:bandit enters local concavity 2} \\
    &= \pi^{(t)}_{\theta}(a^*) \cdot (r(a^*) - \pi_{\theta}^{(t)\top} r) \label{eq:bandit enters local concavity 3} \\
    &\ge \inf_{t\ge 0} \pi^{(t)}_{\theta}(a^*) \cdot (r(a^*) - r(a_2)) \\
    & > 0, \quad \text{for all } \pi_{\theta}^{(t)\top} r \in [0, r(a_2)], \label{eq:bandit enters local concavity 4}
\end{align}
where (\ref{eq:bandit enters local concavity 1}) is followed by \Cref{lemma:softmax_pg} and (\ref{eq:bandit enters local concavity 4}) is by \Cref{lemma:inf-bandit optimal}.

\textbf{Claim b)}
By choosing $\epsilon$ with:
\begin{align}
\epsilon = \min & \left \{ \inf_{t \ge 0, \pi_{\theta}^{(t)\top} r \in [0, r(a_2)]} \left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \theta^{(t)}} \right \|, \right. \\
& \left. \frac{1}{e^\delta + |\cA|-1} \cdot \inf_{t \ge 0, a \ne a^*, \pi_{\theta}^{(t)\top} r \in (r(a_2), r(a^*)]} | r(a) - \pi_{\theta}^{(t) \top} r | \right \} > 0, 
\end{align}
we could ensure that the minimum must occur at $\pi_\theta^{\top} r \in (r(a_2), r(a^*)]$. And so we have $\inf_{t \ge 0, a \ne a^*, \pi_{\theta}^{(t)\top} r \in (r(a_2), r(a^*)]} | r(a) - \pi_{\theta}^{(t) \top} r | > 0$.

Hence, by \Cref{lemma:softmax_pg}, we have for all $a \in \cA$:
\begin{align}
    % \frac{\min_{a \ne a^*} |r(a) - r(a^*)|}{e^\delta + (|\cA|-1)}
    \frac{\inf_{t \ge 0, a \ne a^*, \pi_{\theta}^{(t)\top} r \in (r(a_2), r(a^*)]} | r(a) - \pi_{\theta}^{(t) \top} r |}{e^\delta + (|\cA|-1)} > \left \| \nabla_{\theta} \pi_{\theta}^{\top} r \right \| \ge  \pi_{\theta}(a) \cdot |r(a) - \pi_{\theta}^{\top} r| \label{eq:bandit enters local concavity 5}
\end{align}
by rearranging (\ref{eq:bandit enters local concavity 5}), we get:
% \begin{align}
%     \frac{1}{e^\delta + (|\cA|-1)} \ge \frac{\min_{a \ne a^*} |r(a) - r(a^*)|}{|r(a) - \pi_{\theta}^{\top} r|}\cdot \frac{1}{e^\delta + (|\cA|-1)}  > \pi_{\theta}(a)
% \end{align}
\begin{align}
    \frac{1}{e^\delta + (|\cA|-1)} \ge \frac{\inf_{t \ge 0, a \ne a^*, \pi_{\theta}^{(t)\top} r \in (r(a_2), r(a^*)]} | r(a) - \pi_{\theta}^{(t) \top} r |}{|r(a) - \pi_{\theta}^{\top} r|}\cdot \frac{1}{e^\delta + (|\cA|-1)}  > \pi_{\theta}(a)
\end{align}
for all $a \ne a^*$, leading to our desired result.

% And since $[e^\delta + (|\cA|-1)]^{-1} > \pi_{\theta_t}(a)$ for some $t \le N$, for all $a \ne a^*$, we have:
% \begin{align}
%     \frac{\pi_{\theta_t} (a^*)}{\pi_{\theta_t} (a)} > \frac{\frac{e^\delta}{e^\delta + (n-1)}}{\frac{1}{e^\delta + (n-1)}} = e^\delta
% \end{align}
% which is equivalent to our desired result:
% \begin{align}
%     \theta_t(a^*) - \theta_t(a) > \delta
% \end{align}
% for all $a \ne a^*$.

\textbf{Claim c)}
By \Cref{theorem:convergeoptimal}, we have that there exist a finite time $T_0$ such that $\theta_{a^{*}}^{(t)} > \theta_{a}^{(t)}$ for all $a \neq a^*$ and $\theta_{a}^{(t)}$ will be decreasing for all $a \neq a^*$ for all $ t \ge T_0$. If we run $K$ iterations, the above statement leads to the fact that $\max_{k=1,2,\cdots, K} \left\| \theta^{(k)} \right \|^2 \le \max_{t' \le T_0} \left\| \theta^{(t')} \right \|^2 + |\cA| (\theta_{a^{*}}^{(K)})^2$. We discuss two possible cases as follows:

\begin{itemize}
    \item \textbf{Case 1:} $\theta_{a^{*}}^{(K)} \le 2\ln(K) + \max_{t' \le T_0, a \neq a^*} \{\theta_a^{(t')} \} + \ln(|\cA| - 1)$:
    
    By \Cref{cor:ghadimi_cor2} with the surrogate optimal solution $\theta^{**} \coloneqq \theta^{(K)**} \coloneqq [2\ln(K), 0, 0, \cdots, 0]$, we have:
    \begin{align}
        \min_{k=1,2,\cdots,K} \left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \theta^{(k)}} \right \| 
        &\le 192 L^2 \frac{\left \| \theta^{(0)}  - \theta^{(K)**} \right \|}{K(K+1)(2K+1)} + \frac{48 L^2 }{2K + 1}(4| \ln(K) |^2 + \max_{k=1,2,\cdots, K} \left\| \theta^{(k)} \right \|^2) \\
        &\quad + \frac{48L \cdot | V^{\pi_{\theta^{(K)}}}(\mu) - V^{\pi_{\theta^{**}}}(\mu) |}{2K+1} \\
        &\le 192 L^2 \frac{\left \| \theta^{(0)} \right \| + 2| \ln(K)|}{K(K+1)(2K+1)} \\
        & \quad + \frac{48 L^2 }{2K + 1}(4| \ln(K) |^2 + \max_{t' \le T_0} \left\| \theta^{(t')} \right \|^2 + |\cA| (2\ln(K) + \max_{t' \le T_0, a \neq a^*} \{\theta_a^{(t')} \} + \ln(|\cA| - 1))^2) \\
        &\quad + \frac{48L \cdot | V^{\pi_{\theta^{(K)}}}(\mu) - V^{\pi_{\theta^{**}}}(\mu) |}{2K+1} \\
        & = \tilde{O}(\frac{1}{K}).
    \end{align}

    Hence the result directly holds by choosing (by changing variable from $K$ to $t$),
    \begin{align}
        T = \inf \Biggl\{ t: \epsilon &\ge 192 L^2 \frac{\left \| \theta^{(0)} \right \| + 2| \ln(t)|}{t(t+1)(2t+1)} \\
        & \quad + \frac{48 L^2 }{2t + 1}(4| \ln(t) |^2 + \max_{t \le T_0} \left\| \theta^{(t)} \right \|^2 + |\cA| (2\ln(t) + \max_{t \le T_0, a \neq a^*} \{\theta_a \} + \ln(|\cA| - 1))^2) \\
        &\quad + \frac{48L \cdot | V^{\pi_{\theta^{(t)}}}(\mu) - V^{\pi_{\theta^{**}}}(\mu) |}{2t+1} \Biggl\}.
    \end{align}
    
    \item \textbf{Case 2:} $\theta_{a^{*}}^{(K)} > 2\ln(K) + \max_{t' \le T_0, a \neq a^*} \{\theta_a^{(t')} \} + \ln(|\cA| - 1)$:
    
    Given such $\theta_{a^{*}}^{(K)}$, we have:
    \begin{align}
        \pi_\theta^{(K)}(a^*) = \frac{\exp(\theta_{a^{*}}^{(K)})}{\sum_{a \in \cA} \exp(\theta_{a}^{(K)})} > \frac{\exp(2\ln(K))}{\exp(2\ln(K)) + \sum_{a \neq \cA} \exp(-\ln(|\cA| - 1))} \ge \frac{K^2}{K^2 + 1}.
    \end{align}
    And hence we have:
    \begin{align}
        \left \| \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta}\Big\rvert_{\theta = \theta^{(K)}} \right \|
        &= \sqrt{\sum_{a \in \cA} \pi^{(K)}_{\theta}(a)^2 \cdot (r(a) - \pi_{\theta}^{(K)\top} r)^2} \\
        &\le \sqrt{(r(a^*) - \pi_{\theta}^{(K)\top} r)^2 + \sum_{a \neq a^*} \pi^{(K)}_{\theta}(a)^2} \\
        &\le \sqrt{\frac{1}{(K^2+1)^2} + \frac{1}{(K^2+1)^2} } \\
        &\le \frac{\sqrt{2}}{K^2+1}.
    \end{align}

    Hence the result directly holds by choosing (by changing variable from $K$ to $t$),
    \begin{align}
        T = \inf \Biggl\{ t: \epsilon &\ge \frac{\sqrt{2}}{t^2+1} \Biggl\}.
    \end{align}
    
\end{itemize}

\textbf{Claim d)}
We elaborate on each action $a \neq a^*$ separately. For a fix $a \neq a^*$, since there exists a finite $T$ such that $\theta_{a^*}^{(T)} - \theta_{a}^{(T)} > \delta$ provided by Claim (c), there is a $T_a$ such that $T_a \le T$, $\theta_{a^*}^{(T_a)} - \theta_{a}^{(T_a)} > \delta$, and $\theta_{a^*}^{(T_a - 1)} - \theta_{a}^{(T_a - 1)} \le \delta$. Then, we have
\begin{equation}
\label{eq:lemma2-claimd-eq1}
    \theta_{a^*}^{(T_a)} - \theta_{a^*}^{(T_a-1)} > \theta_{a}^{(T_a)} - \theta_{a}^{(T_a-1)}
\end{equation}

We first show two useful properties:

\textbf{(i)} If $\theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta$ and $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} \ge \omega_{a}^{(t)} - \theta_{a}^{(t)}$, then $\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right\rvert_{\theta = \omega^{(t)}} \ge \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right\rvert_{\theta = \omega^{(t)}}$.

Since $\theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta > 0$, it follows that
\begin{align}
    \omega_{a^*}^{(t)} &= \theta_{a^*}^{(t)} + (\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)}) \\
    &> \theta_{a}^{(t)} + (\omega_{a}^{(t)} - \theta_{a}^{(t)}) \\
    &=  \omega_{a}^{(t)}.
\end{align}

By \Cref{lemma:softmax_pg}, we have
\begin{align}
    \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right\rvert_{\theta = \omega^{(t)}} &= \pi_{\omega^{(t)}}(a^*) \cdot (r(a^*) - \pi_{\omega^{(t)}}^{\top} r) \\
    &\ge \pi_{\omega^{(t)}}(a) \cdot (r(a) - \pi_{\omega^{(t)}}^{\top} r) \label{eq:lemma2-claimd-eq} \\
    &= \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right\rvert_{\theta = \omega^{(t)}},
\end{align}
where (\ref{eq:lemma2-claimd-eq}) holds because of that $\omega_{a^*}^{(t)} > \omega_{a}^{(t)}$ and thus $\pi_{\omega^{(t)}}(a^*) > \pi_{\omega^{(t)}}(a)$, and $r(a^*) > r(a)$.

\textbf{(ii)} If $\theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta$, $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} \ge \omega_{a}^{(t)} - \theta_{a}^{(t)}$, and $\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right\rvert_{\theta = \omega^{(t)}} \ge \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right\rvert_{\theta = \omega^{(t)}}$, then $\theta_{a^*}^{(t+1)} - \theta_{a}^{(t+1)} > \delta$ and $\omega_{a^*}^{(t+1)} - \theta_{a^*}^{(t+1)} \ge \omega_{a}^{(t+1)} - \theta_{a}^{(t+1)}$.

For $\theta_{a^*}^{(t+1)} - \theta_{a}^{(t+1)} > \delta$,
\begin{align}
    \theta_{a^*}^{(t+1)} - \theta_{a}^{(t+1)} &= \left(\theta_{a^*}^{(t)} + (\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)}) + \eta^{(t+1)} \cdot \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right\rvert_{\theta = \omega^{(t)}}\right) - \left(\theta_{a}^{(t)} + (\omega_{a}^{(t)} - \theta_{a}^{(t)}) + \eta^{(t+1)} \cdot \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right\rvert_{\theta = \omega^{(t)}}\right) \\
    &\ge \theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta. \label{eq:lemma2 grad-mom-dominate}
\end{align}
For $\omega_{a^*}^{(t+1)} - \theta_{a^*}^{(t+1)} \ge \omega_{a}^{(t+1)} - \theta_{a}^{(t+1)}$, 

\begin{align}
    \omega_{a^*}^{(t+1)} - \theta_{a^*}^{(t+1)} &= \frac{t}{t+3}(\theta_{a^*}^{(t+1)} - \theta_{a^*}^{(t)})  \\
    &= \frac{t}{t+3}\left(\omega^{(t)}_{a^*} - \theta^{(t)}_{a^*} + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right|_{\theta = \omega^{(t)}}\right)  \\
    &\ge \frac{t}{t+3}\left(\omega^{(t)}_{a} - \theta^{(t)}_{a} + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right|_{\theta = \omega^{(t)}}\right) \label{eq:lemma2-claimd-eq2} \\
    &= \frac{t}{t+3}(\theta_{a}^{(t+1)} - \theta_{a}^{(t)})  \\ 
    &= \omega_{a}^{(t+1)} - \theta_{a}^{(t+1)}, 
\end{align}
where (\ref{eq:lemma2-claimd-eq2}) is followed by the given hypotheses $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} \ge \omega_{a}^{(t)} - \theta_{a}^{(t)}$ and $\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right|_{\theta = \omega^{(t)}} \ge \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right|_{\theta = \omega^{(t)}}$.

By the above two properties, it suffices to show that there is $T'$ such that $\theta_{a^*}^{(T')} - \theta_{a}^{(T')} > \delta$ and $\omega_{a^*}^{(T')} - \theta_{a^*}^{(T')} \ge \omega_{a}^{(T')} - \theta_{a}^{(T')}$, then we will obtain that $\theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta$ for any $t \ge T'$.

We claim that $T' = T_a$.
Since $T_a$ satisfies $\theta_{a^*}^{(T_a)} - \theta_{a}^{(T_a)} > \delta$, we only need to show that $\omega_{a^*}^{(T_a)} - \theta_{a^*}^{(T_a)} \ge \omega_{a}^{(T_a)} - \theta_{a}^{(T_a)}$. To check the condition, we directly expand $\omega_{a^*}^{(T_a)} - \theta_{a^*}^{(T_a)}$, we obtain
\begin{align}
    \omega_{a^*}^{(T_a)} - \theta_{a^*}^{(T_a)} &= \frac{T_a - 1}{T_a + 2} (\theta_{a^*}^{(T_a)} - \theta_{a^*}^{(T_a-1)}) \label{eq:lemma2-claimd-eq3}\\
    &> \frac{T_a - 1}{T_a + 2} (\theta_{a}^{(T_a)} - \theta_{a}^{(T_a-1)}) \label{eq:lemma2-claimd-eq4}\\
    &= \omega_{a}^{(T_a)} - \theta_{a}^{(T_a)},\label{eq:lemma2-claimd-eq5}
\end{align}
where (\ref{eq:lemma2-claimd-eq3}), (\ref{eq:lemma2-claimd-eq5}) use the update of APG, and (\ref{eq:lemma2-claimd-eq4}) holds by (\ref{eq:lemma2-claimd-eq1}). Therefore, we show that $\theta_{a^*}^{(T_a)} - \theta_{a}^{(T_a)} > \delta$ and $\omega_{a^*}^{(T_a)} - \theta_{a^*}^{(T_a)} \ge \omega_{a}^{(T_a)} - \theta_{a}^{(T_a)}$. Hence, $\theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta$ for any $t \ge T_a$.

Since the above statement holds for any action $a \neq a^*$, we obtain that $\theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta$ for all $a \neq a^*, t \ge \max_{a \neq a^*} T_a$. Additionally, $T \ge \max_{a \neq a^*} T_a$, so $\theta_{a^*}^{(t)} - \theta_{a}^{(t)} > \delta$ for all $a \neq a^*, t \ge T$.

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}
% \label{lemma:inf-bandit optimal}
%     Under APG, we have $\inf_{t\ge 0} \pi^{(t)}(a^*) > 0$.
% \end{lemma}
\banditinfbddlemma*
\begin{remark} 
\normalfont Inspired by the proof of \citep{mei2020global}, we consider two ``nice regions'' in terms of time: one region (we call it ``gradient region'') characterized by a positive partial derivative with respect to the optimal action and the negative partial derivatives of all other actions, and another region (we call it ``momentum region'') characterized by the maximum momentum of the optimal action. If our training process enters these regions, we can ensure that the probability of selecting the optimal action does not decrease. Consequently, the infimum of $\pi_{\theta}^{(t)}(a^*)$ will remain greater than zero. It is important to highlight that our approach selects a more aggressive gradient region compared to the one chosen in \citep{mei2020global}. By doing so, we are able to streamline their proof to some extent without oversimplifying it.
\end{remark}
\begin{proof}[Proof of \Cref{lemma:inf-bandit optimal}]
%\naich{check to match the asymptotic convergence theorem statement}

Firstly, we define two sets consisting of time indices with great properties of gradient and momentum.
    \begin{align}
        \mathcal{R}_1 &= \left\{t : \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right\rvert_{\theta = \omega^{(t)}} \ge 0 \ge \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right\rvert_{\theta = \omega^{(t)}}, \text{ for all } a \neq a^*\right\}, \label{lemma: inf-bandit R1}\\
        \mathcal{R}_2 &= \left\{t : \omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} \ge \omega_{a}^{(t)} - \theta_{a}^{(t)}, \text{ for all } a \neq a^*\right\}. \label{lemma: inf-bandit R2}
    \end{align}
    Inspired by \citep{mei2020global}, we make the following claims, and then prove these claims immediately as follows.


    \begin{claim}
        The following hold:
        
        \textbf{a)} There exists a finite $T_1$ such that if $t \ge T_1$, then $\pi^{(t)}_{\theta}(a^*) \ge \frac{r(a_2)}{r(a^*)}$ and $\pi^{(t)}_{\omega}(a^*) \ge \frac{r(a_2)}{r(a^*)}$.
    
        \textbf{b)} If $t \ge T_1$, then $t \in \mathcal{R}_1$.
        
        \textbf{c)} There exists a finite $T_2 \ge T_1$ such that if $t \ge T_2$, then $t \in \mathcal{R}_2$.

        \textbf{d)} If $t \ge T_2$, then $t \in \mathcal{R}_1 \cap \mathcal{R}_2$. Moreover, we have $\pi^{(t+1)}_{\theta}(a^*) \ge \pi^{(t)}_{\theta}(a^*)$. Hence, it follows that
        \begin{equation}
            \inf_{t \ge 0} \pi^{(t)}_{\theta}(a^*) = \min_{0 \le t \le T_2} \pi^{(t)}_{\theta}(a^*).
        \end{equation}
    \end{claim}
    \textbf{Claim a).} By the asymptotic global convergence in \Cref{theorem:convergeoptimal}, we have that $\pi^{(t)}_{\theta}(a^*) \rightarrow 1$ and $\pi^{(t)}_{\omega}(a^*) \rightarrow 1$ as $t \rightarrow \infty$. Since $a^*$ is unique, $\frac{r(a_2)}{r(a^*)} < 1$. According to the $\epsilon-\delta$ argument of limit, there exists a finite $T_1$ such that if $t \ge T_1$, then $\pi^{(t)}_{\theta}(a^*) \ge \frac{r(a_2)}{r(a^*)}$ and $\pi^{(t)}_{\omega}(a^*) \ge \frac{r(a_2)}{r(a^*)}$.

    \textbf{Claim b).} Given $t \ge T_1$, by \Cref{lemma:softmax_pg}, we have
    \begin{align}
        \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right\rvert_{\theta = \omega^{(t)}} &= \pi_{\omega}^{(t)}(a^*) (r(a^*) - \pi^{(t)\top}_{\omega}r) \ge 0, \label{lemma: inf-bandit eq1}
    \end{align}
    where (\ref{lemma: inf-bandit eq1}) holds by $r(a^*)$ is always greater than or equal to the convex combination of rewards. Regarding the sub-optimal actions $a \neq a^*$, 
    \begin{align}
        \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right\rvert_{\theta = \omega^{(t)}} &= \pi_{\omega}^{(t)}(a) (r(a) - \pi^{(t)\top}_{\omega}r) \\ 
        &\le \pi_{\omega}^{(t)}(a) (r(a) - \pi^{(t)}_{\omega}(a^*) r(a^*)) \label{lemma: inf-bandit eq2}\\
        &\le \pi_{\omega}^{(t)}(a)(r(a) - r(a_2)) \label{lemma: inf-bandit eq3} \\
        &\le 0,\label{lemma: inf-bandit eq4}
    \end{align}
    where (\ref{lemma: inf-bandit eq2}) holds since we ignore the terms $\pi^{(t)}_{\omega}(a) r(a) \ge 0$ for every $a \neq a^*$, and (\ref{lemma: inf-bandit eq3}) holds because $t \ge T_1$, we have $\pi^{(t)}_{\omega}(a^*) \ge \frac{r(a_2)}{r(a^*)}$. Combining (\ref{lemma: inf-bandit eq1}-\ref{lemma: inf-bandit eq4}), we obtain $t\in\mathcal{R}_1$.

    \textbf{Claim c).} Part (i): We show that for $t \ge T_1$ and any $a \in \cA$, if $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} \ge \omega_{a}^{(t)} - \theta_{a}^{(t)}$, then $\omega_{a^*}^{(t+1)} - \theta_{a^*}^{(t+1)} \ge \omega_{a}^{(t+1)} - \theta_{a}^{(t+1)}$. By combining the updates (\ref{algorithm:eq1}) and (\ref{algorithm:eq3}), we have
    \begin{align}
        \theta^{(t+1)}_{a} \leftarrow \theta^{(t)}_{a} + (\omega^{(t)}_{a} - \theta^{(t)}_{a}) + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right|_{\theta = \omega^{(t)}}. \label{lemma: inf-bandit eq5}
    \end{align}
    By using the update (\ref{algorithm:eq3}) of \hyperref[algorithm:APG]{APG} with respect to the action $a^*$ and (\ref{lemma: inf-bandit eq5}),
    \begin{align}
        \omega_{a^*}^{(t+1)} - \theta_{a^*}^{(t+1)} &= \frac{t}{t+3}(\theta_{a^*}^{(t+1)} - \theta_{a^*}^{(t)}) \label{lemma: inf-bandit eq6} \\
        &= \frac{t}{t+3}\left(\omega^{(t)}_{a^*} - \theta^{(t)}_{a^*} + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right|_{\theta = \omega^{(t)}}\right) \label{lemma: inf-bandit eq7} \\
        &\ge \frac{t}{t+3}\left(\omega^{(t)}_{a} - \theta^{(t)}_{a} + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right|_{\theta = \omega^{(t)}}\right) \label{lemma: inf-bandit eq8} \\
        &= \frac{t}{t+3}(\theta_{a}^{(t+1)} - \theta_{a}^{(t)}) \label{lemma: inf-bandit eq9} \\ 
        &= \omega_{a}^{(t+1)} - \theta_{a}^{(t+1)}, \label{lemma: inf-bandit eq10}
    \end{align}
    where (\ref{lemma: inf-bandit eq8}) is followed by the hypothesis $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} \ge \omega_{a}^{(t)} - \theta_{a}^{(t)}$ and $t \ge T_1$ so $\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right|_{\theta = \omega^{(t)}} \ge \left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right|_{\theta = \omega^{(t)}}$.
    We finish the proof of Part (i).

    Part (ii): We show that there exists a finite $T_2 \ge T_1$ such that if $t \ge T_2$, then $t \in \cR_2$. We prove it by contradiction. Suppose that there is no such $T_2$. Thus, there are infinitely many $t \ge T_1$ such that there is an action $a$ violating the condition of lying in $\cR_2$ at time $t$, i.e., $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} < \omega_{a}^{(t)} - \theta_{a}^{(t)}$, as the definition (\ref{lemma: inf-bandit R2}) of $\cR_2$. Since our action space is finite, there is an action $\tilde{a}$ such that $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} < \omega_{\tilde{a}}^{(t)} - \theta_{\tilde{a}}^{(t)}$ holds for infinitely many $t \ge T_1$.
    
    We claim that there is a $\tilde{T} \ge T_1$ such that for all $t \ge \tilde{T}$, $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} < \omega_{\tilde{a}}^{(t)} - \theta_{\tilde{a}}^{(t)}$. If not, there is a $t_0 \ge T_1$ such that $\omega_{a^*}^{(t_0)} - \theta_{a^*}^{(t_0)} \ge \omega_{a}^{(t_0)} - \theta_{a}^{(t_0)}$, then by Part (i), $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} \ge \omega_{a}^{(t)} - \theta_{a}^{(t)}$ holds for every $t \ge t_0$, which contradicts to $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} < \omega_{\tilde{a}}^{(t)} - \theta_{\tilde{a}}^{(t)}$ holds for infinitely many $t \ge T_1$. Thus, there is a $\tilde{T} \ge T_1$ such that for all $t \ge \tilde{T}$, $\omega_{a^*}^{(t)} - \theta_{a^*}^{(t)} < \omega_{\tilde{a}}^{(t)} - \theta_{\tilde{a}}^{(t)}$.

    To meet the contradiction, for any $N > \tilde{T}$, we consider
    \begin{align}
        \theta_{a^*}^{(N)} &= \theta_{a^*}^{(\tilde{T})} + \sum_{t=\tilde{T}}^{N-1} (\theta_{a^*}^{(t+1)} - \theta_{a^*}^{(t)}) \label{lemma: inf-bandit eq11} \\
        &= \theta_{a^*}^{(\tilde{T})} + \sum_{t=\tilde{T}}^{N-1} \frac{t+3}{t}(\omega_{a^*}^{(t+1)} - \theta_{a^*}^{(t+1)}) \label{lemma: inf-bandit eq12} \\
        &< \theta_{a^*}^{(\tilde{T})} + \sum_{t=\tilde{T}}^{N-1} \frac{t+3}{t}(\omega_{\tilde{a}}^{(t+1)} - \theta_{\tilde{a}}^{(t+1)}) \label{lemma: inf-bandit eq13} \\
        &= \theta_{a^*}^{(\tilde{T})} + \sum_{t=\tilde{T}}^{N-1} \frac{t+3}{t}\left[\frac{t}{t+3}(\theta_{\tilde{a}}^{(t+1)} - \theta_{\tilde{a}}^{(t)})\right] \label{lemma: inf-bandit eq14} \\
        &=\theta_{a^*}^{(\tilde{T})} + \sum_{t=\tilde{T}}^{N-1} (\theta_{\tilde{a}}^{(t+1)} - \theta_{\tilde{a}}^{(t)}) \label{lemma: inf-bandit eq15} \\
        &= \theta_{a^*}^{(\tilde{T})} - \theta_{\tilde{a}}^{(\tilde{T})} + \theta_{\tilde{a}}^{(N)}, \label{lemma: inf-bandit eq16}
    \end{align}
    where (\ref{lemma: inf-bandit eq11}) uses a simple telescope argument, (\ref{lemma: inf-bandit eq12}) uses the update (\ref{algorithm:eq3}) of \hyperref[algorithm:APG]{APG}, (\ref{lemma: inf-bandit eq13}) holds since $t \ge \tilde{T}$, (\ref{lemma: inf-bandit eq14}) uses the update (\ref{algorithm:eq3}).

    Since (\ref{lemma: inf-bandit eq16}) holds for arbitrary $N > \tilde{T}$, we obtain $\theta_{a^*}^{(N)} < \theta_{a^*}^{(\tilde{T})} - \theta_{\tilde{a}}^{(\tilde{T})} + \theta_{\tilde{a}}^{(N)}$ for any $N > \tilde{T}$, which contradicts $\pi^{(t)}_{\theta}(a^*) \rightarrow 1$ as $t\rightarrow\infty$, {i.e., the asymptotic global convergence theorem}. Hence, there is a $T_2 \ge T_1$ such that if $t \ge T_2$, then $t \in \cR_2$.

    \textbf{Claim d).} Given $t \ge T_2$, we have $t \in \mathcal{R}_2$. In addition, since $T_2 \ge T_1$, we also have $t \in \mathcal{R}_1$. Thus, $t \in \mathcal{R}_1 \cap \mathcal{R}_2$. Then, to show that $\pi^{(t+1)}_{\theta}(a^*) \ge \pi^{(t)}_{\theta}(a^*)$, we have
    \begin{align}
        \pi^{(t+1)}_{\theta}(a^*) &= \frac{\exp\{\theta^{(t+1)}_{a^*}\}}{\sum_{a\in \cA} \exp\{\theta^{(t+1)}_{a}\}} \\
        &= \frac{\exp\left\{\theta^{(t)}_{a^*} + (\omega^{(t)}_{a^*} - \theta^{(t)}_{a^*}) + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right|_{\theta = \omega^{(t)}}\right\}}{\sum_{a\in \cA} \exp\left\{\theta^{(t)}_{a} + (\omega^{(t)}_{a} - \theta^{(t)}_{a}) + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a}}\right|_{\theta = \omega^{(t)}}\right\}} \label{lemma: inf-bandit eq17} \\
        &\ge \frac{\exp\left\{\theta^{(t)}_{a^*} + (\omega^{(t)}_{a^*} - \theta^{(t)}_{a^*}) + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right|_{\theta = \omega^{(t)}}\right\}}{\sum_{a\in \cA} \exp\left\{\theta^{(t)}_{a} + (\omega^{(t)}_{a^*} - \theta^{(t)}_{a^*}) + \eta^{(t+1)}\left.\frac{\partial \pi_{\theta}^\top r}{\partial\theta_{a^*}}\right|_{\theta = \omega^{(t)}}\right\}} \label{lemma: inf-bandit eq18} \\
        &= \frac{\exp\{\theta^{(t)}_{a^*}\}}{\sum_{a\in \cA} \exp\{\theta^{(t)}_{a}\}} = \pi^{(t)}_{\theta}(a^*),
    \end{align}
    where (\ref{lemma: inf-bandit eq17}) holds by (\ref{lemma: inf-bandit eq5}) and (\ref{lemma: inf-bandit eq18}) leverages the properties of $\cR_1$ and $\cR_2$ as the definitions (\ref{lemma: inf-bandit R1}) and (\ref{lemma: inf-bandit R2}). Therefore, $\pi_{\theta}^{(t)}(a^*)$ is non-decreasing after $T_2$. Hence, it follows that
    \begin{equation}
        \inf_{t \ge 0} \pi^{(t)}_{\theta}(a^*) = \min_{0 \le t \le T_2} \pi^{(t)}_{\theta}(a^*) > 0.
    \end{equation}
\end{proof}
%%%%%%%%%%
\newpage
\subsection{Lower Bound of Sub-Optimality Under APG}
\label{app:bandit:lower}

\lowerbddthm*
\begin{proof}[Proof of \Cref{theorem:lower bounded case}] 
\phantom{}
%\mru{TBD}
Given the reward function $r(a^*) = 1, r(a_2) = 0$, we know ${\pi_{\theta}^{(t)}}^{\top} r=\pi_{\theta}^{(t)}(a^*)$, and hence we could focus on $\theta_{a^*}^{(t)}$. Moreover, by Lemma \ref{lemma:sum conservation} and the initialization $\theta^{(0)}_{a^*} = \theta^{(0)}_{a_2} = 0$, we know $\theta_{a^*}^{(t)}+\theta_{a_2}^{(t)}=0$, for all $t$.
Under APG, in this two-armed bandit case, we have
\begin{equation}
    \theta^{(t+1)}=\theta^{(t)}+\frac{t-1}{t+2}(\theta^{(t)}-\theta^{(t-1)})+\eta^{(t+1)}\cdot\nabla (\pi_{\theta}^{\top} r)\big\rvert_{\theta={\omega}^{(t)}}.
\end{equation}
Under the learning rate $\eta^{(t)} = \frac{t}{t+1} \cdot \frac{1}{5}$, one could iteratively verify that $\ln(t+1)-2\leq \theta^{(t)}_{a^*}\leq \ln(t+1)-1$, for all $t\geq 2$.
This implies that the sub-optimality gap is $\Omega(\frac{1}{t^2})$. 

\end{proof}

\begin{comment}

\begin{prop}
\label{prop:lower_bdd_gradient}
Under APG, we have $\inf_{t \ge 1, \pi_{\theta_t}^{\top} r \in [0, r(a_2)]} \left \| \frac{\partial \pi_{\theta_t}^{\top} r}{\partial \theta} \right \| > 0$. \mru{(Note that we can also levergae Non-uniform PL codition to reach this property.)}
\end{prop}

\begin{remark}
    We leverage \Cref{prop:lower_bdd_gradient} to show that the stationary point will only occur at the interval $( r_2, r_1 ]$, which is important while proving \Cref{lemma:stationary_point}.
\end{remark}

\begin{proof}[Proof of \Cref{prop:lower_bdd_gradient}]  
\phantom{}
Since $\frac{\partial \pi_{\theta}^{\top} r}{\partial \theta_{a_i}} = \pi_{\theta_{a_i}} \cdot (r(a_i) - \pi_{\theta}^{\top} r)$ \mru{(ref?)} and there must exist at least one action $a$ such that $\pi_\theta(a) > 0$, the zero gradient point could only occur at $\pi_\theta(a) = 1$ for some $a \ne a^*$. So it remains to show that there exists a $\epsilon > 0$ such that $\pi_{\theta_t}(a) < 1-\epsilon$ for all $t, a \ne a^*$.
% $\inf_{t \ge 1} \left \| \frac{\partial \pi_{\theta_t}^{\top} r}{\partial \theta} \right \| > 0$ while $\pi_{\theta}^{\top} r \in [r-\epsilon, r+\epsilon]$ for all $r \ne r(a^*)$.

To show the above property, we discuss two possible cases as follows, for any $\bar{a} \ne a^*$:

\begin{itemize}
    \item There exists a time $T_1$ such that $\pi_{\theta_{T_1}}^{\top} r > r(\bar{a})$:
    
    Since once we have $\pi_{\theta_{T_1}}^{\top} r > r(\bar{a})$, it will hold for all $t > T_1$, so we have $\frac{\partial \pi_{\theta_t}^{\top} r}{\partial \theta(\bar{a})} = \pi_{\theta_t}(\bar{a}) \cdot (r(\bar{a}) - \pi_{\theta_t}^{\top} r) < 0$ for all $t > T_1$, and since the momentum term under \mru{APG} is bounded above, we have that it must exists a finite time $T_2$ such that $\theta_{t+1}(\bar{a}) - \theta_{t}(\bar{a}) < 0$ for all $t > T_2$, leading to the fact that $\pi_{\theta_t}(\bar{a})$ must be bounded away from 1.

    \item $\pi_{\theta_t}^{\top} r \le r(\bar{a})$ for all $t$:

    We complete this part of the proof by contradiction. Assume that for all $\epsilon > 0$, there exists a time $T_1$ such that $\pi_{\theta_{T_1}}(\bar{a}) \ge 1-\epsilon$. Hence for all $\delta > 0$, there exists a time $T_2$ such that $\theta_{T_2}(\bar{a}) \ge \delta$. Also, since $\sum_{a \in \mathcal{A}} \theta_t(a) = \sum_{a \in \mathcal{A}} \theta_0(a)$ for all $t$ and $\theta_{t+1}(a) - \theta_{t}(a) > 0$ for all $r(a) > r(\bar{a}), t$, we have:
    \begin{align}
        \sum_{a \in \mathcal{A}, r(a) < r(\bar{a})} \theta_{T_2}(a) \le \sum_{a \in \mathcal{A}, r(a) < r(\bar{a})} \theta_0(a) - \delta 
    \end{align}
    given $\theta_{T_2}(\bar{a}) \ge \delta$. \\
    Moreover, since $\frac{\partial \pi_{\theta}^{\top} r}{\partial \theta(a)} = \pi_\theta(a) \cdot (r(a) - \pi_{\theta}^{\top} r)$ and $\pi_{\theta_t}(\bar{a}) \to 1$, we have that $(r(a) - \pi_{\theta_t}^{\top} r) \to r(a) - r(\bar{a})$ and hence the gradient magnitude will be dominated by $\pi_\theta(a)$ for each action $a$. So, each term in the summation of the left hand side inequality above will approach negative infinity by different rate determined by the ratio of the Advantage value as $\theta(\bar{a}) \to \infty$. Hence, for all $\delta_1 > 0$, one could choose a large enough $\delta$ to ensure that $\theta(a) < -\delta_1$ for all $a$ satisfying $r(a) < r(\bar{a})$. \\
    Finally, since there exists a finite time $T_2$ such that $\theta(a) < -\delta_1$ for all $a$ satisfying $r(a) < r(\bar{a})$ and $\theta_{T_2}(a^*)$ is lower bounded by $\theta_{0}(a^*)$, we have that
    \begin{align}
        \theta_{T_2}(a^*) - \theta_{T_2}(a) \ge \theta_{0}(a^*) + \delta_1
    \end{align}
    for all $a$ satisfying $r(a) < r(\bar{a})$. Leading to the contradiction that $\pi_{\theta_t}^{\top} r \le r(\bar{a})$ for all $t$ while $\delta_1$ is large enough.
    
\end{itemize}

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lemma:stationary_point}
Given any $\delta > 0$, there exists a finite time
\begin{align}
    T = 
\end{align}
such that $\theta_t(a^*) - \theta_t(a_i) > \delta$ for all $t > T$.
\end{lemma}

\begin{proof}[Proof of \Cref{lemma:stationary_point}]  
\phantom{}
To show \Cref{lemma:stationary_point}, we leverage \Cref{prop:lower_bdd_gradient} and \Cref{corollary:Ghadimi_cor1} stated in \cite{ghadimi2016accelerated}.

By \Cref{corollary:Ghadimi_cor1} (\ref{eq:main_nocvx2}), there exists a finite time
\begin{align}
    N = \max \left \{ \left \lceil \frac{6 L_\Psi[\Psi(x_0) - \Psi^*]}{\inf_{t \ge 1, \pi_{\theta_t}^{\top} r \in [0, r(a_2)]} \left \| \frac{\partial \pi_{\theta_t}^{\top} r}{\partial \theta} \right \|^2} \right \rceil, \left \lceil \frac{6 L_\Psi[\Psi(x_0) - \Psi^*] \cdot [e^\delta + (n-1)]^2} {\min_{a \ne a^*} (r(a) - r(a^*))^2} \right \rceil \right \} + 1
\end{align}
such that
\begin{align}
\min\limits_{k=1,...,N} \|\nabla \Psi(x^{md}_k)\|^2
& \le \frac{6 L_\Psi[\Psi(x_0) - \Psi^*]}{N} \\
& < \min \left \{ \inf_{t \ge 1, \pi_{\theta_t}^{\top} r \in [0, r(a_2)]} \left \| \frac{\partial \pi_{\theta_t}^{\top} r}{\partial \theta} \right \|^2, \frac{\min_{a \ne a^*} (r(a) - r(a^*))^2}{[e^\delta + (n-1)]^2} \right \}
\end{align}
And by \Cref{prop:lower_bdd_gradient}, we could ensure that the minimum must occur at $\pi_\theta^{\top} r \in [r(a^*), r(a_2))$.

Moreover, by \mru{(ref?)}, we have:
\begin{align}
    \frac{\partial \pi_{\theta}^{\top} r}{\partial \theta(a)} = \pi_{\theta}(a) \cdot (r(a) - \pi_{\theta}^{\top} r)
\end{align}
holds for all $a \in \mathcal{A}$. Hence we have:
\begin{align}
    \frac{\min_{a \ne a^*} (r(a) - r(a^*))^2}{[e^\delta + (n-1)]^2}  > \left \| \nabla_{\theta} \pi_{\theta}^{\top} r \right \|^2 \ge  \pi_{\theta}(a)^2 \cdot (r(a) - \pi_{\theta}^{\top} r)^2
\end{align}
by rearranging the inequality above, we get:
\begin{align}
    \frac{1}{[e^\delta + (n-1)]^2} \ge \frac{\min_{a \ne a^*} (r(a) - r(a^*))^2}{(r(a) - \pi_{\theta}^{\top} r)^2}\cdot \frac{1}{[e^\delta + (n-1)]^2}  > \pi_{\theta}(a)^2
\end{align}
for all $a \ne a^*$.

And since $[e^\delta + (n-1)]^{-1} > \pi_{\theta_t}(a)$ for some $t \le N$, for all $a \ne a^*$, we have:
\begin{align}
    \frac{\pi_{\theta_t} (a^*)}{\pi_{\theta_t} (a)} > \frac{\frac{e^\delta}{e^\delta + (n-1)}}{\frac{1}{e^\delta + (n-1)}} = e^\delta
\end{align}
which is equivalent to our desired result:
\begin{align}
    \theta_t(a^*) - \theta_t(a) > \delta
\end{align}
for all $a \ne a^*$.

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}(Corollary 1(a) in \citep{ghadimi2016accelerated})
\label{corollary:Ghadimi_cor1}
Suppose that $\{\alpha_k\}$ and $\{\beta_k\}$ in the AG method are set to
\begin{align}
% \label{def_alpha_beta}
\alpha_k = \frac{2}{k+1} \ \ \ \mbox{and} \ \ \ \beta_k = \frac{1}{2 L_\Psi}.
\end{align}
% \begin{itemize}
% \item [a)] 
If $\{\lambda_k\}$ satisfies
\begin{align}
% \label{def_lambda}
\lambda_k \in \left[\beta_k,
\left(1+\frac{\alpha_k}{4}\right) \beta_k \right] \ \ \forall k \ge 1,
\end{align}
then for any $N\ge 1$, we have
\begin{align}
\min\limits_{k=1,...,N} \|\nabla \Psi(x^{md}_k)\|^2
\le \frac{6 L_\Psi[\Psi(x_0) - \Psi^*]}{N}.\label{eq:main_nocvx2}
\end{align}
% \item [b)]
% Assume that $\Psi(\cdot)$ is convex
% and that an optimal solution $x^*$ exists for problem NLP.
% If $\{\lambda_k\}$ satisfies
% \begin{align}
% % \label{def_lambda1}
% \lambda_k = \frac{ k \, \beta_k}{2} \ \ \forall k \ge 1,
% \end{align}
% then for any $N \ge 1$, we have
% \begin{align}
% \min\limits_{k=1,...,N} \|\nabla \Psi(x^{md}_k)\|^2 &\le&
% \frac{96 L_\Psi^2 \|x_0 - x^*\|^2}{N^2(N+1)}, \label{cvx_grad1}\\
% \Psi(x^{ag}_N)-\Psi(x^*) &\le& \frac{4 L_\Psi
% \|x_0 - x^*\|^2}{ N (N+1) }. \label{cvx_fun1}
% \end{align}
% \end{itemize}
\end{corollary}

\begin{remark} \mru{(Need to be revised)}
Since the gradient value contained $\pi(a \mid s)$ and $Adv(s,a)$ in each partial derivative to $\theta(s,a)$ \mru{(cite lemma?)}, we leverage \Cref{corollary:Ghadimi_cor1} to derive the explicit form for the time $T$ that makes the APG update approach a stationary point. Also note that the product of $\pi(a \mid s)$ and $Adv(s,a)$ must approaches $0$ at the stationary point, leading to the fact that at least one of them must converge to $0$.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\mru{TODO $($ Must have $\to$ Done $\to$ Good to have $)$:}
\begin{itemize}
    \item \mru{show $V^{\infty}$ exists, About limsup Adv}
    \item \mru{Could Ghadimi proof of APG hold for learning rate start from time $T$? Equation (2.32) in Accelerated Gradient Methods for Nonconvex Nonlinear and Stochastic Programming}
    \item \mru{equivalent argument from bandit 2 MDP.}
    \item \mru{We also have to argue it approach $\theta^*$ where $\theta^*$ is closed to $\infty.$ Also, we have to argue $\pi(a^{*}) \cdot r(a^{*})$ is the lower bdd of the objective.}
    \item \mru{[Done under bandit, MDP worse situation: argue finite time will achieve Q ordering fixed]} closed form of all finite time and $\delta$
    \item \mru{turn $r(a^*)$ into $Q(s, a^*)$ sounds good} difficulty of MDP? how to modified the objective concave function
    \item \mru{$\Omega(\frac{1}{t^2})$ (Good to have)}
\end{itemize}

\endgroup

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mru{Lemma, Thm, Prop, Proof Template}

\begin{prop}
\label{prop:TBD}
\mru{TBD}
\end{prop}

\begin{lemma}
\label{lemma:TBD}
\mru{TBD}
\end{lemma}

\begin{theorem}
\label{theorem:TBD}
\mru{TBD}
\end{theorem}

\begin{proof}[Proof of \Cref{theorem:bandit_convergence_rate}]  
\phantom{}
\mru{TBD}
\end{proof}
\newpage
\end{comment}

\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% good bad case proof
% \begin{lemma}
% \label{lemma:bandit_hard_ease_case}
% Given a finite time $T$ such that $r(a^*) > \pi_{\theta_{T}}^{\top} r > r(a_2)$, Consider the following two different update:
% \begin{itemize}
%     \item\label{bandit_hard_ease_case:case1} Case 1:
%     Update all parameters $\theta$ under \mru{APG (Update 1 / Algorithm 1)} with \mru{stepsize TBD}.
    
%     \item\label{bandit_hard_ease_case:case2} Case 2:
%     Only update the optimal action parameter $\theta_{a^*}$ while considering other parameters to be fixed under \mru{APG (Update 1 / Algorithm 1)} with \mru{stepsize TBD}.
% \end{itemize}
% Then we have:
% \begin{align}
% \underbrace{\left ( \pi^{*} - \pi_{\theta_{t}} \right )^{\top} r}_{\text{Case 1}} \le \underbrace{\left ( \pi^{*} - \pi_{\theta_{t}} \right )^{\top} r}_{\text{Case 2}} \text{, for all } t > T
% \end{align}
% where $\pi^{*}$ is the optimal policy.
% \end{lemma}

% % move this remark to 5-analysis.tex
% \begin{remark}
% \Cref{lemma:bandit_hard_ease_case} shows that the optimality gap under \mru{Case 1} is upper bounded by one under \mru{Case 2} and hence the convergence rate under \mru{Case 1} is lower bounded by one under \mru{Case 2}. This property is useful since the convergence rate of the latter case is easier to be constructed.
% \end{remark}

% \begin{proof}[Proof of \Cref{lemma:bandit_hard_ease_case}]  
% \phantom{}

% \mru{TBD}
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{prop}
% \label{prop:softmax_derivative}
% The partial derivative of the policy weight $\pi_{\theta}(a)$ is:
% \begin{align}
% \frac{\partial \pi_{\theta}(a)}{\partial \theta(a')} = 
% \begin{cases}
%  \pi_{\theta}(a) \cdot (1-\pi_{\theta}(a)) & \text{,if } a = a'\\
%  -\pi_{\theta}(a) \cdot \pi_{\theta}(a') & \text{,if } a \neq a'
% \end{cases}
% \end{align}
% \end{prop}

% \begin{proof}[Proof of \Cref{prop:softmax_derivative}]  
% \phantom{}
% By softmax parameterization, we have:
% \begin{align}
% \pi_{\theta}(a) &= \frac{\exp(\theta(a))}{\sum_{\tilde{a} \in \mathcal{A}} \exp(\theta(\tilde{a}))}
% \end{align}

% Hence, we have:
% \begin{align}
% \frac{\partial \pi_{\theta}(a)}{\partial \theta(a')}
% &= \frac{\frac{\partial \exp(\theta(a))}{\partial \theta(a')} \cdot \sum_{\tilde{a} \in \mathcal{A}} \exp(\theta(\tilde{a})) - \exp(\theta(a)) \cdot \frac{\partial \sum_{\tilde{a} \in \mathcal{A}} \exp(\theta(\tilde{a}))}{\partial \theta(a')}}{\left ( \sum_{\tilde{a} \in \mathcal{A}} \exp(\theta(\tilde{a})) \right )^2} \\
% &= \frac{ \mathbb{I} \left \{ a = a' \right \} \cdot \theta(a) \cdot \sum_{\tilde{a} \in \mathcal{A}} \exp(\theta(\tilde{a})) - \exp(\theta(a)) \cdot \exp(\theta(a'))}{\left ( \sum_{\tilde{a} \in \mathcal{A}} \exp(\theta(\tilde{a})) \right )^2} \\
% &= \mathbb{I} \left \{ a = a' \right \} \pi_{\theta}(a) - \pi_{\theta}(a) \cdot \pi_{\theta}(a')
% \end{align}

% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{prop}
% \label{prop:finite_time_concave}
% Given $r(a^*) > \pi_{\theta_{T}}^{\top} r > r(a_2)$ where $\theta_T$ is the policy parameters at time $T$, consider the \mru{Case 2} update we've stated in \Cref{lemma:bandit_hard_ease_case}
% Then there exists a finite time
% \begin{align}
% T_1 = TBD
% \end{align}
% such that $\pi_{\theta_{t}(a^{*})}(a^{*}) \ge \frac{1}{2}$ for all $t > T_1 $.
% \end{prop}

% \begin{proof}[Proof of \Cref{prop:finite_time_concave}]  
% \phantom{}
% \mru{TBD, concept: since gradient must be positive and momentum must be bounded, there exists a finite time such that momentum is positive, and hence we can accumulate the momentum improvement since it will approach infty}

% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}
% \label{lemma:bandit_sigmoid_concave}
% \mru{TBD}
% Given $r(a^*) > \pi_{\theta_{T}}^{\top} r > r(a_2)$ where $\theta_T$ is the policy parameters at time $T$, consider the \mru{Case 2} update we've stated in \Cref{lemma:bandit_hard_ease_case}
% Then after a finite time $T_1$, we have:
% \begin{align}
% \left ( \pi^{*} - \pi_{\theta_{t}} \right )^{\top} r = O(\frac{1}{t^2}) \quad \text{ , for all } t > T_1 
% \end{align}
% where $\pi^{*}$ is the optimal policy.
% \end{lemma}

% \begin{proof}[Proof of \Cref{lemma:bandit_sigmoid_concave}]  
% \phantom{}

% By \mru{Case 2},the policy parameters $\theta_{t}(a_i)$ is fixed for $i = 2, 3, \cdots, n$, so $\theta_{t}(a_i) = \theta_{0}(a_i)$ for all $t > T$, and hence the objective $\pi_{\theta_{t}}^{\top} r$ will be parameterized by a single parameter $\theta_t(a^{*})$:
% \begin{align}
% \pi_{\theta_{t}(a^{*})}^{\top} r
% &= \sum_{a \in \mathcal{A}} \pi_{\theta_{t}(a^{*})}(a) \cdot r(a) \\
% &= \frac{\exp(\theta_t(a^{*}))}{\exp(\theta_t(a^*))+ \sum_{j=1}^{n} \exp(\theta_0(a_j))} \cdot r(a^{*}) \\ 
% &\quad + \sum_{i=2}^{n} \frac{\exp(\theta_0(a_i))}{\exp(\theta_t(a^*)) + \sum_{j=1}^{n} \exp(\theta_0(a_j))} \cdot r(a_i)
% \end{align}

% So, we can easily compute the second derivative of our objective:
% \begin{align}
% \frac{\mathrm{d}^2}{\mathrm{d} \theta_{t}(a^{*})^2} \pi_{\theta_{t}(a^{*})}^{\top} r &= 
% \frac{\mathrm{d}}{\mathrm{d} \theta_{t}(a^{*})} \left ( \frac{\mathrm{d}}{\mathrm{d} \theta_{t}(a^{*})} \pi_{\theta_{t}(a^{*})}^{\top} r \right ) \\
% &= \frac{\mathrm{d}}{\mathrm{d} \theta_{t}(a^{*})} \left( \frac{\mathrm{d}}{\mathrm{d} \theta_{t}(a^{*})} \sum_{a \in \mathcal{A}} \pi_{\theta_{t}(a^{*})}(a) \cdot r(a) \right) \\
% &= \frac{\mathrm{d}}{\mathrm{d} \theta_{t}(a^{*})} \left( \pi_{\theta_{t}(a^{*})}(a^{*}) \cdot r(a^{*}) - \pi_{\theta_{t}(a^{*})}(a^{*}) \cdot \sum_{a \in \mathcal{A}} \pi_{\theta_{t}(a^{*})}(a) \cdot r(a) \right) \\
% &= \frac{\mathrm{d}}{\mathrm{d} \theta_{t}(a^{*})} \left ( \pi_{\theta_{t}(a^{*})}(a^{*}) \cdot \left ( r(a^{*}) - \pi_{\theta_{t}(a^{*})}^{\top} r \right) \right) \\
% &= \pi_{\theta_{t}(a^{*})}(a^{*}) \cdot (1 - \pi_{\theta_{t}(a^{*})}(a^{*})) \cdot \left ( r(a^{*}) - \pi_{\theta_{t}(a^{*})}^{\top} r \right ) \\
% & \quad - \pi_{\theta_{t}(a^{*})}(a^{*}) \cdot \pi_{\theta_{t}(a^{*})}(a^{*}) \cdot \left ( r(a^{*}) - \pi_{\theta_{t}(a^{*})}^{\top} r \right) \\
% &= \pi_{\theta_{t}(a^{*})}(a^{*}) \cdot (1 - 2\pi_{\theta_{t}(a^{*})}(a^{*})) \cdot \left ( r(a^{*}) - \pi_{\theta_{t}(a^{*})}^{\top} r \right ) \label{eq:hessian} \\
% & \le 0 \quad \text{ , for all } \pi_{\theta_{t}(a^{*})}(a^{*}) \ge \frac{1}{2} \label{eq:concanve_condition}
% \end{align}

% The third and fifth equation holds by \Cref{prop:softmax_derivative}.\\
% The last inequality holds since $\pi_{\theta_{t}(a^{*})}(a^{*})$ and $\left ( r(a^{*}) - \pi_{\theta_{t}(a^{*})}^{\top} r \right )$ in \ref{eq:hessian} is non-negative.

% From \ref{eq:concanve_condition}, we show that the objective will be concave once $\pi_{\theta_{t}(a^{*})}(a^{*}) \ge \frac{1}{2}$ holds. And by \Cref{prop:finite_time_concave}, there exists a finite time $T_1$ such that $\pi_{\theta_{t}(a^{*})}(a^{*}) \ge \frac{1}{2}$ for all $t > T_1$. Finally, by \mru{Nesterov convergence rate}, the desired result holds.

% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{prop}
% \label{prop:global_min_imply_local_convexity}
% The objective $\pi_{\theta}^{\top} r$ enjoys local convexity at the optimal policy parameters $\theta^{*}$. Moreover, there exists $\tilde{\theta}$ such that the objective $\pi_{\theta}^{\top} r$ is convex for all $\theta_{a^{*}} > \tilde{\theta}$ and \mru{TBD}.
% \end{prop}

% \begin{proof}[Proof of \Cref{prop:global_min_imply_local_convexity}]  
% \phantom{}

% Proof Sketch:
% \begin{enumerate}
%     \item \mru{(Show)} Since $\pi_{\theta_{t}}^{\top} r \to \pi_{\theta^{*}}^{\top} r$ while $\pi_{\theta_{t}}(a^{*}) \to 1$, we have that the objective is locally concave in $\pi_{\theta_{t}}(a^{*}) \in \left[ 1-\epsilon, 1 \right]$ for some $\epsilon > 0$ and hence it is locally concave in $\theta_t(a^{*}) > \epsilon_1$ for some $\epsilon_1$.
%     \item \mru{(Show)} $\theta \to \pi_{\theta}$ is concave for $\theta_{a^{*}} > \epsilon_2$ for some $\epsilon_2$. \mru{Maybe we need some constraints on other $\theta$s.}
%     \item By \mru{Lemma in Stephen Boyd's textbook, P.86}, we have $\pi_{\theta}^{\top} r$ is concave while $\theta_{a^{*}} > \max \left\{ \epsilon_1, \epsilon_2 \right\}$ and $\theta_{a_i} \cdots$ \mru{TBD}.
    
% \end{enumerate}

% TBD

% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

\endgroup

==> app/backup-11-add-adaptive-apg.tex <==
\newpage
\section{APG With Exponentially-Growing Step Sizes}
\label{app:add-adaptive-apg}

\begingroup
\allowdisplaybreaks

%\subsection{Asymptotic Convergence of APG With Exponentially-Growing Step Sizes}
%\begin{theorem}
%    [\textbf{Asymptotic convergence under softmax parameterization}]
%    \label{theorem:global_convergence_adaptive_apg}
%    \mru{Consider a tabular softmax parameterized policy $\pi_{\theta}$. Under \hyperref[algorithm:APG]{APG} with modifying \cref{algorithm:eq1} by 
%    \begin{align*}
%        \theta^{(t)} &\leftarrow \omega^{(t-1)} + \Big[ \eta^{(t)} \nabla_{\theta}{V^{\pi_{\theta}}(\mu)} \Big\rvert_{\theta = \omega^{(t-1)}} \Big]^{+K},
%    \end{align*}
%    where $\eta^{(t)} = \beta^t \cdot \frac{(1-\gamma)^3}{8}$ for any $\beta > 1$, $\mu$ initialized uniformly at random, and $K > \ln2 + 2\ln\beta$, 
%    we have $V^{\pi_{\theta}^{(t)}}(s) \rightarrow V^{*}(s)$ as $t\rightarrow \infty$, for all $s\in\cS$.}
%\end{theorem}
%\cpcomment{It looks like in \Cref{lemma:max Is0} we actually need the
%stepsizes to be upper bounded.
%Please double check this issue.
%If indeed that condition is needed, then asymptotic convergence
%doesn't hold as claimed here for exponentially-growing stepsizes.}
%\begin{proof}[Proof of \Cref{theorem:global_convergence_adaptive_apg}]
%Using the similar arguments of \Cref{theorem:convergeoptimal} and \Cref{lemma: convergence to stationarity}-\ref{lemma:compare pi(a+) and pi(a-)}, we have
%the results. 
%Please note that after clipping, it is invalid to apply \Cref{lemma:sum conservation} in \Cref{lemma:Is- negative infinity} anymore, but it could be relaxed by showing that $\sum_{a \in \cA} \theta_{s,a}^{(t)} \le \sum_{a \in \cA} \theta_{s,a}^{(0)}$ for all $t \ge 0$, $s \in \cS$, and $a \in \cA$.
% 
%% Upon meticulous examination, it becomes apparent that the
%% step sizes $\eta^{(t)}$ can be modified to $\beta^{t} \cdot
%% \frac{(1-\gamma^3)}{8}$ while retaining the validity of all the proofs
%% in \Cref{lemma: convergence to stationarity}-\ref{lemma:compare pi(a+)
%% and pi(a-)}.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence Rate of APG With Exponentially-Growing Step Sizes}

%\begin{restatable}{lemma}{stationarylemma2}
%\label{lemma: adaptive apg enter local concavity}
%    Consider a tabular softmax parameterized policy $\pi_{\theta}$. Under \hyperref[algorithm:APG]{APG} {$\eta^{(t)} = \beta^t \cdot \frac{(1-\gamma^3)}{8}$ for any $\beta > 1$}, given any $M > 0$, there exists a finite time T such that for all $t \ge T$, $s\in\cS$, and $a \neq a^*(s)$, we have, (i) $\theta_{s, a^*(s)} - \theta_{s, a} > M$, (ii) $V^{\pi_{\theta}^{(t)}}(s) > Q^*(s, a_2(s))$, (iii) $\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s, a^*(s)}}\right\rvert_{\theta = \omega^{(t)}} > 0 > \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s, a}}\right\rvert_{\theta = \omega^{(t)}}$, (iv) $\omega_{s, a^*(s)}^{(t)} - \theta_{s, a^*(s)}^{(t)} \ge \omega_{s, a}^{(t)} - \theta_{s, a}^{(t)}$.
%\end{restatable}
%\begin{proof}[Proof of \Cref{lemma: adaptive apg enter local concavity}]
%Using the similar arguments of \Cref{lemma: enter local concavity}, we have the results.
%\end{proof}

% \begin{theorem}[\textbf{Convergence Rate of APG with adaptive learning rate}]
% \label{theorem: adaptive apg convergence rate}
%     Consider a tabular softmax parameterized policy $\pi_{\theta}$. Under \hyperref[algorithm:APG]{APG} with {$\eta^{(t)} = \beta^t \cdot \frac{(1-\gamma)^3}{8}$ for any $\beta > 1$}, there exists a finite time $T$ such that for all $t \ge T$, we have
%     \begin{align}
%         V^{*}(\rho) - V^{{\pi_\theta^{(t)}}}(\rho) = O(e^{-ct}),
%     \end{align}
%     for some constant $c > 0$.
% \end{theorem}
\adaptiveapg*
\begin{proof}[Proof of \Cref{theorem: adaptive apg convergence rate}]

By \Cref{lemma:perf_diff}, we have
\begin{align*}
    V^{*}(\mu) - V^{\pi_{\theta}^{(t)}}(\mu) &= \frac{1}{1 - \gamma} \sum_{s, a} d_{\mu}^{\pi^*}(s) \pi^*(a|s) A^{\pi_{\theta}^{(t)}}(s, a) \\
    &= \frac{1}{1 - \gamma} \sum_{s, a} d_{\mu}^{\pi^*}(s) (\pi^*(a|s) - \pi_{\theta}^{(t)}(a|s)) A^{\pi_{\theta}^{(t)}}(s, a) \\
    &\le \frac{1}{1 - \gamma} \sum_{s, a} \Bigg | d_{\mu}^{\pi^*}(s) (\pi^*(a|s) - \pi_{\theta}^{(t)}(a|s)) A^{\pi_{\theta}^{(t)}}(s, a) \Bigg | \\
    &\le \frac{2}{(1 - \gamma)^2} \left\lVert {d_{\mu}^{\pi^*}} \right\rVert_{\infty} \sum_{s, a} \Bigg | \pi^*(a|s) - \pi_{\theta}^{(t)}(a|s) \Bigg | \\
    &= \frac{2}{(1 - \gamma)^2} \left\lVert {d_{\mu}^{\pi^*}} \right\rVert_{\infty} \sum_{s} \Bigg( \Bigg | \pi^*(a^*|s) - \pi_{\theta}^{(t)}(a^*|s) \Bigg | + \sum_{a \neq a^*} \Bigg | \pi^*(a|s) - \pi_{\theta}^{(t)}(a|s) \Bigg | \Bigg) \\ 
    &= \frac{2}{(1 - \gamma)^2} \left\lVert {d_{\mu}^{\pi^*}} \right\rVert_{\infty} \sum_{s} 2(1-\pi_\theta^{(t)}(a^*|s)).
\end{align*}

To obtain the desired outcome, it is sufficient to show that there
exist $\bar{c}, \tilde{c} > 0$ such that
$1 - \pi_{\theta}^{(t)}(a^*(s) | s) \le \tilde{c} e^{-\bar{c}t}$ for
all $s \in \cS$ and all $t \ge T$.
We prove this result by contradiction.
Selecting $T$ from \Cref{lemma: enter local concavity}, we assume that after time-step $T$, there exists one state $s'$ and an infinite time sequence $\{ t_i\}_{i=1}^{\infty}$ such that for any $\bar{c}, \tilde{c} > 0$, we have $1 - \pi_{\theta}^{(t)}(a^*(s') | s') > \tilde{c} e^{-\bar{c}t}$ for all $t \in \{ t_i\}_{i=1}^{\infty}$. 

Define:
\begin{align*}
    C \coloneqq \inf_{t \ge T} \Big\{ \frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*(s')|s') \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))) \Big\},
\end{align*}
then we have $C > 0$ since $d^{\pi_\omega^{(t)}}_{\mu}(s') \ge (1-\gamma)\mu(s')$ by \Cref{lemma:lower_bound_of_state_visitation_distribution}, $\pi_\omega^{(t)}(a^*(s')|s') > \frac{1}{|\cA|}$ since $\theta_{s', a^*(s')} > \theta_{s', a}$ for all $a \neq a^*(s')$ by property (i) of \Cref{lemma: enter local concavity}, and $Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) \ge V^{\pi_\theta^{(t)}}(s') > Q^{*}(s', a^*(s'))) > \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))$ by properties (ii) of \Cref{lemma: enter local concavity} and \Cref{lemma: Q^* a_2}.

By choosing $\tilde{c} = \frac{K}{C}$ and $\bar{c} = \beta$, we have:
\begin{align}
    A^{\pi_{\theta}^{(t)}}(s', a^*(s'))
    &= Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - V^{\pi_{\theta}^{(t)}}(s') \nonumber \\
    &= Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \sum_{a \in \cA} \pi_{\theta}^{(t)}(a(s')|s') Q^{\pi_{\theta}^{(t)}}(s', a) \nonumber \\
    &= (1-\pi_{\theta}^{(t)}(a^*(s')|s')) Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \sum_{a \neq a^*(s')} \pi_{\theta}^{(t)}(a|s') {Q^{\pi_{\theta}^{(t)}}(s', a)} \nonumber \\
    &\ge (1-\pi_{\theta}^{(t)}(a^*(s')|s')) Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \sum_{a \neq a^*(s')} \pi_{\theta}^{(t)}(a|s') \cdot \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a) \nonumber \\
    &= (1-\pi_{\theta}^{(t)}(a^*(s')|s')) Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - (1-\pi_{\theta}^{(t)}(a^*|s')) \cdot \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a) \nonumber \\
    &= (1-\pi_{\theta}^{(t)}(a^*(s')|s')) \underbrace{(Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a))}_{\text{bounded away from 0}} \nonumber \\
    &> \frac{K}{C\beta^t} \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a)). \label{eq:adaptive_apg_2}
\end{align}

% But the policy parameter $\theta_{s', a^*(s')}$ follows that
By following (\ref{eq:adaptive_apg_2}), for all $t \in \{ t_i\}_{i=1}^{\infty}$, we have
\begin{align}
    &\theta_{s', a^*(s')}^{(t+1)} - \theta_{s', a^*(s')}^{(t)} \nonumber \\
    &= \underbrace{(\theta_{s', a^*(s')}^{(t+1)} - \omega_{s', a^*(s')}^{(t)})}_{\text{gradient}} + \underbrace{(\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)})}_{\text{momentum}} \nonumber \\
    &= \min \Big\{K, \eta^{(t)} \nabla_{\theta}{V^{\pi_{\theta}}(\mu)} \Big\rvert_{\theta = \omega^{(t)}} \Big\} + (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)}) \nonumber \\
    &= \min \Big\{K, \eta^{(t)} \cdot \frac{1}{1-\gamma} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}({a^*}|s') \cdot A^{\pi_\omega^{(t)}}(s',{a^*}) \Big\} + (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)}) \nonumber \\
    &\ge K + \max_{a \neq a^*(s')} \Big\{ \omega_{s', a}^{(t)} - \theta_{s', a}^{(t)} \Big\} \label{eq:adaptive_apg_3},
    % &> \min \Big\{ K, \beta^t \cdot \frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*|s') \cdot e^{-\bar{c}t} \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))) \Big\} \nonumber \\
    % &= \min \Big\{ K, \big(\underbrace{\frac{\beta}{\beta_0}}_{>1}\big)^t \cdot \underbrace{\frac{(1-\gamma)^3}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*|s') \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s')))}_{\text{bounded away from 0}} \Big\}, \label{eq:adaptive_apg_3} 
\end{align}
where \cref{eq:adaptive_apg_3} holds by \Cref{lemma: enter local concavity} and the fact that
\begin{align*}
    &\eta^{(t)} \cdot \frac{1}{1-\gamma} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}({a^*}|s') \cdot A^{\pi_\omega^{(t)}}(s',{a^*}) \\
    &> \beta^t \cdot \frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*|s') \cdot \frac{K}{C\beta^t} \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s'))) \\
    &= \frac{\frac{(1-\gamma)^2}{8} \cdot d^{\pi_\omega^{(t)}}_{\mu}(s') \cdot \pi_\omega^{(t)}(a^*(s')|s') \cdot (Q^{\pi_{\theta}^{(t)}}(s', a^*(s')) - \max_{a \neq {a^*(s')}} Q^{\pi_{\theta}^{(t)}}(s', a^*(s')))}{C} \cdot K \\
    &\ge K.
\end{align*}

Now we discuss two possible cases:
\begin{itemize}
    \item The infinite time sequences $\{ t_i\}_{i=1}^{\infty}$ contains all $t > T$. (i.e., $\{ t_i\}_{i=1}^{\infty} = \{ T+1, T+2, T+3, \cdots \}$): \\
    In this case, by \cref{eq:adaptive_apg_3} and \Cref{lemma: enter local concavity}, we have that
    \begin{align*}
        \theta_{s', a^*(s')}^{(t+1)} - \theta_{s', a^*(s')}^{(t)} 
        &\ge K + \max_{a \neq a^*(s')} \Big\{ \omega_{s', a}^{(t)} - \theta_{s', a}^{(t)} \Big\} \\
        &> K + \max_{a \neq a^*(s')} \Big\{ \underbrace{(\theta_{s', a}^{(t+1)} - \omega_{s', a}^{(t)})}_{\text{gradient} < 0} \Big\} + \max_{a \neq a^*(s')} \Big\{ \underbrace{(\omega_{s', a}^{(t)} - \theta_{s', a}^{(t)})}_{\text{momentum}} \Big\} \\
        &\ge K + \max_{a \neq a^*(s')} \Big\{ \theta_{s', a}^{(t+1)} - \theta_{s', a}^{(t)} \Big\}
    \end{align*}
    This indicates a constant growth of the policy parameter $\theta_{s' ,a^*(s')}$. Consequently, by softmax parameterization, it follows that $1 - \pi_\theta^{(t)}(a^* | s') = O(e^{-\bar{c}t})$ for some $\bar{c} > 0$, thereby completing our contradiction.

    \item There exists at least one $(t_i-1) > T$ such that $(t_i-1) \notin \{ t_i\}_{i=1}^{\infty}$ (i.e., $1 - \pi_{\theta}^{(t_i-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t_i-1}}$):\\
    In this case, we set $K > \ln2 + 2\ln\beta$ to ensure that the one step improvement $\pi_{\theta}^{(t_i+1)}(a^*(s) | s') - \pi_{\theta}^{(t_i)}(a^*(s) | s')$ is sufficiently large once we follow the update $\theta_{s', a^*(s')}^{(t_i+1)} = \omega_{s', a^*(s')}^{(t_i)} + K$. \\
    By \Cref{lemma: enter local concavity}, we have:
    \begin{align}
        &\pi_{\theta}^{(t+1)}(a^*(s) | s') \nonumber \\
        &= \frac{\exp(\theta_{s', a^*(s')}^{(t+1)})}{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t+1)})} \nonumber \\
        &= \frac{\exp(\theta_{s', a^*(s')}^{(t)} + (\theta_{s', a^*(s')}^{(t+1)} - \omega_{s', a^*(s')}^{(t)}) + (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)}))}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t)} + (\theta_{s', a}^{(t+1)} - \omega_{s', a}^{(t)}) + (\omega_{s', a}^{(t)} - \theta_{s', a}^{(t)}))} \nonumber \\
        &= \frac{\exp(\theta_{s', a^*(s')}^{(t)})}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t)} + \underbrace{(\theta_{s', a}^{(t+1)} - \omega_{s', a}^{(t)}) + (\omega_{s', a}^{(t)} - \theta_{s', a}^{(t)}) - (\theta_{s', a^*(s')}^{(t+1)} - \omega_{s', a^*(s')}^{(t)}) - (\omega_{s', a^*(s')}^{(t)} - \theta_{s', a^*(s')}^{(t)})}_{\le 0})} \nonumber \\
        &\ge \frac{\exp(\theta_{s', a^*(s')}^{(t)})}{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t)})} \nonumber \\
        &= \pi_{\theta}^{(t)}(a^*(s) | s'). \label{eq:adaptive_apg_3-1}
    \end{align}
    Following \cref{eq:adaptive_apg_3-1}, since $\pi_{\theta}^{(t)}(a^*(s) | s')$ is increasing for all $t > T$, we have
    \begin{align}
        \sum_{a \neq a^*(s')} \pi_{\theta}^{(t_i)}(a| s') = 1 - \pi_{\theta}^{(t_i)}(a^*(s) | s') < 1 - \pi_{\theta}^{(t_i-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t_i-1}}.
        \label{eq:adaptive_apg_4}
    \end{align}
    Moreover, by \Cref{lemma: enter local concavity}, we have 
    \begin{align}
        \frac{\sum_{a \neq a^*(s')} \exp (\theta_{s', a}^{(t_i)})}{2 \exp (\theta_{s', a^*(s')}^{(t_i)})} \le \sum_{a \neq a^*(s')} \pi_{\theta}^{(t_i)}(a| s') \le \frac{K}{C \beta^{t_i-1}}. \label{eq:adaptive_apg_5}
    \end{align}
    Combining \cref{eq:adaptive_apg_3,eq:adaptive_apg_4,eq:adaptive_apg_5}, we get
    \begin{align}
        1 - \pi_{\theta}^{(t_i+1)}(a^*(s) | s')
        &= \sum_{a \neq a^*(s')} \pi_{\theta}^{(t_i+1)}(a| s') \nonumber\\
        &= \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \theta_{s', a}^{(t_i)}))}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \theta_{s', a}^{(t_i)}))} \nonumber\\
        &= \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)} + \overbrace{(\theta_{s', a}^{(t_i+1)} - \omega_{s', a}^{(t_i)})}^{<0} + \overbrace{(\omega_{s', a}^{(t_i)} - \theta_{s', a}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)})}^{\le0})}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \omega_{s', a}^{(t_i)}) + (\omega_{s', a}^{(t_i)} - \theta_{s', a}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        % &\le \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)})}{\sum_{a \in \cA} \exp(\theta_{s', a}^{(t_i)} + (\theta_{s', a}^{(t_i+1)} - \omega_{s', a}^{(t_i)}) + (\omega_{s', a}^{(t_i)} - \theta_{s', a}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        &\le \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)})}{\exp(\theta_{s', a^*(s')}^{(t_i)} + (\theta_{s', a^*(s')}^{(t_i+1)} - \omega_{s', a}^{(t_i)}) + (\omega_{s', a^*(s')}^{(t_i)} - \theta_{a^*(s')}^{(t_i)}) - (\omega_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        &\le \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)}))}{ \exp(\theta_{s', a^*(s')}^{(t_i)} + (\theta_{s', a^*(s')}^{(t_i+1)} - \omega_{s', a^*(s')}^{(t_i)}))} \nonumber\\ 
        &= \frac{\sum_{a \neq a^*(s')} \exp(\theta_{s', a}^{(t_i)})}{ \exp(\theta_{s', a^*(s')}^{(t_i)})} \cdot \exp(-K) \nonumber\\
        &\le \frac{2K}{C \beta^{t_i-1}} \cdot \exp(-K) \nonumber\\
        &\le \frac{K}{C \beta^{t_i+1}}. \label{eq:adaptive_apg_6},
    \end{align}
    where \cref{eq:adaptive_apg_6} holds by setting $K > \ln2 + 2\ln\beta$.
    
    Hence we get that once $1 - \pi_{\theta}^{(t)}(a^*(s) | s') > \frac{K}{C \beta^{t}}$ occurs for any $t \in \{ t_i\}_{i=1}^{\infty}$, we could ensure that $1 - \pi_{\theta}^{(t+1)}(a^*(s) | s') \le \frac{K}{C \beta^{t+1}}$ (i.e., $(t_i+1) \notin \{ t_i\}_{i=1}^{\infty}$ for all $t_i \in  \{ t_i\}_{i=1}^{\infty}$),
    In other words, for all $t \in  \{ t_i\}_{i=1}^{\infty}$, we have $t-1 \notin  \{ t_i\}_{i=1}^{\infty}$ and hence $1 - \pi_{\theta}^{(t-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t-1}}$.
    Combining with the monotonicity of $1 -\pi_{\theta}^{(t-1)}(a^*(s) | s')$ in \cref{eq:adaptive_apg_3-1}, we get $1 -\pi_{\theta}^{(t)}(a^*(s) | s') \le 1 -\pi_{\theta}^{(t-1)}(a^*(s) | s') \le \frac{K}{C \beta^{t-1}}$.
    Finally, we could conclude that $1 - \pi_{\theta}^{(t)}(a^*(s) |
	s') \le \frac{K}{C \beta^{t-1}}$ for all $t > T$, which also
	complete our contradiction.\qedhere
\end{itemize}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This indicates a constant growth of the policy parameter $\theta_{s ,a^*}$. Consequently, it follows that $1 - \pi_\theta^{(t)}(a^* | s') = O(e^{-\bar{c}t})$ for some $\bar{c} > 0$, thereby completing our contradiction.

% Following \cref{eq:adaptive_apg_3}, we then show that $1 - \pi_{\theta}^{(t)}(a^* | s') \le \big(\frac{1}{
% \beta_0
% }\big)^{t-1}$ for all large enough $t \in \{ t_i\}_{i=1}^{\infty}$ by contradiction. Assume $1 - \pi_{\theta}^{(t_i-1)}(a^* | s') > \big(\frac{1}{
% \beta_0
% }\big)^{t_i-1}$ for some $i \in \mathbb{N}_+$, then we have
% \begin{align*}
%     &\theta_{s', a^*(s')}^{(t_i)} \\
%     &= \theta_{s', a^*(s')}^{(t_i-1)} + (\theta_{s', a^*(s')}^{(t_i)} - \theta_{s', a^*(s')}^{(t_i-1)}) \\
%     &> \underbrace{\theta_{s', a^*(s')}^{(t_i-1)}}_{\text{bounded below}} + \underbrace{\big(\frac{\beta}{\beta_0}\big)^{t_i-1}}_{\rightarrow \infty \text{, exponentially}} \cdot \underbrace{\frac{(1-\gamma)^3}{8} \cdot d^{\pi_\omega^{(t_i-1)}}_{\mu}(s') \cdot \pi_\omega^{(t_i-1)}(a^*|s') \cdot (Q^{\pi_{\theta}^{(t_i-1)}}(s', a^*(s')) - \max_{a \neq {a^*}} Q^{\pi_{\theta}^{(t_i-1)}}(s', a^*(s')))}_{\text{bounded away from 0}} \\
%     &\ge \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} + \ln (2|\cA|) + t \ln \beta_0.
% \end{align*}
% And so we have
% \begin{align}
%     &1- \pi_\theta^{(t_i)} \\ 
%     &= 1 - \frac{\exp (\theta_{s', a^*(s')}^{(t_i)})}{\exp (\theta_{s', a^*(s')}^{(t_i)}) + \sum_{a \neq a^*(s')} \exp (\theta_{s', a}^{(t_i)})} \\
%     & = 1 - \frac{\exp (\theta_{s', a^*(s')}^{(t_i)} - \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} - \ln (2|\cA|))}{\exp (\theta_{s', a^*(s')}^{(t_i)} - \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} - \ln (2|\cA|)) + \sum_{a \neq a^*(s')} \exp (\theta_{s', a}^{(t_i)} - \max_{t \le T, a \neq a^*(s')} \{ \theta^{(t)}_{s', a} \} - \ln (2|\cA|))} \\
%     &\le 1 - \frac{\exp (t_i \ln \beta_0)}{\exp (t_i \ln \beta_0) + (|\cA|-1) \exp(-\ln (2|\cA|))} \\
%     &\le 1 - \frac{\exp (t_i\ln \beta_0)}{\exp (t_i\ln \beta_0) + 1/2} \\
%     &\le 1 - \frac{\beta_0^{t_i}}{\beta_0^{t_i} + \frac{\beta_0^{t_i}}{\beta_0^{t_i}-1}} \\
%     &= \big(\frac{1}{\beta_0}\big)^{t_i},
% \end{align}
% which contradict to $1 - \pi_{\theta}^{(t)}(a^* | s') > \big(\frac{1}{\beta_0}\big)^t$ for all $t \in \{ t_i\}_{i=1}^{\infty}$.

% Combining with the fact that $1 - \pi_{\theta}^{(t)}(a^* | s')$ is non-increasing, we have $1 - \pi_{\theta}^{(t)}(a^* | s') \le \big(\frac{1}{\beta_0}\big)^{t-1}$ for all large enough $t \in \mathbb{N}$ and hence we complete the proof.
%
\end{proof}


% \newpage
% \subsection{Table to put at introduction}
% \begin{table}[!ht]
% \color{blue}
% \caption{Convergence Rates with Exact Gradients for the Tabular Case}
% \label{table:rate}
% \vskip 0.11in
% \begin{center}
%     \begin{small}
%     \begin{sc}
%         \begin{tabular}{cccc}
%         \toprule
%                    & \textbf{APG (Ours)}               & NPG          & GNPG         \\
%         \midrule
%         Constant step sizes & \boldsymbol{$\tilde{O}({1} / {t^2})$} (\Cref{theorem: MDP convergence rate}) & $O({1} / {t})$ \citep{agarwal2021theory, xiao2022convergence} & N/A          \\
%         Adaptive step sizes & \boldsymbol{$O(e^{-ct})$} (\Cref{theorem: adaptive apg convergence rate})             & $O(e^{-ct})$ \citeauthor{khodadadian2021linear, xiao2022convergence}& $O(e^{-ct})$ \citep{mei2021leveraging} \\
%         \bottomrule
% \end{tabular}
%     \end{sc}
%     \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

\subsection{Numerical Validation of the Linear Convergence Rate}
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
  % \vspace{-\intextsep}
  % \vspace{-\intextsep}
  \includegraphics[width=0.35\textwidth]{img_icml/adaptive-apg.png}
  \hspace{-5mm}
  \caption{The sub-optimality gap of APG with exponentially-growing
  step sizes under an MDP of five states and five actions with uniform initialization.}
  % \vspace{-\intextsep}
  \label{exp:adaptiveapg}
\end{wrapfigure}

In this subsection, we empirically validate the convergence rate of
APG with an exponentially-growing step size scheduling by conducting
experiments on an MDP with five states and five actions. This MDP is identical to the one discussed in \Cref{sec:disc:exp}, and detailed configuration information is provided in \Cref{app:experiment}.
The figure illustrating the logarithmic sub-optimality gap of APG with
an exponentially-growing step size shceduling aaunder uniform
initialization is presented in \Cref{exp:adaptiveapg}.
It is evident that after ten iterations, the curve tends to form a
linear pattern.
This behavior aligns with the linear convergence rate demonstrated in \Cref{theorem: adaptive apg convergence rate}.

\endgroup


==> app/backup-3-asym.tex <==
\newpage
\section{Asymptotic Convergence}
\label{app:asym_conv}

% For ease of exposition, we restate the bandit case setting as follows:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Bandit Case.}
% A bandit case is a special case of the reinforcement learning problem in which there is only one single state. Given a bandit case with $|\mathcal{A}|$ actions $\left[ a^*, a_2, \cdots, a_{|\mathcal{A}|} \right]$ and rewards $r = \left[ r(a^*), r(a_2), \cdots, r(a_{|\mathcal{A}|}) \right]$.
% We parametrized the policy under softmax, (i.e. we define $\pi_{\theta} = \text{softmax}(\theta)$ where $\theta = [\theta_{a^*}, \theta_{a_2}, \cdots, \theta_{a_{|\mathcal{A}|}}]$.
% Without loss of generality and for simplicity, we assume that the optimal action $a^*$ is unique and $r(a^*) > r(a_2) > \cdots > r(a_{|\mathcal{A}|})$. The uniqueness assumption can be lifted with a little extra work.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Supporting Lemmas for Asymptotic Convergence of APG}
\label{app:asym_conv:lemmas}

%In this subsection, we assume that the step sizes $\eta^{(t)}$ are both lower and upper bounded. We will set $\eta^{(t)} = \frac{t}{t+1} \cdot \frac{(1-\gamma)^3}{16}$ in the subsequent \Cref{theorem:convergeoptimal} in \Cref{app:asym_conv:all}, which is a lower and upper bounded configuration. Moreover, we consider the case that the initial momentum $m^{(1)} = \bm{0}$.}

%\begin{assumption}
%    $\big\lVert \nabla_\theta V^{\pi_\theta}(\mu) \big\rVert =0 $ only if $\pi_\theta$ is deterministic.
%\end{assumption}
\begin{lemma}
\label{lemma: convergence to stationarity}
Under APG for softmax parameterzation with any surrogate initial state
distribution $\mu$,
%\cpfn{Now we don't
%	have $m^{(1)}$, please update this part \updatecomment{update to $m_{\text{init}}$.}}
as long as there is $\eta > 0$ such that $\eta^{(t)} \geq \eta$ for
all $t$,
the limits of both $V^{\pi_{\omega}^{(t)}}(\mu)$
and $V^{\pi_{\theta}^{(t)}}(\mu)$ when $t$ approaches infinity exist, and 
$\lim_{t\rightarrow \infty} V^{\pi_{\omega}^{(t)}}(\mu) =\lim_{t\rightarrow \infty} V^{\pi_{\theta}^{(t)}}(\mu)$.
Moreover, for every state $s\in \cS$,
\begin{align*}
   &\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega_t} \big\rVert =0,\\
   &\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\theta_t} \big\rVert =0.
\end{align*}
\end{lemma}
%\cpcomment{You need to make sure that $\eta^{(t)}$
%is lower bounded to ensure it is indeed the gradient but not its
%coefficient that approaches zero, but there is no assumption on this variable in the
%lemma statement.}
%\updatecomment{Lower bounded $\eta^{(t)}$ are required. We add a sentence to assume that the step sizes are lower bounded in Subsection C.1.}


%\updatecomment{We have checked the green comments in the Proof  of \Cref{lemma: convergence to stationarity}.}
\begin{proof}[Proof of \Cref{lemma: convergence to stationarity}]
%\mru{TBD}
Under APG, we have that for any $t\in \mathbb{N}$,
\begin{equation}
   V^{\pi_{\omega}^{(t+1)}}(\mu) \geq V^{\pi_{\theta}^{(t+1)}}(\mu)\geq    V^{\pi_{\omega}^{(t)}}(\mu) \geq V^{\pi_{\theta}^{(t)}}(\mu).\label{eq: V omega >= Vtheta}
\end{equation}
By \cref{eq: V omega >= Vtheta} and that $V^{\pi_\theta}(\mu)\leq
\frac{1}{1-\gamma}$ for all $\theta$ from \Cref{lemma: reward range to
value range},
we know that the
limits of both $V^{\pi_{\omega}^{(t)}}(\mu)$ and $V^{\pi_{\theta}^{(t)}}(\mu)$ exist and 
$\lim_{t\rightarrow \infty} V^{\pi_{\omega}^{(t)}}(\mu) =\lim_{t\rightarrow \infty} V^{\pi_{\theta}^{(t)}}(\mu)$.
Therefore,
by the update rule \cref{algorithm:eq1} of APG, the
Lipschitz continuity of $\nabla_\theta V^{\pi_\theta}(\mu)$ from
\Cref{lemma:mdp_smoothness}, and our assumption that $\eta^{(t)}$ is
bounded away from zero, we further see
\begin{equation}
   \lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(\mu)\rvert_{\theta=\omega^{(t)}} \big\rVert =0. \label{eq: staionarity in omega_t}
\end{equation}
By \cref{eq: staionarity in omega_t} {and again application
	of \cref{algorithm:eq1} and the Lipschitz continuity of
	$\nabla_\theta V^{\pi_\theta}(\mu)$ together with the boundedness
	of $\{\eta^{(t)}\}$},
%\citep[Lemma D.4]{agarwal2021theory},
we also have
\begin{equation}
   \lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(\mu)\rvert_{\theta=\theta^{(t)}} \big\rVert =0. \label{eq: staionarity in theta_t}
\end{equation}
By the expression of softmax policy gradient in
\Cref{lemma:softmax_pg}, \cref{eq: staionarity in omega_t} and \cref{eq: staionarity in theta_t} imply that for all $(s,a)$,
\begin{align}
    &\pi_{\omega}^{(t)}(a|s)A^{\pi_{\omega}^{(t)}}(s,a)\rightarrow 0, \quad \text{as } t\rightarrow \infty,\label{eq:sum of Is+ and Is- eq1} \\
    &\pi_{\theta}^{(t)}(a|s)A^{\pi_{\theta}^{(t)}}(s,a)\rightarrow 0, \quad \text{as } t\rightarrow \infty.\label{eq:pi A theta goes to 0} 
\end{align}
Therefore, we have that for every state $s\in \mathcal{S}$,
\begin{align*}
   &\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\omega^{(t)}} \big\rVert =0,\\
   &\lim_{t\rightarrow \infty} \big\lVert \nabla_\theta V^{\pi_{\theta}}(s)\rvert_{\theta=\theta^{(t)}} \big\rVert =0.
   \qedhere
\end{align*}
\end{proof}

\begin{comment}
\pch{For ease of the following discussion, let $\bm{V}^{\pi}$ denote the $\lvert \cS\rvert$-dimensional vector that has all the $V^\pi(s)$ of all the states $s\in \cS$ as its entries.
Note that \Cref{lemma: convergence to stationarity} tells us that under APG, the sequence of policies would converge to stationary points, which might not be unique.
In other words, if we consider the trajectory of $\bm{V}^{\pi^{(t)}}$, there could be multiple accumulation points.
Accordingly, given any initialization $\theta^{(0)}$, let
$\bV(\theta^{(0)})$ denote the set of accumulation points,
\textit{i.e.},
\begin{equation}
    \bV(\theta^{(0)}):=\{\bm{V}:\}
\end{equation}
}
\end{comment}

% \begin{lemma}
% \label{lemma: monotone limits exist}
% Under APG, the following statements hold almost surely: 
% \begin{itemize}
%     \item The limits $\lim_{t\rightarrow \infty}V^{\pi_\theta^{(t)}}(s)$, $\lim_{t\rightarrow \infty}Q^{\pi_\theta^{(t)}}(s,a)$, and $\lim_{t\rightarrow \infty}A^{\pi_\theta^{(t)}}(s,a)$ all exist, for all $s\in \cS$ and all $a \in \cA$.
%     \item The limits $\lim_{t\rightarrow \infty}V^{\pi_\omega^{(t)}}(s)$, $\lim_{t\rightarrow \infty}Q^{\pi_\omega^{(t)}}(s,a)$, and $\lim_{t\rightarrow \infty}A^{\pi_\omega^{(t)}}(s,a)$ all exist, for all $s\in \cS$ and all $a \in \cA$.
%     \item $\lim_{t\rightarrow \infty}V^{\pi_\theta^{(t)}}(s) = \lim_{t\rightarrow \infty}V^{\pi_\omega^{(t)}}(s)$ for all $s \in\cS$.
%     \item $\lim_{t\rightarrow \infty}Q^{\pi_\theta^{(t)}}(s,a) = \lim_{t\rightarrow \infty}Q^{\pi_\omega^{(t)}}(s,a)$ for all $s\in\cS$ and all $a\in\cA$.
%     \item $\lim_{t\rightarrow \infty}A^{\pi_\theta^{(t)}}(s,a) = \lim_{t\rightarrow \infty}A^{\pi_\omega^{(t)}}(s,a)$ for all $s\in\cS$ and all $a\in\cA$.
% \end{itemize}

% \end{lemma}
\begin{lemma}
\label{lemma: monotone limits exist}
{Under the setting of \Cref{lemma: convergence to
stationarity},}
the following statements hold almost surely:
\begin{itemize}
    \item The limits $\lim_{t\rightarrow \infty}V^{\pi_\omega^{(t)}}(s)$, $\lim_{t\rightarrow \infty}Q^{\pi_\omega^{(t)}}(s,a)$, and $\lim_{t\rightarrow \infty}A^{\pi_\omega^{(t)}}(s,a)$ all exist for all $s\in \cS$ and all $a \in \cA$.
    \item The limits $\lim_{t\rightarrow \infty}V^{\pi_\theta^{(t)}}(s)$, $\lim_{t\rightarrow \infty}Q^{\pi_\theta^{(t)}}(s,a)$, and $\lim_{t\rightarrow \infty}A^{\pi_\theta^{(t)}}(s,a)$ all exist for all $s\in \cS$ and all $a \in \cA$.
\end{itemize}
Furthermore, we have
\begin{equation*}
    \lim_{t\rightarrow \infty}V^{\pi_\omega^{(t)}}(s) = \lim_{t\rightarrow \infty}V^{\pi_\theta^{(t)}}(s); \quad \lim_{t\rightarrow \infty}Q^{\pi_\omega^{(t)}}(s,a) = \lim_{t\rightarrow \infty}Q^{\pi_\theta^{(t)}}(s,a); \quad \lim_{t\rightarrow \infty}A^{\pi_\omega^{(t)}}(s,a) = \lim_{t\rightarrow \infty}A^{\pi_\theta^{(t)}}(s,a)
\end{equation*}
for all $s\in\cS$ and all $a\in\cA$ when these limits exist when these
limits exist.


\end{lemma}
\begin{proof}[Proof of \Cref{lemma: monotone limits exist}]
Recall that we use $\bm{V}^{\pi}$ to denote the $\lvert
\cS\rvert$-dimensional vector whose $s$-th component is $V^\pi(s)$ for
all $s\in \cS$. Our first goal is to show that the limit of the value
vector $\bm{V}^{\pi_{\omega}^{(t)}}$ exists, \textit{i.e.},
$\lim_{t\rightarrow\infty} V^{\pi_{\omega}^{(t)}}(s)$ exist for all
$s\in\cS$.
We define
% For any $\varepsilon > 0$, we define
% \begin{align*}
%     \mathcal{C}_{\varepsilon} &\coloneqq \Big\{ (\pi, \bm{V}^{\pi}) : \big\lvert \pi(a | s) A^{\pi}(s, a)\big\rvert < \varepsilon \text{, for all } (s, a) \in \cS\times\cA \Big\}, \\
%     \mathcal{V}_{\varepsilon} &\coloneqq \Big\{ \bm{V}^{\pi} : \exists \pi \text{ such that } (\pi, \bm{V}^{\pi}) \in \mathcal{C}_{\varepsilon} \Big\}.
% \end{align*}
% Both $\mathcal{C}_{\varepsilon}$ and $\mathcal{V}_{\varepsilon}$ are sequences of decreasing sets as $\varepsilon \rightarrow 0$. Therefore, by the limit of decreasing sequence of sets, we have
\begin{align}
    % \lim_{\varepsilon\rightarrow 0} \mathcal{C}_{\varepsilon} &= \bigcap_{k=1}^{\infty} \mathcal{C}_{1/k} = \Big\{ (\pi, \bm{V}^{\pi}) : \big\lvert \pi(a | s) A^{\pi}(s, a)\big\rvert = 0 \text{, for all } (s, a) \in \cS\times\cA \Big\} \eqqcolon \mathcal{C}, \label{def:mathcal{C}}\\
    \mathcal{V} \coloneqq \Big\{ \bm{V}^{\pi} : \big\lvert \pi(a | s)
	A^{\pi}(s, a)\big\rvert = 0 , \forall (s, a) \in \cS\times\cA \Big\}. \label{def:mathcal{V}}
\end{align}
Before starting our proof, we make the following claim.
\begin{claim}
	\label{claim}
	The cardinality of $\mathcal{V}$ is at most $\lvert \cA\rvert^{\lvert \cS\rvert}$.
\end{claim}
To prove \Cref{claim}, we first observe that there are $\lvert
\cA\rvert^{\lvert \cS\rvert}$ deterministic policies. {In addition, by
\Cref{lemma:sum_pi_A}, we know that the value vector of any deterministic policy belongs to $\mathcal{V}$.
For any stochastic policy $\pi$ such that $\bm{V}^{\pi} \in
\mathcal{V}$, by \cref{def:mathcal{V}}, it follows that for any
$(s, a)$ satisfying the condition $\pi(a|s) > 0$, we have $A^{\pi}(s, a)
= 0$. Consequently, selecting the deterministic policy $\pi'$
associated with $\pi$, wherein for all states $s \in \cS$ we set
$\pi'(a|s) = 1$ for some action $a$ satisfying $\pi(a|s) > 0$, allows
us to confirm that $\bm{V}^{\pi} = \bm{V}^{\pi'}$ using
\Cref{lemma:perf_diff}. Hence, for every value vector $\bm{V}^{\pi}$
in $\mathcal{V}$, there exists at least one corresponding
deterministic policy. Since there are only $\lvert
\cA\rvert^{\lvert \cS\rvert}$ deterministic policies,  the number of
distinct value vectors in $\mathcal{V}$ is at most $\lvert
\cA\rvert^{\lvert \cS\rvert}$, establishing the claim.}
%\cpfn{I guess your argument is that for each
%	stochastic policy that is in $\sC$, you have $\pi(a|s) \in (0,1)$
%	for multiple $a$ with $A = 0$ so that can reduce to only one pi or
%	something like that? Intuitively plausible but please expand the
%explanation. \updatecomment{We expand the explanation here. Please take a look.}}

With \Cref{claim} proven, we are now ready to prove \Cref{lemma:
monotone limits exist}.
For any point $x$ and any set $Y$,
we define 
\[
	d(x, Y) \coloneqq \inf_{y \in Y} \lVert y - x \rVert_{1}
\]
as the distance between $x$ and $Y$ measured by the $L_1$-norm.
We first show that 
\begin{equation}
	\label{eq:conv}
	\lim_{t\rightarrow\infty} d(\bm{V}^{\pi_{\omega}^{(t)}}, \cV) =
	0.
\end{equation}
{
Given any $\varepsilon > 0$, let $\varepsilon' = \frac{(1-\gamma)\varepsilon}{|\cS|^2}$.
By \cref{eq:sum of Is+ and Is- eq1}, we know that there exists
$T \geq 0$ such that
\begin{equation}
	\label{eq:piA}
	\lvert
	\pi_{\omega}^{(t)}(a|s)A^{\pi_{\omega}^{(t)}}(s,a)\rvert <
	\frac{\varepsilon'}{ |\cA|},\quad \forall (s,a) \in \cS \times \cA, \quad
	\forall t \geq T.
\end{equation}
Since $\sum_{a\in\cA} \pi(a|s) = 1$ for any $s \in \cS$ and any policy
$\pi$, there must be at least one action at each state satisfying
$\pi_{\omega}^{(t)}(a|s) \ge 1 / |\cA|$. We can thus observe from
\cref{eq:piA} that for
any $t \ge T$ and any $s\in\cS$, there must be an action $a_{s}^{(t)}$ such that $\lvert A^{\pi_{\omega}^{(t)}}(s,a_{s}^{(t)})\rvert < \varepsilon'$.
Therefore, for every $t \ge T$, we pick $\bm{V}^{(t)}
\in \cV$ as the value vector corresponding to the deterministic policy
$\pi^{(t)}$ with $\pi^{(t)}(a_s^{(t)} | s) = 1$ and $\pi^{(t)}(a|s) = 0$ for all $a\neq a_s^{(t)}$ for all $s\in\cS$.
(Note that the value vector of any deterministic policy belongs to
$\mathcal{V}$.)
Then, we can see that for every $t \ge T$,
\begin{align}
    d(\bm{V}^{\pi_{\omega}^{(t)}}, \cV) &\le
    \lVert \bm{V}^{(t)} - \bm{V}^{\pi_{\omega}^{(t)}} \rVert_{1} \nonumber \\
    &= \sum_{s} \Big\lvert \frac{1}{1-\gamma} \sum_{s'} d_{s}^{\pi^{(t)}}(s') \sum_{a} \pi^{(t)}(a | s') A^{\pi_{\omega}^{(t)}}(s', a)\Big\rvert \label{eq: norm convergence eq1} \\
    &= \sum_{s} \Big\lvert \frac{1}{1-\gamma} \sum_{s'}
	\underbrace{d_{s}^{\pi^{(t)}}(s')}_{\in [0, 1]}
	A^{\pi_{\omega}^{(t)}}(s', a_{{s'}}^{(t)})\Big\rvert \label{eq: norm convergence eq2} \\
    &\le \sum_{s} \frac{1}{1-\gamma} \sum_{s'} \Big\lvert
	A^{\pi_{\omega}^{(t)}}(s', a_{{s'}}^{(t)})\Big\rvert \nonumber \\
    &=\frac{|\cS|}{1-\gamma} \sum_{s'} \Big\lvert
	A^{\pi_{\omega}^{(t)}}(s', a_{{s'}}^{(t)})\Big\rvert \nonumber \\
    &< \frac{|\cS|^2}{1-\gamma} \varepsilon' = \varepsilon, \nonumber
\end{align}
where \cref{eq: norm convergence eq1} holds by \Cref{lemma:perf_diff}
and \cref{eq: norm convergence eq2} is due to the fact that
$\pi^{(t)}(a_s^{(t)} | s) = 1$. Since $\varepsilon$ is arbitrary, we have
proven \cref{eq:conv}.}
%Moreover, by \Cref{claim}, $\cV$ is a finite set which directly implies that it is closed in the metric space $(\R^{|\cS|}, d)$. Hence, combining the above two results, we obtain the convergence of $\{\bm{V}^{\pi_{\omega}^{(t)}}\}_{t=1}^{\infty}$ into the set $\cV$.}
% By \cref{eq:sum of Is+ and Is- eq1}, we have that for any $k \in\mathbb{N}_{+}$, there exists $T_k$ such that $\big\lvert \pi_{\omega}^{(t)}(a | s) A^{\pi_{\omega}^{(t)}}(s, a)\big\rvert < 1/k$ for all $(s, a)\in\cS\times \cA$ and $t \ge T_k$. Thus, we have 
% 	$(\pi_{\omega}^{(t)}, \bm{V}^{\pi_{\omega}^{(t)}}) \in
% 	\mathcal{C}$
% 	as $t \rightarrow \infty$, leading to $\bm{V}^{\pi_{\omega}^{(t)}}
% 	\in \mathcal{V}$ as $t \rightarrow \infty$.
% \cpfn{I see your point,
%		but this argument is not rigorous.
%		You probably meant to argue that the distance between $(\pi^t,
%		V^t)$ and $\cV$ decreases to zero or something like that, but
%		you need to indeed check the distance. This measure of
%	$\pi\cdot A$ is not a valid distance measure. \updatecomment{What we want to show is that if $(\pi^t, \bm{V}^t)$ do not belong to $\mathcal{C}$ as t goes to infinity, then there must exist some $\epsilon > 0$ and any large enough $T$ such that $(\pi^T, \bm{V}^T) \notin \mathcal{C}_\epsilon$, which is not possible due to \cref{eq:sum of Is+ and Is- eq1}. What do you think?}
%	\cpcomment{The flaw is that $(\pi^t, \bm{V}^t) \notin \mathcal{C}$
%	for any $t$. You only have that for any $\epsilon > 0$ you can
%	find a corresponding $t$ such that $|\pi^t A^t| < \epsilon$ but
%	you don't have such a $t$ for $\epsilon = 0$.
%	and therefore this claim of ``$(\pi^t, \bm{V}^t)$ do
%	not belong to $\mathcal{C}$ as t goes to infinity'' is in general
%	always true.
%	Infinity doesn't work this way.
%	If you want to write infinity, one way is to first establish that
%	the sequence indeed converges to a point, and that point is in
%	$mathcal{C}$,
%	but surely that is not guaranteed.
%	For what you are arguing, I guess showing that the distance
%	between $(\pi^t, V^t)$ and $\mathcal{C}$ decreases to $0$ suffices.
%	But you need to prove that with a proper norm.
%	The current criterion of $|\pi^t A^t|$ might not be linked with a
%	distance measure.
%}
%\updatecomment{We have updated the proof argument.}
%}

Accordingly, since $\cV$ is a finite and bounded (and thus compact) set according to \Cref{claim},
there are two possible scenarios:
(i) There exists $\bm{V} \in \cV$ such that
$\lim_{t \rightarrow \infty} 
\bm{V}^{\pi_{\omega}^{(t)}}=\bm{V}$; (ii)
$\big\{\bm{V}^{\pi_{\omega}^{(t)}}\big\}_{t=1}^{\infty}$ has at least
two limit points in $\mathcal{V}$.

For (i), we obtain the desired results. Regarding (ii), we prove that
with probability one, this scenario will not occur.
% For any two deterministic policies $\pi_1$ and $\pi_2$ with distinct value
% vectors (i.e., $\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$), we know that the set of $\mu$ such that $V^{\pi_1}(\mu) = V^{\pi_2}(\mu)$ is a hyperplane with strictly smaller dimension in $\Delta(\cS)$ due to the given hypothesis $\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$. Thus, the set of $\mu$ such that $V^{\pi_1}(\mu) = V^{\pi_2}(\mu)$ is of measure zero in $\Delta(\cS)$. Additionally, since there are only finitely many deterministic policies, the union of those sets of $\mu$ is still of measure zero in $\Delta(\cS)$. Hence, by the uniformly random initialization of the surrogate
% initial state distribution $\mu$, we have that with probability one, any two deterministic policies $\pi_1$ and $\pi_2$ with distinct value
% vectors (i.e., $\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$), satisfy
% $V^{\pi_1}(\mu) \neq V^{\pi_2}(\mu)$.
{For any two distinct value vectors $\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$
in $\mathcal{V}$, we know that the set of $\mu$ such that
$V^{\pi_1}(\mu) = V^{\pi_2}(\mu)$ is a subset in $\Delta(\cS)$ with dimension strictly less than the dimension of $\Delta(\cS)$ due
to the given hypothesis $\bm{V}^{\pi_1}\neq
\bm{V}^{\pi_2}$.
Thus, the set of $\mu$ such that $V^{\pi_1}(\mu) = V^{\pi_2}(\mu)$ is
of measure zero in $\Delta(\cS)$. Additionally, since there are only
finitely many distinct value vectors in $\mathcal{V}$ by \Cref{claim}, the union of those sets of $\mu$ is still of measure zero in $\Delta(\cS)$. Hence, by the uniformly random initialization of the surrogate initial state distribution $\mu$, we have that with probability one, any two distinct value vectors $\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$ in $\mathcal{V}$ satisfy
$V^{\pi_1}(\mu) \neq V^{\pi_2}(\mu)$.}


%Since $\{\bm{V}^{\pi_{\omega}^{(t)}}\}$ is bounded by \Cref{lemma:
%reward range to value range}, we know that
%$\{\bm{V}^{\pi_{\omega}^{(t)}}\}$ has at least one limit point.
Let $\bm{V}_1$ and $\bm{V}_2$ be two distinct limit points in
in scenario (ii), and $\{i_t\}$ and $\{j_t\}$ be two infinite index
sequences such that
\begin{equation*}
	\lim_{t \rightarrow \infty} \bm{V}^{\pi_{\omega}^{(i_t)}} = \bm{V}_1, \quad
	\lim_{t \rightarrow \infty} \bm{V}^{\pi_{\omega}^{(j_t)}} = \bm{V}_2,
\end{equation*}
which implies
\begin{equation}
	\label{eq:limit}
	\lim_{t \rightarrow \infty} V^{\pi_{\omega}^{(i_t)}}(\mu) =
	V_1(\mu), \quad
	\lim_{t \rightarrow \infty} V^{\pi_{\omega}^{(j_t)}}(\mu) =
	V_2(\mu).
\end{equation}

We have argued that with probability one, $V_1(\mu) \neq V_2(\mu)$,
and let us assume without loss of generality that $V_1(\mu) >
V_2(\mu)$ and denote $\epsilon \coloneqq V_1(\mu) - V_2(\mu)$.
From \cref{eq:limit}, almost surely there is $T_1 \geq 0$ such that
\begin{equation}
V^{\pi_{\omega}^{(i_t)}}(\mu) > V_1(\mu) - \frac{\epsilon}{2},\quad \forall
t \geq T_1.
\label{eq:Vvalue}
\end{equation}
By \cref{eq: V omega >= Vtheta}, we see that
$V^{\pi_{\omega}^{(t)}}(\mu)$ is monotonically increasing, which
together with \cref{eq:Vvalue} implies that
\[
V^{\pi_{\omega}^{(t)}}(\mu) \geq V_2 (\mu) + \frac{\epsilon}{2},
\quad \forall t \geq i_{T_1},
\]
contradicting the second equality of \cref{eq:limit} and that $\{j_t\}$ should
be an infinite sequence.
Therefore,
$\{\bm{V}^{\pi_{\omega}^{(t)}}\}$ converges to a point.
Since
$\lim_{t\rightarrow\infty} V^{\pi_{\omega}^{(t)}}(s)$ exists for all
$s\in\cS$,
we see that $\lim_{t\rightarrow \infty}Q^{\pi_\omega^{(t)}}(s,a)$ and
therefore $\lim_{t\rightarrow \infty}A^{\pi_\omega^{(t)}}(s,a)$ also
exist for all $s\in \cS$ and all $a \in \cA$ according to \cref{eq:state_value_function}.
%Therefore,
%$\bm{V}^{\pi_{\omega}^{(t)}}$ can only move to a different value vector in $\mathcal{V}$ with improved $V^{\pi_{\omega}^{(t)}}(\mu)$ since if $\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$ in $\mathcal{V}$ then $V^{\pi_1}(\mu) \neq V^{\pi_2}(\mu)$.
%Furthermore, by Claim (a), it can only move to different value vectors with only finitely many times. Hence, we obtain that $\lim_{t\rightarrow\infty} V^{\pi_{\omega}^{(t)}}(s)$ exist for all $s\in\cS$. Finally, since $\lim_{t\rightarrow \infty}{V}^{\pi_{\omega}^{(t)}}(s)$ exists for all $s\in\cS$, we know that $\lim_{t\rightarrow \infty}{Q}^{\pi_{\omega}^{(t)}}(s, a)$ exists for all $(s, a)\in \cS\times\cA$ by \cref{eq:state_action_value_function}. Additionally, $A^{\pi_{\omega}^{(t)}}(s, a) = Q^{\pi_{\omega}^{(t)}}(s, a) - V^{\pi_{\omega}^{(t)}}(s)$, we also obtain that the limit of $A^{\pi_{\omega}^{(t)}}(s, a)$ exist for all $(s, a)\in \cS\times\cA$.
Existence of the limit of $\{\bm{V}^{\pi_{\theta}^{(t)}}\}$,
$\{Q^{\pi_\theta^{(t)}}(s,a)\}$, and $\{A^{\pi_\theta^{(t)}}(s,a)\}$
follows the same argument above with \cref{eq:sum of Is+ and Is- eq1}
replaced by \cref{eq:pi A theta goes to 0}.
%Specifically, by utilizing the sets described in \cref{def:mathcal{C}}
%and \cref{def:mathcal{V}}, and integrating \cref{eq:pi A theta goes to
%0} with analogous reasoning, we can conclude the existence of the
%limit $\bm{V}^{\pi_{\theta}^{(t)}}$ as $t \rightarrow \infty$. Since
%$\lim_{t\rightarrow\infty} V^{\pi_{\theta}^{(t)}}(s)$ exist for all
%$s\in\cS$, $\lim_{t\rightarrow \infty}Q^{\pi_\theta^{(t)}}(s,a)$, and
%therefore $\lim_{t\rightarrow \infty}A^{\pi_\theta^{(t)}}(s,a)$ also
%exist for all $s\in \cS$ and all $a \in \cA$ according to \cref{eq:state_value_function}.

Finally, we demonstrate that the limits of the value function, the
$Q$-value function, and the advantage function with respect to
$\omega^{(t)}$ and $\theta^{(t)}$ are equal.
It suffices to show that $\lim_{t\rightarrow
\infty}V^{\pi_\omega^{(t)}}(s) = \lim_{t\rightarrow
\infty}V^{\pi_\theta^{(t)}}(s)$ for all $s\in\cS$, \textit{i.e.}, $\lim_{t\rightarrow \infty} \bm{V}^{\pi_{\omega}^{(t)}} = \lim_{t\rightarrow \infty} \bm{V}^{\pi_{\theta}^{(t)}}$.
We will prove it by contradiction.
Let 
\[
	\bm{V}^{\pi_{\omega}^{(\infty)}} \coloneqq \lim_{t\rightarrow
	\infty} \bm{V}^{\pi_{\omega}^{(t)}},\quad  \bm{V}^{\pi_{\theta}^{(\infty)}} \coloneqq \lim_{t\rightarrow \infty} \bm{V}^{\pi_{\theta}^{(t)}}
\]
and suppose that $\bm{V}^{\pi_{\omega}^{(\infty)}} \neq
\bm{V}^{\pi_{\theta}^{(\infty)}}$.
Recall that from our uniformly random initialization of $\mu$, if
$\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$ in $\mathcal{V}$, then
$V^{\pi_1}(\mu) \neq V^{\pi_2}(\mu)$ almost surely.
We know that both $\bm{V}^{\pi_{\omega}^{(\infty)}}$ and $\bm{V}^{\pi_{\theta}^{(\infty)}}$ belong to $\mathcal{V}$.
By the hypothesis, with probability one we have
$V^{\pi_{\omega}^{(\infty)}}(\mu) \neq
V^{\pi_{\theta}^{(\infty)}}(\mu)$, leading to the contradiction due to
the fact that $\lim_{t\rightarrow \infty} V^{\pi_{\omega}^{(t)}}(\mu)
=\lim_{t\rightarrow \infty} V^{\pi_{\theta}^{(t)}}(\mu)$ from \cref{eq: V omega >= Vtheta}.
Hence, we obtain that with probability one, $\lim_{t\rightarrow \infty}V^{\pi_\omega^{(t)}}(s) = \lim_{t\rightarrow \infty}V^{\pi_\theta^{(t)}}(s)$ for all $s\in\cS$, and by \cref{eq:state_action_value_function} we also obtain the desired results for both the $Q$-value function and the advantage function.
\qedhere
%     Recall that we use $\bm{V}^{\pi}$ to denote the $\lvert \cS\rvert$-dimensional vector of the $V^\pi(s)$ of all the states $s\in \cS$.
% \cpupdate{
% 	\Cref{lemma: convergence to stationarity} \st{tells us that under APG,
% 	the sequence of policies would converge to either one or multiple
% stationary points with the same
% 	$V^{\pi}(\mu)$.
%     In other words, if we consider the trajectory of $\bm{V}^{\pi^{(t)}}$, there could possibly be multiple accumulation points, which all have the same $V^{\pi}(\mu)$. 
% With that said, o}}
% \cpupdate{Our first} goal is to show that the limit of the value vector $\bm{V}^{\pi^{(t)}}$ also exists.\footnote{\cpcomment{
% 	\begin{itemize}
% 		\item $\pi^{(t)}$ is not defined up to my memory
% 		\item You have no guarantee that there is at least one limit
% 			point. Also there is no such thing of converging to
% 			multiple points. I am keeping your original text here for
% 			reference, but please remove them once you've understood
% 		the concept.
% \end{itemize}
% }
% }
%     %Accordingly, given any initialization $\theta^{(0)}$, let $\bV(\theta^{(0)})$ denote the set of accumulation points, i.e.,
%     %\begin{equation}
%     %    \bV(\theta^{(0)}):=\{\bm{V}:\}
%     %\end{equation} 
%     To achieve this, we first divide all the policies into multiple categories by defining equivalence classes as follows: For each real vector $\bm{V}\in\mathbb{R}^{\lvert\cS\rvert}$,
%     \begin{equation}
%         \mathcal{C}(\bm{V}):=\Big\{\pi_{\theta}: \nabla_\theta V^{\pi_\theta}(\mu)=0\hspace{2pt} \text{and}\hspace{2pt}   \bm{V}^{\pi_\theta}=\bm{V}\Big\}.\label{eq:C_V}
%     \end{equation}
%     \textit{\textbf{Claim (a).} There are at most $\lvert \cA\rvert^{\lvert \cS\rvert}$ non-empty equivalence classes.}\\    
%     To prove Claim (a), let us first fix some non-empty
% 	$\mathcal{C}(\bm{V})$. For any stochastic policy in
% 	$\mathcal{C}(\bm{V})$, one can verify that there must be a
% 	corresponding deterministic policy in $\mathcal{C}(\bm{V})$ by
% 	using the stationarity condition in \cref{eq:C_V} and the
% 	performance difference lemma in \Cref{lemma:perf_diff}. Hence,
% 	every non-empty $\mathcal{C}(\bm{V})$ must consist of at least one
% 	deterministic policy.\footnote{\cpcomment{Still having trouble
% 		understanding this existence part. How do you do
% 		differentiation with respect to $\theta$ when this is a
% 	deterministic policy not parameterized? Also, according to later
% developments, it looks like those solution policies do not really
% correspond to any $\theta$ that is in $R^n$ because you will have some
% coordinates at infinity, and thus it is not really a point of
% $\theta$.
% In that regard, looks like your equivalence classes are all empty. I
% am proceeding on assuming that this claim is true, but likely there
% are quite a lot of issues here.}}
%     Moreover, since there are only $\lvert \cA\rvert^{\lvert
% 	\cS\rvert}$ deterministic policies, there shall indeed at most be $\lvert \cA\rvert^{\lvert \cS\rvert}$ non-empty equivalence classes.

% By %Claim (a) and
% the uniform random initialization of the surrogate
% initial state distribution $\mu$, we know that with probability one,
% any two deterministic policies $\pi_1$ and $\pi_2$ with distinct value
% vectors (i.e., $\bm{V}^{\pi_1}\neq \bm{V}^{\pi_2}$), satisfy
% $V^{\pi_1}(\mu) \neq V^{\pi_2}(\mu)$.
% In other words, we know that
% with probability one, each non-empty equivalence classes
% $\mathcal{C}(\bm{V})$ corresponds  to a different value of $\langle \mu, \bm{V}\rangle$.
% By \Cref{lemma: convergence to stationarity} and the fact that $\{\bm{V}^{\pi^{(t)}}\}$ stays in the compact
% set $[0,(1 - \gamma)^{-1}]^{|\mathcal{S}|}$, we know the limit
% of the value vector $\bm{V}^{\pi^{(t)}}$ also exists, i.e.,
% $\lim_{t\rightarrow \infty}{V}^{\pi^{(t)}}(s)$ exists, for every state
% $s\in \cS$.

%\footnote{\cpcomment{We know A exists and therefore A exists? What do you want to say?} \updatecomment{We want to say that since $\lim V^{(t)}$ exists, we have $\lim Q^{(t)}$ exists by (1). We update this issue.}}
% \mru{By \Cref{lemma:perf_diff} and \Cref{lemma:sum_pi_A}, for all $s \in \cS$ we have: }

% \color{blue}
% \begin{align}
%     \Big| V^{\pi_{\theta}^{(t)}}(s) - V^{\pi_{\omega}^{(t-1)}}(s) \Big|
%     &= \Big| \frac{1}{1-\gamma} \sum_{s' \in \cS } d^{\pi_{\theta}^{(t)}}_{s}(s') \sum_{a \in \cA} \big(\pi_{\theta}^{(t)}(a|s') - \pi_{\omega}^{(t-1)}(a|s') \big)A^{\pi_{\omega}^{(t-1)}}(s',a) \Big| \label{eq: monotone limits exist 0} \\
%     &\le \frac{1}{1-\gamma} \sum_{s' \in \cS } d^{\pi_{\theta}^{(t)}}_{s}(s') \sum_{a \in \cA} \Big| \pi_{\theta}^{(t)}(a|s') - \pi_{\omega}^{(t-1)}(a|s') \Big| \cdot \Big| A^{\pi_{\omega}^{(t-1)}}(s',a) \Big| \nonumber \\
%     &\le \frac{1}{(1-\gamma)^2} \sum_{(s',a) \in \cS\times\cA} \Big| \pi_{\theta}^{(t)}(a|s') - \pi_{\omega}^{(t-1)}(a|s') \Big| \label{eq: monotone limits exist 1} \\
%     &\le \frac{1}{(1-\gamma)^2} \sum_{(s',a) \in \cS\times\cA} \Big| \frac{5}{4} \cdot \lVert \theta^{(t)}_{s'} - \omega^{(t-1)}_{s'} \rVert^2_2 + \big\langle \nabla_{\theta_{s}} \pi_{\theta_s}^\top r_{a}\big\rvert_{\theta_s=\omega^{(t-1)}_{s'}}, \theta^{(t)}_{s'} - \omega^{(t-1)}_{s'} \big\rangle \Big| \label{eq: monotone limits exist 2} \\
%     &= \frac{1}{(1-\gamma)^2} \sum_{(s',a) \in \cS\times\cA} \Big| \frac{5}{4} \cdot \Big\lVert \eta^{(t)} \nabla_{\theta_{s}} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \Big\rVert^2_2 \nonumber\\
%     &\quad\quad\quad\quad\quad\quad\quad\quad\quad + \big\langle \nabla_{\theta_s} \pi_{\theta_s}(a|s') \big\rvert_{\theta_s=\omega^{(t-1)}_{s'}}, \eta^{(t)} \nabla_{\theta_s} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \big\rangle \Big| \label{eq: monotone limits exist 3}\\
%     &\le \frac{1}{(1-\gamma)^2} \sum_{(s',a) \in \cS\times\cA} \Big| \frac{5}{4} \cdot \Big\lVert \eta^{(t)} \nabla_{\theta_{s}} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \Big\rVert^2_2 \Big| \nonumber\\
%     &\quad\quad\quad\quad\quad\quad\quad\quad\quad + \Big| \big\langle \nabla_{\theta_s} \pi_{\theta_s}(a|s') \big\rvert_{\theta_s=\omega^{(t-1)}_{s'}}, \eta^{(t)} \nabla_{\theta_s} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \big\rangle \Big| \nonumber\\
%     &\le \frac{1}{(1-\gamma)^2} \sum_{(s',a) \in \cS\times\cA} \frac{5}{4} \cdot \Big\lVert \eta^{(t)} \nabla_{\theta_{s}} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \Big\rVert^2_2  + \frac{1}{4} \Big\lVert \eta^{(t)} \nabla_{\theta_s} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \Big\rVert_1 \label{eq: monotone limits exist 4}\\
%     &\le \frac{1}{(1-\gamma)^2} \sum_{(s',a) \in \cS\times\cA} \frac{5}{4} \cdot \Big\lVert \eta^{(t)} \nabla_{\theta_{s}} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \Big\rVert^2_2  + \frac{\lvert\cA\rvert}{4} \Big\lVert \eta^{(t)} \nabla_{\theta_s} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \Big\rVert_2^2\nonumber \\
%     &\le \frac{\lvert \cS \rvert \lvert \cA \rvert (5+\lvert \cA \rvert) \max_{t} \eta^{(t)}}{4(1-\gamma)^2} \cdot \Big\lVert \nabla_{\theta_s} V^{\pi_{\theta_s}^{(t)}}(\mu) \Big\rvert_{\theta_s = \omega^{(t-1)}_{s'}} \Big\rVert_2^2, \label{eq: monotone limits exist 5}
% \end{align}
% where (\ref{eq: monotone limits exist 1}) holds due to the condition $d^{\pi_\theta^{(t)}}s(s') \le 1$ and $A^{\pi_{\omega}^{(t-1)}}(s',a) \le \frac{1}{1-\gamma}$ for all $(s', a) \in \mathcal{S} \times \mathcal{A}$. (\ref{eq: monotone limits exist 2}) holds by \Cref{lemma:bandit_smoothness}, where $r_a$ represents the $|\mathcal{A}|$-dimensional vector with a $1$ in the $a$-th coordinate and $0$'s elsewhere. (\ref{eq: monotone limits exist 3}) holds through the update process of APG.  (\ref{eq: monotone limits exist 4}) holds since for all $(s, a) \in \cS \times \cA$
% \begin{align*}
%     \frac{\partial \pi_{\theta}(a|s)}{\partial \theta_{s, a'}}= \left\{\begin{matrix}
%     \pi_{\theta}(a|s)(1-\pi_{\theta}(a|s))  & \text{if } a = a'\\
%     -\pi_{\theta}(a|s)\pi_{\theta}(a'|s)  & \text{if } a \neq a'
%     \end{matrix}\right.
%     \le \frac{1}{4}.
% \end{align*}

% Combining \Cref{lemma: convergence to stationarity} with (\ref{eq: monotone limits exist 0}-\ref{eq: monotone limits exist 5}), we have 
% $\lim_{t \rightarrow \infty} \Big| V^{\pi_{\theta}^{(t)}}(s) - V^{\pi_{\omega}^{(t)}}(s)\Big| = 0$ for all $s \in \cS$. Based on the existence of $\lim_{t \rightarrow \infty}  V^{\pi_{\theta}^{(t)}}(s)$ we have

% \color{black}

%     \begin{itemize}
%         \item $\lim_{t\rightarrow \infty}V^{\pi_\theta^{(t)}}(s) = \lim_{t\rightarrow \infty}V^{\pi_\omega^{(t)}}(s)$ for all $s \in\cS$.
%         \item $\lim_{t\rightarrow \infty}Q^{\pi_\theta^{(t)}}(s,a) = \lim_{t\rightarrow \infty}Q^{\pi_\omega^{(t)}}(s,a)$ for all $s\in\cS$ and all $a\in\cA$.
%         \item $\lim_{t\rightarrow \infty}A^{\pi_\theta^{(t)}}(s,a) = \lim_{t\rightarrow \infty}A^{\pi_\omega^{(t)}}(s,a)$ for all $s\in\cS$ and all $a\in\cA$.
%     \end{itemize}
% \footnote{\cpcomment{But you do not have monotonicity for each coordinate, right?}}
\end{proof}
%%%%%
In the sequel, we use the following notations.
\begin{equation}
% 	\begin{cases}
% A^{(t)}(s,a) &\coloneqq A^{\pi_{\omega}^{(t)}}(s,a)\\
% Q^{(t)}(s,a) &\coloneqq Q^{\pi_{\omega}^{(t)}}(s,a)\\
% V^{(t)}(s) &\coloneqq V^{\pi_{\omega}^{(t)}}(s)
% \end{cases},
% \quad
\begin{cases}
A^{(\infty)}(s,a) &\coloneqq
\lim_{t\rightarrow\infty}A^{\pi_{\omega}^{(t)}}(s,a) = \lim_{t\rightarrow\infty}A^{\pi_{\theta}^{(t)}}(s,a),\\
Q^{(\infty)}(s,a) &\coloneqq \lim_{t\rightarrow\infty}Q^{\pi_{\omega}^{(t)}}(s,a) = \lim_{t\rightarrow\infty}Q^{\pi_{\theta}^{(t)}}(s,a),\\
V^{(\infty)}(s) &\coloneqq
\lim_{t\rightarrow\infty}V^{\pi_{\omega}^{(t)}}(s) \quad = \lim_{t\rightarrow\infty}V^{\pi_{\theta}^{(t)}}(s).
\end{cases}
\label{eq:def}
\end{equation}
We divide the action space into the following subsets based on the advantage function:
\begin{align*}
    I_s^{+}&:=\{a\in \cA: A^{(\infty)}(s,a)>0\},\\
    I_s^{-}&:=\{a\in \cA: A^{(\infty)}(s,a)<0\},\\
    I_s^{0}&:=\{a\in \cA: A^{(\infty)}(s,a)=0\}.
    %I_s^{\dagger}&:=\{a\in \cA: \limsup_{t\rightarrow \infty}A_t(s,a)>0, \liminf_{t\rightarrow \infty}A_t(s,a)<0\}
\end{align*}
The above action sets are well-defined as the limiting value functions
exist by \Cref{lemma: monotone limits exist}.
% {Moreover, we would like to highlight that our following results in
% 	\Cref{app:asym_conv:lemmas,app:asym_conv:all} are also applicable
% to the general MDP case, as long as the limiting value functions
% exist.}

For each state $s$, we define 
\begin{equation*}
    \Delta_s:=\min_{a\in I_s^+\cup I_s^-}\lvert A^{(\infty)}(s,a)\rvert.
\end{equation*}
Accordingly, we know that for each state $s\in \cS$, there must exist some $\bar{T}_s$ such that the following hold:
\begin{itemize}[leftmargin=*]
\item (i) For all $a\in I_s^+$,
    \begin{equation}
        A^{\pi_{\omega}^{(t)}}(s,a)\geq +\frac{\Delta_s}{4}, \quad \text{for all } t\geq \bar{T}_s,\label{eq:adv I_s+}
    \end{equation}
\item  (ii) For all $a\in I_s^-$,
\begin{equation}
    A^{\pi_{\omega}^{(t)}}(s,a)\leq -\frac{\Delta_s}{4}, \quad\text{for all }t\geq \bar{T}_s.\label{eq:adv I_s-}
\end{equation}
\item (iii) For all $a\in I_s^0$,
\begin{equation}
    \lvert A^{\pi_{\omega}^{(t)}}(s,a)\lvert \leq \frac{\Delta_s}{4}, \quad\text{for all }t\geq \bar{T}_s.\label{eq:adv I_s0}
\end{equation}
\end{itemize}


\begin{lemma}
\label{lemma:sum of Is+ and Is- goes to zero}
{Under the setting of \Cref{lemma: convergence to
stationarity},}
for any state $s\in \cS$,
we have 
\begin{equation*}
	\lim_{t \rightarrow \infty}\,
	\sum_{a\in I_s^{+}\cup I_s^{-}}\pi_\omega^{(t)}(a\rvert
	s)= 0,\quad
	\lim_{t \rightarrow \infty}\,
	\sum_{a\in I_s^{+}\cup I_s^{-}}\pi_\theta^{(t)}(a\rvert
	s)= 0.
\end{equation*}
As a result, we also have
\begin{equation*}
	\lim_{t \rightarrow \infty}\,
	\sum_{a\in I_s^{0}}\pi_\omega^{(t)}(a\rvert
	s)= 1,\quad
	\lim_{t \rightarrow \infty}\,
	\sum_{a\in I_s^{0}}\pi_\theta^{(t)}(a\rvert
	s)= 1.
\end{equation*}
\end{lemma}

\begin{proof}[Proof of \Cref{lemma:sum of Is+ and Is- goes to zero}]
%Given that the limiting value functions exist as well as the fact that
%$d^{\pi_\theta}_\mu(s)\geq \frac{\mu(s)}{1-\gamma}>0$, we know that
%for any state-action pair $(s,a)$,\footnote{\cpcomment{Isn't this
%	already shown in
%	the proof of \Cref{lemma: convergence to stationarity}?}
%\begin{equation}
%   \pi_{\theta}^{(t)}(a\rvert s)A^{\pi_{\theta}^{(t)}}(s,a)\rightarrow 0 \quad \text{as }t\rightarrow \infty.\label{eq:sum of Is+ and Is- eq1}
%\end{equation} 
%\begin{itemize}[leftmargin=*]
    %\item
	For any $a\in I_s^{+}$, we have
	$\lim_{t\rightarrow\infty}A^{\pi_{\omega}^{(t)}}(s,a) =
	\lim_{t\rightarrow\infty}A^{\pi_{\theta}^{(t)}}(s,a) > 0$. By
	\cref{eq:sum of Is+ and Is- eq1} and \cref{eq:pi A theta goes to
	0}, this implies that $\pi_\omega^{(t)}(a\rvert s)\rightarrow 0$
	and $\pi_\theta^{(t)}(a\rvert s)\rightarrow 0$ as $t\rightarrow
	\infty$ for all $a\in I_s^{+}$.
    Similarly, for any $a\in I_s^{-}$, we also have $\lim_{t\rightarrow\infty}A^{\pi_{\omega}^{(t)}}(s,a) = \lim_{t\rightarrow\infty}A^{\pi_{\theta}^{(t)}}(s,a) < 0$. Again, by \cref{eq:sum of Is+ and Is- eq1} and \cref{eq:pi A theta goes to 0}, this implies that $\pi_\omega^{(t)}(a\rvert s)\rightarrow 0$ and $\pi_\theta^{(t)}(a\rvert s)\rightarrow 0$ as $t\rightarrow \infty$ for all $a\in I_s^{-}$.
    Hence, we conclude that $\sum_{a\in I_s^{+}\cup I_s^{-}}\pi_\omega^{(t)}(a\rvert s)\rightarrow 0$ and $\sum_{a\in I_s^{+}\cup I_s^{-}}\pi_\theta^{(t)}(a\rvert s)\rightarrow 0$ as $t\rightarrow \infty$ due to the finiteness of the cardinality of $\mathcal{A}$.
\end{proof}
% It is worth noting that since we also have \cref{eq:sum of Is+ and Is- eq1}, the results of \Cref{lemma:sum of Is+ and Is- goes to zero} also hold for $\pi_{\omega}^{(t)}$.


{\begin{lemma}
\label{lemma:Is+ bounded}
    Consider any state $s\in \cS$. Let $a$ be an action in
	$I_{s}^{+}$.
{Under the setting of \Cref{lemma: convergence to
stationarity},}
	$\{\theta_{s,a}^{(t)}\}_{t=1}^{\infty}$ and $\{\omega_{s,a}^{(t)}\}_{t=1}^{\infty}$ are bounded from below.
\end{lemma}}
\begin{proof}[Proof of \Cref{lemma:Is+ bounded}]
	Recall the part of our definition in \cref{eq:adv I_s+} of
	$\bar{T}_s$.
	From \Cref{lemma:softmax_pg}, we see that
\begin{equation}
	\eta^{(t)} \nabla_{\theta_{s,a}}{V^{\pi_{\theta}}(\mu)}
	\Big\rvert_{\theta = \omega^{(t-1)}} \geq 0,\quad \forall t \geq
	\bar{T}_s+1.
	\label{eq:posgrad}
\end{equation}
	We let
	$\delta_{\bar{T}_s}:=\theta_{s,a}^{(\bar{T}_s)}-\theta_{s,a}^{(\bar{T}_s-1)}$.
	Regarding the case $\delta_{\bar{T}_s} \geq 0$,
	by \cref{eq:posgrad} and the update rules in
	\cref{algorithm:eq1,algorithm:eq2},
	the sequences $\{\theta_{s,a}^{(t)}\}_{t\geq \bar T_s+1},
	\{\omega_{s,a}^{(t)}\}_{t\geq \bar T_s+1}$ are monotonically
	increasing and therefore lower-bounded.

	On the other hand, if $\delta_{\bar{T}_s} < 0$, for any $M\in \bbN$, we have
    \begin{align}
        \theta^{(\bar{T}_s+M)}_{s,a}
        &=\omega^{(\bar{T}_s+M-1)}_{s,a}+\eta^{(\bar{T}_s+M)} \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(\bar{T}_s+M-1)}} \nonumber \\
        &\geq \theta^{(\bar{T}_s+M-1)}_{s,a}
         +\mathbb{I} \left\{V^{\pi_{\varphi}^{(\bar{T}_s + M -1)}}(\mu) \ge V^{\pi_{\theta}^{(\bar{T}_s + M -1)}}(\mu)\right \} \cdot \frac{\bar{T}_s+M-2}{\bar{T}_s+M+1}(\theta_{s,a}^{(\bar{T}_s+M-1)}-\theta_{s,a}^{(\bar{T}_s+M-2)}) \nonumber \\
        &\geq \theta_{s,a}^{(\bar{T}_s)}+\frac{\bar{T}_s-1}{\bar{T}_s+2}\delta_{\bar{T}_s}+\frac{\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+3)(\bar{T}_s+2)}\delta_{\bar{T}_s}+\cdots+\frac{(\bar{T}_s+M-2)\cdots (\bar{T}_s-1)}{(\bar{T}_s+M+1)\cdots (\bar{T}_s+2)}\delta_{\bar{T}_s}\label{eq:Is+ bounded eq3}\\
        &= \theta_{s,a}^{(\bar{T}_s)}+\Big[\frac{\bar{T}_s-1}{\bar{T}_s+2}+\frac{\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+3)(\bar{T}_s+2)}+\sum_{\tau=2}^{M}\frac{(\bar{T}_s+1)\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+\tau+2)(\bar{T}_s+\tau+1)(\bar{T}_s+\tau)}\Big] \delta_{\bar{T}_s},\nonumber
    \end{align}
    where \cref{eq:Is+ bounded eq3} holds by disregarding the updates
	contributed by the gradients taken at all $t > \bar{T}_s$, which
	are always nonnegative according to \cref{eq:posgrad}.
    
    We note that for any $M\in \bbN$,
    \begin{align}
        &~\sum_{\tau=2}^{M}\frac{(\bar{T}_s+1)\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+\tau+2)(\bar{T}_s+\tau+1)(\bar{T}_s+\tau)}\nonumber\\
        =&~(\bar{T}_s+1)\bar{T}_s(\bar{T}_s-1)\sum_{\tau=2}^{M}\frac{1}{2}\Big(\frac{1}{(\bar{T}_s+\tau)(\bar{T}_s+\tau+1)}-\frac{1}{(\bar{T}_s+\tau+1)(\bar{T}_s+\tau+2)}
		\Big)\nonumber\\
        =&~(\bar{T}_s+1)\bar{T}_s(\bar{T}_s-1)\cdot
		\frac{1}{2}\Big(\frac{1}{(\bar{T}_s+2)(\bar{T}_s+3)}-\frac{1}{(\bar{T}_s+M+1)(\bar{T}_s+M+2)}\Big)\nonumber\\
        \leq&~ \frac{\bar{T}_s}{2}.\label{eq:Is+ bounded eq8}
    \end{align}
    Therefore, it follows that for any $M\in \bbN$,
    \begin{align*}
        \theta^{(\bar{T}_s+M)}_{s,a}\geq
		\theta^{(\bar{T}_s)}_{s,a}-\left(2+\frac{\bar{T}_s}{2}\right)\lvert \delta_{\bar{T}_s}\rvert.
    \end{align*}
    Hence, $\theta^{(t)}_{s,a}\geq \theta^{(\bar{T}_s)}_{s,a}-(2+\frac{\bar{T}_s}{2})\lvert \delta_{\bar{T}_s}\rvert $ for all $t\geq \bar{T}_s$.
    As the gradient under softmax parameterization is always
	bounded according to \cref{eq:posgrad}, this also implies that $\{\omega^{(t)}_{s,a}\}_{t=1}^{\infty}$ is bounded from below for all $s\in\cS$ and $a\in I_{s}^{+}$.
\end{proof}

{\begin{lemma}
\label{lemma:Is- bounded}
    Consider any state $s\in \cS$. Let $a$ be an action in
	$I_{s}^{-}$.
{Under the setting of \Cref{lemma: convergence to
stationarity},}
	$\{\theta_{s,a}^{(t)}\}_{t=1}^{\infty}$ and $\{\omega_{s,a}^{(t)}\}_{t=1}^{\infty}$ are bounded from above.
\end{lemma}}
\begin{proof}[Proof of \Cref{lemma:Is- bounded}]
We follow the same procedure as that in
\Cref{lemma:Is+ bounded}.  Again, let $\delta_{\bar{T}_s}:=\theta_{s,a}^{(\bar{T}_s)}-\theta_{s,a}^{(\bar{T}_s-1)}$.
	From \cref{eq:adv I_s+} and \Cref{lemma:softmax_pg}, we see that
\begin{equation}
	\eta^{(t)} \nabla_{\theta_{s,a}}{V^{\pi_{\theta}}(\mu)}
	\Big\rvert_{\theta = \omega^{(t-1)}} \leq 0,\quad \forall t \geq
	\bar{T}_s+1.
	\label{eq:neggrad}
\end{equation}
Therefore, by \cref{algorithm:eq1,algorithm:eq2,eq:neggrad}, we have
\begin{align*}
    \theta^{(\bar{T}_s+1)}_{s,a}&=\omega^{(\bar{T}_s)}_{s,a}+\eta^{(\bar{T}_s+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(\bar{T}_s)}}\leq \omega^{(\bar{T}_s)}_{s,a}.
    %=\theta^{(\bar{T}_s)}_{s,a}+\frac{\bar{T}_s-1}{\bar{T}_s+2}(\theta_{s,a}^{(\bar{T}_s)}-\theta_{s,a}^{(\bar{T}_s-1)}).
\end{align*}
Regarding the case of $\delta_{\bar{T}_s} \leq 0$, the result directly
holds by \cref{eq:neggrad} as argued in the proof of \Cref{lemma:Is+
bounded}.
Considering $\delta_{\bar{T}_s} > 0$, for any $M\in \bbN$, we have
\begin{align*}
    \theta^{(\bar{T}_s+M)}_{s,a}
    &=\omega^{(\bar{T}_s+M-1)}_{s,a}+\eta^{(\bar{T}_s+M)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(\bar{T}_s+M-1)}}\\
    &\leq \theta^{(\bar{T}_s+M-1)}_{s,a}
    + \mathbb{I} \left\{V^{\pi_{\varphi}^{(T_0 + M -1)}}(\mu) \ge V^{\pi_{\theta}^{(T_0 + M -1)}}(\mu)\right \} \cdot\frac{\bar{T}_s+M-2}{\bar{T}_s+M+1}(\theta_{s,a}^{(\bar{T}_s+M-1)}-\theta_{s,a}^{(\bar{T}_s+M-2)})\\
    &\leq \theta_{s,a}^{(\bar{T}_s)}+\frac{\bar{T}_s-1}{\bar{T}_s+2}\delta_{\bar{T}_s}+\frac{\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+3)(\bar{T}_s+2)}\delta_{\bar{T}_s}+\cdots+\frac{(\bar{T}_s+M-2)\cdots (\bar{T}_s-1)}{(\bar{T}_s+M+1)\cdots (\bar{T}_s+2)}\delta_{\bar{T}_s}\\
    &=\theta_{s,a}^{(\bar{T}_s)}+\Big[\frac{\bar{T}_s-1}{\bar{T}_s+2}+\frac{\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+3)(\bar{T}_s+2)}+\sum_{\tau=2}^{M}\frac{(\bar{T}_s+1)\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+\tau+2)(\bar{T}_s+\tau+1)(\bar{T}_s+\tau)}\Big] \delta_{\bar{T}_s}.
\end{align*}
By \cref{eq:Is+ bounded eq8}, we know $\sum_{\tau=2}^{M}\frac{(\bar{T}_s+1)\bar{T}_s(\bar{T}_s-1)}{(\bar{T}_s+\tau+2)(\bar{T}_s+\tau+1)(\bar{T}_s+\tau)}\leq \frac{\bar{T}_s}{2}$. 
As a result, for any $M\in \bbN$,
\begin{align*}
    \theta^{(\bar{T}_s+M)}_{s,a}\leq \theta^{(\bar{T}_s)}_{s,a}+(2+\frac{\bar{T}_s}{2})\lvert \delta_{\bar{T}_s}\rvert.
\end{align*}
Hence, $\theta^{(t)}_{s,a}\leq \theta^{(\bar{T}_s)}_{s,a}+(2+\frac{\bar{T}_s}{2})\lvert \delta_{\bar{T}_s}\rvert $ for all $t\geq \bar{T}_s$.
As the gradient is bounded according to \cref{eq:neggrad}, this
also implies that $\{\omega^{(t)}_{s,a}\}_{t=1}^{\infty}$ is bounded from above for all $s\in\cS$ and $a\in I_{s}^{-}$.
\end{proof}

\begin{lemma}
\label{lemma:max Is0}
Consider any state $s\in \cS$.
{Under the setting of \Cref{lemma: convergence to
stationarity},}
if $I_s^{+}$ is non-empty, then
	\[
		\lim_{t \rightarrow \infty}\; \max_{a\in I_s^{0}}\,
		\omega_{s,a}^{(t)}= \infty,\quad
		\lim_{t \rightarrow \infty}\;
		\max_{a\in I_s^{0}} \theta_{s,a}^{(t)}= \infty.
	\]
\end{lemma}
\begin{proof}
    By \Cref{lemma:sum of Is+ and Is- goes to zero},
	we know $\sum_{a\in I_s^{0}}\pi_{\omega}^{(t)}(a\rvert
	s)\rightarrow 1$ and $\sum_{a\in I_s^{0}}\pi_{\theta}^{(t)}(a\rvert s)\rightarrow 1$ as $t\rightarrow \infty$.
    Moreover, by \Cref{lemma:Is+ bounded}, we know
	$\{\omega_{s,a}^{(t)}\}$ and $\{\theta_{s,a}^{(t)}\}$ are lower-bounded for all $a\in I_s^{+}$.
    Therefore, under the softmax policy parameterization, we obtain
	the desired results.
%	$\max_{a\in I_s^{0}}\omega_{s,a}^{(t)}\rightarrow \infty$.
%    \mru{Furthermore, since \Cref{lemma:sum of Is+ and Is- goes to zero,lemma:Is+ bounded} are also true for the parameter $\{\theta^{(t)}_{s, a}\}_{t=1}^{\infty}$, we can utilize the same argument to show that $\max_{a\in I_s^{0}}\theta_{s,a}^{(t)}\rightarrow \infty$.}\footnote{\updatecomment{Since \Cref{lemma:sum of Is+ and Is- goes to zero,lemma:Is+ bounded} also hold for $\theta$, we do not need the upper-boundedness of the step sizes $\eta^{(t)}$.}}
\end{proof}

Recall from \cref{eq:adv I_s-} that for all $a\in I_s^-$, we have $A^{\pi_{\omega}^{(t)}}(s,a)\leq -\frac{\Delta_s}{4}$ for all $t\geq \bar{T}_s$.
{\begin{lemma}
\label{lemma:Is- negative infinity}
Consider any state $s\in \cS$.
{Under the setting of \Cref{lemma: convergence to
stationarity},}
if $I_s^{+}$ is non-empty, then for any $a\in I_s^{-}$, we have $\omega_{s,a}^{(t)}\rightarrow -\infty$ as $t\rightarrow \infty$.
\end{lemma}}
\begin{proof}[Proof of \Cref{lemma:Is- negative infinity}]
We prove this by contradiction. 
Motivated by the proof of Lemma C11 in \citep{agarwal2021theory}, our
proof here extends their argument to the case with momentum by
considering the cumulative effect of all the gradient terms on the
policy parameter $\theta^{(t)}$.

{We will show that $\lim_{t\rightarrow\infty}\theta^{(t)}_{s, a} = -\infty$.
Then the desired result follows from the uniform boundedness of the gradient updates.
We first prove 
\begin{equation}
	\liminf_{t\rightarrow\infty}\theta^{(t)}_{s, a} = -\infty
	\label{eq:liminf}
\end{equation}
by contradiction.} Given an action $a\in I_s^{-}$, suppose that there exists $\vartheta$ such that $\theta_{s,a}^{(t)}>\vartheta$ for all $t\geq\bar{T}_s$.
Then, by \Cref{lemma:sum conservation,lemma:max Is0}, we know there must exist an action $a'\in \cA$ such that $\liminf_{t\rightarrow \infty}\theta_{s,a'}^{(t)}=-\infty$.
Let $\delta>0$ be some positive scalar such that $\theta_{s,a}^{(\bar{T}_s)}\geq \vartheta -\delta$. For each $t\geq \bar{T}_s$, define 
\begin{equation}
    \nu(t):=\sup\{\tau:\theta_{s,a'}^{(\tau)}\geq \vartheta-\delta,\quad \bar{T}_s\leq \tau\leq t \},\label{eq:Is- negative infinity 1}
\end{equation}
which is the latest iteration that $\theta_{s,a'}^{(\tau)}$ remains no
smaller than $\vartheta-\delta$.
We consider two cases: (i) $\{\nu(t)\}_{t=1}^{\infty}$ is bounded, and
(ii) $\lim_{t \rightarrow \infty} \nu(t) = \infty$.

For case (i), we define the following index set
\begin{equation}
    \cJ^{(t)}:=\Big\{\tau: \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(\tau)}}<0,\quad \nu(t)<\tau < t\Big\}.\label{eq:Is- negative infinity 2}
\end{equation}
and denote the cumulative effect (up to iteration $t$) of the gradient terms from those iterations in $\cJ^{(t)}$ as
\begin{equation}
    Z^{(t)}:=\sum_{t'\in \cJ^{(t)}} \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',t),\label{eq:Is- negative infinity 3}
\end{equation}
where $G(t',t)$ is defined in \cref{eq:G}.
If $\cJ^{(t)}=\emptyset$, we define $Z^{(t)}=0$.

By setting $R_{\text{max}} = 1$ in \Cref{lemma: reward range to value range}, we have the upper bounds $V^{\pi}(s) \le 1/(1-\gamma)$ for any $s\in\cS$ and any $\pi$, $Q^{\pi}(s, a) \le 1/(1-\gamma)$ for any $(s, a) \in\cS\times\cA$ and any $\pi$, and also $\lvert A(s, a)\rvert \le 1/(1-\gamma)$ for any $(s, a) \in\cS\times\cA$ and any $\pi$.
Leveraging these upper bounds and \Cref{lemma:softmax_pg}, we have
\begin{equation}
	\lvert\partial V^{\pi_{\theta}}(\mu)/\partial\theta_{s,a}\rvert \leq
	1/(1-\gamma)^2,\quad \forall (s, a) \in\cS\times\cA.
	\label{eq:boundV}
\end{equation}
Accordingly, for any $t>\bar{T}_s$, we have
%\cpcomment{Here when you bound $\nabla V$ by $(1- \gamma)^{-2}$ and
%later there is a place you used that ineq $|A(s,a)| \leq (1 -
%\gamma)^{-1}$ (both highlighted in red). This result is explained in
%the document, but it is never mentioned and is not that obvious from
%the definition. You could even just simply state that from the
%definition you get upper and lower bounds for $V$ and $Q$ and then
%$A$.}
%\updatecomment{We add \Cref{lemma: reward range to value range} to explain the upper bounds on the $V, Q$, and $A$. We also explain the upper bound of the partial derivatives.}
\begin{align}
	\nonumber
    Z^{(t)}
    &\leq \sum_{t'\in \cJ^{(t)}} \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}\cdot
		G(t',t)+\sum_{t':t'\notin \cJ^{(t)}, \nu(t)<t'<t}
		\underbrace{\eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',t)}_{\geq
				0, \text{by the definition of }\cJ^{(t)}}\\
    &\quad\quad +\sum_{t'\leq\nu(t)}\underbrace{\eta^{(t'+1)}\cdot
	\Big(\frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}+\frac{1}{(1-\gamma)^2}\Big)\cdot
G(t',t)}_{\geq 0, \text{ by \cref{eq:boundV}
}}\nonumber\\
    &= \sum_{t' \le t} \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',t)
		+\sum_{t'\leq\nu(t)}\eta^{(t'+1)}\frac{1}{(1-\gamma)^2}G(t',t)
		\nonumber\\
    &= (\theta_{s,a'}^{(t)}-\theta_{s,a'}^{(1)}) +\sum_{t'\leq\nu(t)}\eta^{(t'+1)}\frac{1}{(1-\gamma)^2}G(t',t),\label{eq:Is- negative infinity 6}
\end{align}
where \cref{eq:Is- negative infinity 6} is from the update scheme of
APG as in \Cref{algorithm:APG}.
% Note that as $\liminf_{t\rightarrow \infty}\theta_{s,a'}^{(t)}=-\infty$, then $\nu(t)$ must be finite, for all $t$.
Since $\{\nu(t)\}_{t=1}^{\infty}$ is bounded, there is a finite constant $M$ such that
$\sum_{t'\leq\nu(t)}\eta^{(t'+1)}\frac{1}{(1-\gamma)^2}G(t',t) \leq M$
for all $t$.
Therefore, by taking the limit infimum on \cref{eq:Is- negative infinity 6}, we know 
\begin{equation}
    \liminf_{t\rightarrow \infty} Z^{(t)} = -\infty.\label{eq:Is- negative infinity 7}
\end{equation}
Now we are ready to quantify $\theta_{s,a}^{(t)}$ for the action $a\in I_s^-$. 
For all $t'\in\cJ^{(t)}$, we have
\begin{align}
    \frac{\lvert (\partial V^{\pi_{\theta}}(\mu)/\partial \theta_{s,a})|_{\theta=\omega^{(t')}}\rvert}{\lvert (\partial V^{\pi_{\theta}}(\mu)/\partial \theta_{s,a'})|_{\theta=\omega^{(t')}}\rvert}&=\bigg\lvert \frac{\pi_{\omega}^{(t')}(a\rvert s)A^{\pi_{\omega}^{(t')}}(s,a)}{\pi_{\omega}^{(t')}(a'\rvert s)A^{\pi_{\omega}^{(t')}}(s,a')} \bigg\rvert\geq \exp(\vartheta-\theta_{s,a'}^{(t')})\cdot\frac{(1-\gamma)\Delta_s}{4}\geq \exp(\delta)\cdot\frac{(1-\gamma)\Delta_s}{4},\label{eq:Is- negative infinity 8}
\end{align}
where the first inequality follows from the softmax parameterization,
the assumed upper bound of $\theta_{s,a}^{(t)}$, that $\lvert
A^{\pi_{\omega}^{(t')}}(s,a')\rvert \leq 1/(1-\gamma)$, and that $A^{\pi_{\omega}^{(t')}}(s,a) \leq
-\Delta_s/4$, and the second one holds by the definition of $\nu(t)$
in \cref{eq:Is- negative infinity 1}.
For any $\cJ^{(t)}\neq \emptyset$, we have
\begin{align}
	\nonumber
    \theta_{s,a}^{(t)}-\theta^{(1)}_{s,a}&=\sum_{t':1\leq
		t'<\bar{T}_s}\eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}}\cdot
			G(t',t)+\sum_{t': t'\geq\bar{T}_s}\eta^{(t'+1)}\cdot
			\frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}}\cdot
			G(t',t)\\
    &\leq \sum_{t':1\leq t'<\bar{T}_s}\eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',t)+\sum_{t': t'\in \cJ^{(t)}}\eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',t)\label{eq:Is- negative infinity 10}\\
    &\leq \underbrace{\sum_{t':1\leq t'<\bar{T}_s}\eta^{(t'+1)} \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}} G(t',t)}_{<\infty \text{ and does not depend on }t }+\exp(\delta) \frac{(1-\gamma)\Delta_s}{4}\underbrace{\sum_{t': t'\in \cJ^{(t)}}\eta^{(t'+1)} \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}} G(t',t)}_{\equiv Z^{(t)}},\label{eq:Is- negative infinity 11}
\end{align}
where \cref{eq:Is- negative infinity 10} holds by the fact that
$A^{\pi_{\omega}^{(t')}}(s,a)<0$ for all $t\geq \bar{T}_s$, and \cref{eq:Is- negative infinity 11} is a direct result of \cref{eq:Is- negative infinity 8}.
Therefore, by taking the limit infimum on \cref{eq:Is- negative infinity 11}, we have $\liminf_{t\rightarrow \infty}\theta_{s,a}^{(t)} =-\infty$, which leads to a contradiction.

For the case (ii), given that $\nu(t)$ becomes unbounded as $t\rightarrow\infty$, there are infinitely many $\tau \ge \bar{T}_{s}$ such that $\theta_{s,a'}^{(\tau)}\geq \vartheta-\delta$. In addition, recall that $a'$ is an action that satisfies $\liminf_{t\rightarrow \infty}\theta_{s,a'}^{(t)}=-\infty$. Therefore, we can find a subsequence $\{t_i\}_{i=1}^{\infty}$ of time indices satisfying the following properties:
\begin{itemize}
    \item $t_1 \ge \bar{T}_s$
    \item $\lim_{i\rightarrow\infty} \theta_{s, a'}^{(t_i)} = -\infty$.
    \item $\theta_{s, a'}^{(t_i)} < \vartheta - \delta$ for all $i \ge 1$.
    \item There is always a $\tau_{i} \ge \bar{T}_s$ satisfying that
		$\theta_{s,a'}^{(\tau_i)}\geq \vartheta-\delta$, $\tau_i \in
		(t_i, t_{i+1})$, and we specifically let $\tau_i \coloneqq \inf\{\tau \in (t_i, t_{i+1}): \theta_{s,a'}^{(\tau_i)}\geq \vartheta-\delta\}$ for each $i \ge 1$.
\end{itemize}
%    {\color{red}{Despite that $\lim_{i\rightarrow\infty}
%		\theta_{s, a'}^{(t_i)} = -\infty$,
%		we can always find $\tau_i >
%		t_i$ such that $\theta_{s, a'}^{(\tau_i)} > \theta_{s, a'}^{(t_i)}$.
%		Therefore,
%		it follows that the momentum must be canceled by the
%		gradients. Thus, we can always select $t_i$ such that there exists an absolute finite constant $C_m > 0$ where the
%		momentum $\theta^{(t_i)}_{s, a'} - \theta^{(t_i-1)}_{s, a'}$ with respect to the direction $(s, a')$ at time $t_i$ satisfies $-C_m \le \theta^{(t_i)}_{s, a'} - \theta^{(t_i-1)}_{s, a'} \le 0$ for every $i \ge 1$.}}\footnote{\cpcomment{$C_m$
%			and $m_{s,a'}^{(t)}$ are undefined, and thus can't
%			parse/verify the next ineq. Also please remove the eq
%		numbers not referred.} \updatecomment{We directly write the momentum at time $t_i$.}}
{Since $\lim_{i\rightarrow\infty} \theta_{s, a'}^{(t_i)} = -\infty$,
we can select $\{t_i\}$ in a way such that $\theta^{(t_i)}_{s, a'} -
\theta^{(t_i-1)}_{s, a'} < 0$ for all $i$.
Therefore,}
\begin{align}
    \theta^{(\tau_i)}_{s, a'} - \theta^{(t_i)}_{s, a'}
	&= {(\theta^{(t_i)}_{s, a'} - \theta^{(t_i-1)}_{s,
	a'})\cdot (G({t_i-1}, \tau_i) - 1) + \sum_{t_i \le t' <
	\tau_i} \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',\tau_i)} \nonumber \\
    &\le \sum_{t_i \le t' < \tau_i} \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',\tau_i) \nonumber \\
    &\le \sum_{t_i \le t' < \tau_i} \Big\lvert \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a'}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',\tau_i) \Big\rvert \nonumber \\
    % &= \Big\lvert m^{(t_i)}_{s, a'} \Big\lvert + \sum_{t_i \le t' < \tau_i} \Big\lvert \eta^{(t'+1)}\cdot \frac{1}{1-\gamma} \cdot d^{\pi^{(t')}}_{\mu}(s) \cdot \pi_\theta(a'|s) \cdot A^{\pi_\theta}(s,a') \cdot G(t',t_i) \Big\rvert \\
    % &= \Big\lvert m^{(t_i)}_{s, a'} \Big\lvert + \sum_{t_i \le t' < \tau_i} \eta^{(t'+1)}\cdot \frac{1}{1-\gamma} \cdot d^{\pi_\theta}_{\mu}(s) \cdot \pi_\theta(a'|s) \cdot \Big\lvert A^{\pi_\theta}(s,a') \Big\lvert \cdot G(t',t_i) \\
    &\le \frac{4}{(1-\gamma)\Delta_s} \cdot \sum_{t_i \le t' < \tau_i}
	\Big\lvert \eta^{(t'+1)}\cdot \frac{\partial
		V^{\pi_\theta}(\mu)}{\partial \theta_{s,{a}}}\Big\rvert_{\theta=\omega^{(t')}} \cdot G(t',\tau_i)\Big\rvert, \label{eq:Is- negative infinity 12}
\end{align}
where \cref{eq:Is- negative infinity 12} is from that
\begin{equation}
    \frac{\lvert (\partial V^{\pi_{\theta}}(\mu)/\partial \theta_{s,a'})|_{\theta=\omega^{(t')}}\rvert}{\lvert (\partial V^{\pi_{\theta}}(\mu)/\partial \theta_{s,a})|_{\theta=\omega^{(t')}}\rvert}=\bigg\lvert \frac{\pi_{\omega}^{(t')}(a'\rvert s)A^{\pi_{\omega}^{(t')}}(s,a')}{\pi_{\omega}^{(t')}(a\rvert s)A^{\pi_{\omega}^{(t')}}(s,a)} \bigg\rvert \leq \bigg\lvert \frac{A^{\pi_{\omega}^{(t')}}(s,a')}{A^{\pi_{\omega}^{(t')}}(s,a)} \bigg\rvert \leq \frac{4}{(1-\gamma)\Delta_s},
\end{equation}
where the first inequality holds because $\theta^{(t')}_{s, a'} \le
\theta^{(t')}_{s, a}$, implying $\pi_{\omega}^{(t')}(a'\rvert s) \le \pi_{\omega}^{(t')}(a\rvert s)$. Since $\theta^{(\tau_i)}_{s, a'} - \theta^{(t_i)}_{s, a'} \rightarrow \infty$ as $i\rightarrow\infty$, we have
\begin{equation}
\label{eq: grad Is- infinity}
    \lim_{i \rightarrow\infty}\sum_{t_i \le t' < \tau_i} \Big\lvert \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',\tau_i) \Big\rvert = \lim_{i \rightarrow\infty}\Big\lvert\sum_{t_i \le t' < \tau_i} \eta^{(t'+1)}\cdot \frac{\partial V^{\pi_\theta}(\mu)}{\partial \theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}}\cdot G(t',\tau_i) \Big\rvert = \infty,
\end{equation}
where the first equality holds because $a\in I^{-}_s$ together with
$t' \ge \bar{T}_s$ implies that $\frac{\partial
	V^{\pi_\theta}(\mu)}{\partial
		\theta_{s,a}}\big\rvert_{\theta=\omega^{(t')}}< 0$ for all $t'$
	included in the summation. {
		Now consider
		\[
    \theta^{(t)}_{s, a} - \theta^{(\bar T_s)}_{s, a}
	= {(\theta^{(\bar T_s)}_{s, a} - \theta^{(\bar T_s-1)}_{s,
	a})\cdot (G({\bar T_s -1}, t) - 1) + \sum_{t' = \bar T_s
	}^{t-1} \eta^{(t'+1)}\cdot \frac{\partial
		V^{\pi_\theta}(\mu)}{\partial
			\theta_{s,a}}\Big\rvert_{\theta=\omega^{(t')}}\cdot
		G(t',\tau_i)}.
		\]
		By an argument similar to \cref{eq:Is+ bounded eq8},
		%because
		%of the finiteness of $\bar{T}_s$ and $\theta^{(\bar{T}_s)}_{s,
		%a} - \theta^{(\bar{T}_s-1)}_{s, a}$,
		the first term above is at most $(\theta^{(\bar{T}_s)}_{s, a}
		- \theta^{(\bar{T}_s-1)}_{s, a}) \cdot O(\bar{T}_s)$
		regardless of $t$.
Combining this with \cref{eq: grad Is- infinity,eq:neggrad},
we obtain $\liminf_{t \rightarrow\infty} \theta^{(t)}_{s, a} = -\infty$,
which also leads to a contradiction.}
Therefore, \cref{eq:liminf} is proven.
%\cpfn{Not quite seeing what this
%	part is about.
%	$\theta^{(\bar{T}_s)}_{s, a'} - \theta^{(\bar{T}_s-1)}_{s, a'}$ is
%	finite for sure, but when you say the cumulative effect, you are
%	talking about it times $G(\bar{T}_s, t_i)$, right?
%	This term might not be bounded.
%	Also, you don't have any bound for the gradients from $\tau_i$ to
%	$t_{i+1}$, so how did you arrive at your conclusion? \updatecomment{The cumulative effect of the momentum at time $\bar{T}_s$ will be the momentum at that time multiplies by the time $\bar{T}_s$ itself. Moreover, since $a\in I_s^-$, the gradients after time $\bar{T}_s$ is negative, the $\liminf$ has to go to $-\infty$. We have updated the statement.}}

Finally, we show that there exists a time $\bar{T}_s'
\ge \bar{T}_s$ such that $\theta^{(\bar T_s'+1)}_{s, a} -
\theta^{(\bar T_s')}_{s, a}
\le 0$.
If such a $\bar{T}_s'$ does not exist, which means that $\{\theta_{s,
a}^{(t)}\}$ is monotonically increasing, we see a contradiction with
\cref{eq:liminf}.
Since $a\in I^{-}_s$, from \cref{eq:neggrad}, we know that if
$\theta^{(\bar{T}_s'+1)}_{s, a} - \theta^{(\bar{T}_s')}_{s, a} \leq
0$, then $\theta^{(t+1)}_{s, a} - \theta^{(t)}_{s, a} \leq 0$ for all
$t \geq \bar T_s$, meaning that $\theta^{(t)}_{s, a}$ is monotonically
decreasing after $\bar T_s'$.
Therefore, combining this monotinicity after $\bar T_s'$ and
\cref{eq:liminf},
%\ge \bar{T}_s$.\cpfn{I
%	don't see why
%	the finiteness of $\theta^{(\bar{T}_s)}_{s, a'} -
%	\theta^{(\bar{T}_s-1)}_{s, a'}$ (which is trivially true anyway)
%leads to monotinicity. \updatecomment{We have updated the argument.}}}
%Hence, combining the monotonicity with the proven result of
%$\liminf_{t\rightarrow\infty} \theta^{(t)}_{s, a} = -\infty$,
we obtain
$\lim_{t\rightarrow\infty} \theta^{(t)}_{s, a} = -\infty$.
\end{proof}

In the following lemma, we use the notation
{$\Delta\theta_{s,a}^{(t)}\coloneqq\theta_{s,a}^{(t+1)}-\theta_{s,a}^{(t)}$},
for each state-action pair $(s,a)$ and each $t\in \bbN$.


\begin{lemma}
    \label{lemma: ordering unchanged}
    Consider any state $s$ with non-empty $I_s^+$ and some $a_+\in
	I_s^+$ and $a\in I_s^0$.
{Under the setting of \Cref{lemma: convergence to
stationarity},}
	if
	{$\omega_{s,a_+}^{(\tau)}>\omega_{s,a}^{(\tau)}$} and
	$\Delta\theta_{s,a_+}^{(\tau)}>\Delta\theta_{s,a}^{(\tau)}$ for
	some $\tau > \bar{T}_s$, then
	{$\omega_{s,a_+}^{(t)}>\omega_{s,a}^{(t)}$} and
	$\Delta\theta_{s,a_+}^{(t)}>\Delta\theta_{s,a}^{(t)}$ for all $t>
	\tau$.
\end{lemma}

\begin{proof}[Proof of \Cref{lemma: ordering unchanged}]
    We prove this by induction. Suppose at some time $\tau > \bar{T}_s$, we have $\omega_{s,a_+}^{(\tau)}>\omega_{s,a}^{(\tau)}$ and $\Delta\theta_{s,a_+}^{(\tau)}>\Delta\theta_{s,a}^{(\tau)}$.
    Recalling our definition in \cref{eq:adv I_s+} and \cref{eq:adv I_s0}, we have from \Cref{lemma:softmax_pg} that
    \begin{align}
        \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a_{+}}}\right|_{\theta = \omega^{(\tau)}}&=\frac{1}{1-\gamma} \cdot d^{\pi^{(\tau)}_{\omega}}_{\mu}(s) \cdot \pi^{(\tau)}_\omega(a_+\rvert s) \cdot A^{\pi_{\omega}^{(\tau)}}(s,a_+)\nonumber\\
        &>\frac{1}{1-\gamma} \cdot d^{\pi^{(\tau)}_{\omega}}_{\mu}(s) \cdot \pi_\omega^{(\tau)}(a\rvert s) \cdot A^{\pi_{\omega}^{(\tau)}}(s,a)\label{eq: ordering unchanged 3}\\
        &=\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a}}\right|_{\theta = \omega^{(\tau)}},\label{eq: ordering unchanged 4}
    \end{align}
    where \cref{eq: ordering unchanged 3} holds by
	$\omega_{s,a_+}^{(\tau)}>\omega_{s,a}^{(\tau)}$ and the fact that
	$\tau >\bar{T}_s$ implies $A^{\pi_{\omega}^{(\tau)}}(s,a_+)\geq
	A^{\pi_{\omega}^{(\tau)}}(s,a)$ from \cref{eq:adv I_s+}.
	By the update rule \cref{algorithm:eq1}, \cref{eq: ordering
	unchanged 4} and that
	$\omega_{s,a_+}^{(\tau)}>\omega_{s,a}^{(\tau)}$ imply
		\begin{equation}
			\label{eq:thetaorder}
			\theta_{s,a_+}^{(\tau + 1)}>\theta_{s,a}^{(\tau + 1)}.
		\end{equation}
	Thus,
	from $\Delta\theta_{s,a_+}^{(\tau)}>\Delta\theta_{s,a}^{(\tau)}$,
	\cref{algorithm:eq2,algorithm:eq3,eq:thetaorder}, we have
    \begin{align}
        \omega_{s,a_+}^{(\tau+1)}
        &=\theta_{s,a_+}^{(\tau+1)}+\mathbb{I} \left\{V^{\pi_{\varphi}^{(\tau+1)}}(\mu) \ge V^{\pi_{\theta}^{(\tau+1)}}(\mu)\right \} \cdot\frac{\tau}{\tau+3}(\theta_{s,a_+}^{(\tau+1)}-\theta_{s,a_+}^{(\tau)}) \nonumber \\
        &>\theta_{s,a}^{(\tau+1)}+\mathbb{I}
		\left\{V^{\pi_{\varphi}^{(\tau+1)}}(\mu) \ge
		V^{\pi_{\theta}^{(\tau+1)}}(\mu)\right \}
		\cdot\frac{\tau}{\tau+3}(\theta_{s,a}^{(\tau+1)}-\theta_{s,a}^{(\tau)})=\omega_{s,a}^{(\tau+1)}.\label{eq: ordering unchanged 1}
    \end{align}
    By \cref{eq: ordering
	unchanged 1}, \cref{eq:softmax}, and that $A^{\pi_{\omega}^{(\tau+1)}}(s,a_+)\geq A^{\pi_{\omega}^{(\tau+1)}}(s,a)$, we have 
    \begin{equation}
        \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a_{+}}}\right|_{\theta = \omega^{(\tau+1)}} > \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a}}\right|_{\theta = \omega^{(\tau + 1)}}.\label{eq: ordering unchanged tau + 1}
    \end{equation}
    Furthermore, by \cref{eq: ordering unchanged tau + 1} and that
	$\Delta\theta_{s,a_+}^{(\tau)}>\Delta\theta_{s,a}^{(\tau)}$, we have
    \begin{align*}
        \Delta\theta_{s,a_+}^{(\tau+1)}&=\mathbb{I} \left\{V^{\pi_{\varphi}^{(\tau+1)}}(\mu) \ge V^{\pi_{\theta}^{(\tau+1)}}(\mu)\right \} \cdot\frac{\tau}{\tau+3}\Delta\theta_{s,a_+}^{(\tau)}+\eta^{(\tau+2)}\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a_{+}}}\right|_{\theta = \omega^{(\tau+1)}}\\
        &>\mathbb{I} \left\{V^{\pi_{\varphi}^{(\tau+1)}}(\mu) \ge V^{\pi_{\theta}^{(\tau+1)}}(\mu)\right \} \cdot\frac{\tau}{\tau+3}\Delta\theta_{s,a}^{(\tau)}+\eta^{(\tau+2)}\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a}}\right|_{\theta = \omega^{(\tau+1)}}=\Delta\theta_{s,a}^{(\tau+1)}.
    \end{align*}
    By repeating the above argument, we know $\omega_{s,a_+}^{(t)}>\omega_{s,a}^{(t)}$ and $\Delta\theta_{s,a_+}^{(t)}>\Delta\theta_{s,a}^{(t)}$ for all $t>\tau$.
\end{proof}

% \begin{proof}[Proof of \Cref{lemma: ordering unchanged}]
%     {We prove this by induction. Suppose at some time $\tau > \bar{T}_s$, we have $\theta_{s,a_+}^{(\tau)}>\theta_{s,a}^{(\tau)}$ and $\Delta\theta_{s,a_+}^{(\tau)}>\Delta\theta_{s,a}^{(\tau)}$.} Then, we have
%     \begin{align}
%         \omega_{s,a_+}^{(\tau)}
%         &=\theta_{s,a_+}^{(\tau)}+\mathbb{I} \left\{V^{\pi_{\varphi}^{(\tau)}}(\mu) \ge V^{\pi_{\theta}^{(\tau)}}(\mu)\right \} \cdot\frac{\tau-1}{\tau+2}(\theta_{s,a_+}^{(\tau)}-\theta_{s,a_+}^{(\tau-1)}) \nonumber \\
%         &>\theta_{s,a}^{(\tau)}+\mathbb{I}
% 		\left\{V^{\pi_{\varphi}^{(\tau)}}(\mu) \ge
% 		V^{\pi_{\theta}^{(\tau)}}(\mu)\right \}
% 		\cdot\frac{\tau-1}{\tau+2}(\theta_{s,a}^{(\tau)}-\theta_{s,a}^{(\tau-1)})=\omega_{s,a}^{(\tau)}.\label{eq: ordering unchanged 1}
%     \end{align}
% 	Recalling our definition in \cref{eq:def},
% 	we have from \Cref{lemma:softmax_pg} that
%     \begin{align}
%         \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a_{+}}}\right|_{\theta = \omega^{(\tau)}}&=\frac{1}{1-\gamma} \cdot d^{\pi^{(\tau)}_{\omega}}_{\mu}(s) \cdot \pi^{(\tau)}_\omega(a_+\rvert s) \cdot A^{\pi_{\omega}^{(\tau)}}(s,a_+)\nonumber\\
%         &>\frac{1}{1-\gamma} \cdot d^{\pi^{(\tau)}_{\omega}}_{\mu}(s) \cdot \pi_\omega^{(\tau)}(a\rvert s) \cdot A^{\pi_{\omega}^{(\tau)}}(s,a)\label{eq: ordering unchanged 3}\\
%         &=\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a}}\right|_{\theta = \omega^{(\tau)}},\label{eq: ordering unchanged 4}
%     \end{align}
%     where \cref{eq: ordering unchanged 3} holds by \cref{eq: ordering unchanged 1} and the fact that $\tau >\bar{T}_s$ implies $A^{\pi_{\omega}^{(\tau)}}(s,a_+)\geq A^{\pi_{\omega}^{(\tau)}}(s,a)$.
%     Therefore, by \cref{eq: ordering unchanged 1,eq: ordering unchanged 4}, we have
%     \begin{align*}
%         \theta_{s,a_+}^{(\tau+1)}&=\omega_{s,a_+}^{(\tau)}+\eta^{(\tau+1)}\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a_{+}}}\right|_{\theta = \omega^{(\tau)}}>\omega_{s,a}^{(\tau)}+\eta^{(\tau+1)}\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a}}\right|_{\theta = \omega^{(\tau)}}=\theta_{s,a}^{(\tau+1)},\\
%         \Delta\theta_{s,a_+}^{(\tau+1)}&=\mathbb{I} \left\{V^{\pi_{\varphi}^{(\tau)}}(\mu) \ge V^{\pi_{\theta}^{(\tau)}}(\mu)\right \} \cdot\frac{\tau-1}{\tau+2}\Delta\theta_{s,a_+}^{(\tau)}+\eta^{(\tau+1)}\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a_{+}}}\right|_{\theta = \omega^{(\tau)}}\\
%         &>\mathbb{I} \left\{V^{\pi_{\varphi}^{(\tau)}}(\mu) \ge V^{\pi_{\theta}^{(\tau)}}(\mu)\right \} \cdot\frac{\tau-1}{\tau+2}\Delta\theta_{s,a}^{(\tau)}+\eta^{(\tau+1)}\left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial\theta_{s,a}}\right|_{\theta = \omega^{(\tau)}}=\Delta\theta_{s,a}^{(\tau+1)}.
%     \end{align*}
%     By repeating the above argument, we know $\theta_{s,a_+}^{(t)}>\theta_{s,a}^{(t)}$ and $\Delta\theta_{s,a_+}^{(t)}>\Delta\theta_{s,a}^{(t)}$ for all $t>\tau$.
% \end{proof}

Next, we take a closer look at the actions in $I_s^0$. We further
decompose $I_s^0$ into two subsets as follows: Consider any state $s$ with
a non-empty $I_s^+$, for any $a_+\in I_s^+$, we define
\begin{align*}
    B_s^0(a_+)&:=\Big\{a\in I_s^0: \text{For any } t\geq \bar{T}_s, \text{either } {\omega^{(t)}_{s,a}\geq \omega^{(t)}_{s,a_+}} \text{or } \Delta\theta^{(t)}_{s,a}\geq \Delta\theta^{(t)}_{s,a_+}\Big\}
\end{align*}
and use $\bar{B}_s^0(a_+)$ to denote its complement in $I_s^0$. We could thus also write $\bar{B}_s^0(a_+)$ as
\begin{equation*}
    \bar{B}_s^0(a_+):=\Big\{a\in I_s^0: {\omega^{(t)}_{s,a}< \omega^{(t)}_{s,a_+}} \text{and } \Delta\theta^{(t)}_{s,a}<\Delta\theta^{(t)}_{s,a_+} \text{for some } t\geq \bar{T}_s \Big\}.
\end{equation*}

\begin{lemma}
    \label{lemma:sum of Bs0 goes to 1}
	Consider any state $s$.
{Under the setting of \Cref{lemma: convergence to
stationarity},}
    if $I_s^+$ is nonempty, then:
    
    \textbf{(a)} For all $a_+\in I_s^+$, we have
    \begin{equation*}
	\lim_{t\rightarrow \infty}\,
	\sum_{a\in B_s^{0}(a_+)}\pi_\omega^{(t)}(a\rvert s) = 1.
    \end{equation*}

    \textbf{(b)} For all $a_+\in I_s^+$, we have
    \begin{equation*}
	\lim_{t\rightarrow \infty}\,
	\max_{a\in B_s^{0}(a_+)}\omega_{s,a}^{(t)} = \infty.
    \end{equation*}

    \textbf{(c)} For all $a_+\in I_s^+$, we have
    \begin{equation*}
	\lim_{t\rightarrow \infty}\,
        \sum_{a\in B_s^{0}(a_+)}\omega_{s,a}^{(t)} = \infty.
    \end{equation*}    
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:sum of Bs0 goes to 1}]
Regarding \textbf{(a)}, by the definition of $\bar{B}_{s}^{0}(a_+)$, for each $a\in \bar{B}_{s}^{0}(a_+)$, there must exist some $T'\geq \bar{T}_s$ such that {$\omega_{s,a_+}^{(T')}>\omega_{s,a}^{(T')}$} and $\Delta\theta_{s,a_+}^{(T')}>\Delta\theta_{s,a}^{(T')}$.
Then, by \Cref{lemma: ordering unchanged}, we know 
\begin{equation}
    {\omega_{s,a_+}^{(t)}>\omega_{s,a}^{(t)}} \quad \text{ and }\quad \Delta\theta_{s,a_+}^{(t)}>\Delta\theta_{s,a}^{(t)},\quad \text{for all }t\geq T'.\label{eq:sum of Bs0 goes to 1 eq4}
\end{equation}
Moreover, by \Cref{lemma:sum of Is+ and Is- goes to zero} and that
$a_+\in I_s^+$, we have {$\pi_{\omega}^{(t)}(a_+\rvert s)\rightarrow 0$} as
$t\rightarrow \infty$. Based on \cref{eq:sum of Bs0 goes to 1 eq4},
this further implies that {$\pi_{\omega}^{(t)}(a\rvert s)\rightarrow 0$} as
$t\rightarrow \infty$, for all $a\in \bar{B}_{s}^{0}(a_+)$.
Hence, together with \cref{lemma:sum of Is+ and Is- goes to zero} we
obtain the desired result.

Regarding \textbf{(b)}, by the result in \textbf{(a)} and
the argument in the proof of \Cref{lemma:max Is0}, we directly see
that the statement holds true.


Regarding \textbf{(c)}, let us consider any action $a\in {B}_{s}^{0}(a_+)$.
By the definition of $B_s^{0}(a_+)$, at each iteration $t\geq \bar{T}_s$, either {$\omega^{(t)}_{s,a}\geq \omega^{(t)}_{s,a_+}$} or $\Delta\theta^{(t)}_{s,a}\geq \Delta\theta^{(t)}_{s,a_+}$ holds.
Given the result in \textbf{(b)}, it suffices to show that $\{\omega_{s,a}^{(t)}\}_{t=1}^{\infty}$ is bounded from below for all $a \in {B}_{s}^{0}(a_+)$. We prove it by contradiction.
Suppose that there exists an action
$\bar{a} \in {B}_{s}^{0}(a_+)$ such that $\liminf_{t\rightarrow\infty}
\omega^{(t)}_{s, \bar{a}} = -\infty$.
By \Cref{lemma:Is+ bounded}, we know that
$\{\omega_{s,a_+}^{(t)}\}_{t=1}^{\infty}$ is bounded from below.
Therefore, once $\omega^{(t)}_{s,\bar{a}}< \omega^{(t)}_{s,a_+}$ for
some $t$, we will have $\Delta\theta^{(t)}_{s,\bar{a}}\geq
\Delta\theta^{(t)}_{s,a_+}$.
\mru{Following an argument similar to that in
the
proof of \Cref{lemma:Is- negative infinity} (for case (ii)) to choose a subsequence of
$\omega^{(t)}_{s,\bar{a}}$ converging to negative infinity and
combining it with $\Delta\theta^{(t)}_{s,\bar{a}}\geq \Delta\theta^{(t)}_{s,a_+}$, we know that $\liminf_{t\rightarrow\infty}
\omega^{(t)}_{s, a_+} = -\infty$.}\cpfn{I don't see how you can
	directly apply the argument there to here.
	I am not quite seeing how $\Delta\theta^{(t)}_{s,\bar{a}}\geq
	\Delta\theta^{(t)}_{s,a_+}$ leads to the conclusion of $-\infty$.
Please elaborate on that.}
This leads to the desired contradiction and concludes our proof.
\end{proof}

\begin{lemma}
\label{lemma:B_s0 bar}
	Consider any state $s$.
{Under the setting of \Cref{lemma: convergence to
stationarity},}
    for any $a_+\in I_s^+$, the following hold.
    
    \textbf{(a)} There exists $T_{a_+}$ such that for all $a\in \bar{B}_s^{0}(a_+)$,
    \begin{equation*}
    {\pi_{\omega}^{(t)}(a_+\rvert s )>\pi_{\omega}^{(t)}(a\rvert s ),\quad \text{for all } t>T_{a_+}.}
    \end{equation*}
    \textbf{(b)} There exists $T_{a_+}^{\dagger}$ such that for all $a\in \bar{B}_s^{0}(a_+)$, 
    \begin{equation}
        {\lvert A^{\pi_\omega^{(t)}}(s,a)\rvert < \frac{\pi_{\omega}^{(t)}(a_+\rvert s)}{\pi_{\omega}^{(t)}(a\rvert s)} \cdot \frac{\Delta_s}{16 \lvert \cA\rvert}, \quad \text{for all } t>T_{a_+}^\dagger.}\label{eq:B_s0 bar eq2}
    \end{equation}
    This also implies that 
    \begin{equation}
        {\sum_{a\in \bar{B}_s^{0}(a_+)}\pi_{\omega}^{(t)}(a\rvert s) A^{\pi_\omega^{(t)}}(s,a) > -{\pi_{\omega}^{(t)}(a_+\rvert s)}\cdot \frac{\Delta_s}{16 }, \quad \text{for all } t>T_{a_+}^\dagger.}\label{eq:B_s0 bar eq3}
    \end{equation}
\end{lemma}
%\cpcomment{It looks like what you are really using in other proofs is
%	\cref{eq:B_s0 bar eq3}, and all other parts are only things to
%	lead to this conclusion, so they are kind of lemmas of this lemma.
%	I'd suggest to put these two statements in the proof, as some
%parts of claims.}
\begin{proof}[Proof of \Cref{lemma:B_s0 bar}]
    Regarding \textbf{(a)}, for each $a\in \bar{B}_s^{0}(a_+)$, we define 
    \begin{equation*}
        u_a(a_+):=\inf\{\tau\geq \bar{T}_s: {\omega_{s,a_+}^{(\tau)}>\omega_{s,a}^{(\tau)}} \text{ and } \Delta\theta_{s,a_+}^{(\tau)}>\Delta\theta_{s,a}^{(\tau)}\}.
    \end{equation*}
    By the definition of $\bar{B}_s^{0}(a_+)$, we know the following
	two facts: (i) $u_a(a_+)$ is finite for all $a\in
	\bar{B}_s^{0}(a_+)$. (ii) By \Cref{lemma: ordering unchanged}, for all $t \geq u_a(a_+)$, we have {$\omega_{s,a_+}^{(t)}>\omega_{s,a}^{(t)}$} and $\Delta\theta_{s,a_+}^{(t)}>\Delta\theta_{s,a}^{(t)}$.
    Therefore, by choosing $T_{a_+}:=\max_{a\in \bar{B}_s^{0}(a_+)} u_a(a_+)$, we must have {$\pi_{\omega}^{(t)}(a_+\rvert s )>\pi_{\omega}^{(t)}(a\rvert s )$} for all $t>T_{a_+}$.

	Regarding \textbf{(b)}, we have from \textbf{(a)} 
	\begin{equation*}
		\frac{\pi_{\omega}^{(t)}(a_+\rvert
	s)}{\pi_{\omega}^{(t)}(a\rvert s)}>1, \quad \forall t> T_{a_+}.
\end{equation*}
 Thus, we know that for each $a\in \bar{B}_s^{0}(a_+)\subseteq I_s^0$, there exists some finite $t'_{a}>T_{a_+}$ such that 
     \begin{equation*}
         {\lvert A^{\pi_\omega^{(t)}}(s,a)\rvert < \frac{\pi_\omega^{(t)}(a_+\rvert s)}{\pi_\omega^{(t)}(a\rvert s)} \cdot \frac{\Delta_s}{16 \lvert \cA\rvert}, \quad \text{for all } t\geq t'_a.}
     \end{equation*}
     As a result, by choosing $T_{a_+}^{\dagger}:=\max_{a\in\bar{B}_{s}^{0}(a_+)}t'_a$, we conclude that \cref{eq:B_s0 bar eq2}-\cref{eq:B_s0 bar eq3} indeed hold. 
\end{proof}

\begin{lemma}
    \label{lemma:compare pi(a+) and pi(a-)}
{Under the setting of \Cref{lemma: convergence to
stationarity},}
    if $I_s^{+}$ is non-empty, then for any $a_+\in I_s^+$, there exists some finite $\tilde{T}_{a_+}$ such that
    \begin{equation}
        {\sum_{a\in I_s^-}\pi_{\omega}^{(t)}(a\rvert
		s)A^{\pi_\omega^{(t)}}(s,a)> -\pi_{\omega}^{(t)}(a_+\rvert
		s)\frac{\Delta_s}{16}, \quad \forall t\geq \tilde{T}_{a_+}.}\label{eq:compare pi(a+) and pi(a-) eq1}
    \end{equation}
\end{lemma}
\begin{proof}
    {Consider any $a_-\in I_s^-$. By \Cref{lemma:Is+
	bounded,lemma:Is- negative infinity}, we know
	$\{\omega_{s,a_+}^{(t)}\}$ is bounded from below and $\omega_{s,a_-}^{(t)}\rightarrow -\infty$ as $t\rightarrow\infty$.
    This implies that $\pi_{\omega}^{(t)}(a_-\rvert s)/\pi_{\omega}^{(t)}(a_+\rvert
	s)\rightarrow 0$ as $t \rightarrow \infty$.
    Therefore, there exists some finite $t'_{a_-} \ge \bar{T}_s$ such that
    \begin{equation}
        \frac{\pi_{\omega}^{(t)}(a_-\rvert
	s)}{\pi_{\omega}^{(t)}(a_+\rvert s)} < \frac{\Delta_s
	(1-\gamma)}{16\lvert \cA\rvert }, \quad \forall t \geq t'_{a_-}.
	\label{eq:piratio}
    \end{equation}
    By the definition of $\bar{T}_s$ in \cref{eq:adv I_s-} and
	\Cref{lemma: reward range to value range}, we know that
	\begin{equation}
		-\frac{1}{1-\gamma} \le A^{\pi_\omega^{(t)}}(s, a_{-}) < 0,\quad
		\forall t \geq t'_{a_-}.
		\label{eq:Abound}
	\end{equation}
	Combining \cref{eq:piratio,eq:Abound} leads to
    \begin{equation}
        \pi_{\omega}^{(t)}(a_-\rvert s) A^{\pi_\omega^{(t)}}(s, a_{-}) > -\pi_{\omega}^{(t)}(a_+\rvert s)\frac{\Delta_s}{16\lvert\mathcal{A}\rvert}.
		\label{eq:singleitem}
    \end{equation}
    By choosing $\tilde{T}_{a_+}:=\max_{a_-\in I_s^-}t'_{a_-}$ and
	summing \cref{eq:singleitem} over $a_i \in I_s^-$, we obtain
	\cref{eq:compare pi(a+) and pi(a-) eq1}.}
\end{proof}
%\cpcomment{I believe the statement is correct, but this proof
%	seems to be irrelevant to the claim?}
%\updatecomment{We have updated the correct proof.}
%%%%%%%%%%
\newpage
\subsection{Putting Everything Together: Asymptotic Convergence of APG}
\label{app:asym_conv:all}
Now we are ready to put everything together and prove \Cref{theorem:convergeoptimal},
which we restate below.%\cpfn{In the theorem statement there should be
%	some descriptions about the setting of $m_{init}$. \updatecomment{We remove $m_{\text{init}}$ and update the related statements and proofs.}}

%\cpcomment{Here and in several places in the main text, you mentioned
%	``tabular'' softmax parameterization, but the term ``tabular'' is
%not defined or explained anywhere.}
%\updatecomment{We add the explanation of the term ``tabular'' in \Cref{sec:prelim} when introducing softmax parameterization.}
\convergeoptimalthm*

\begin{proof}[Proof of \Cref{theorem:convergeoptimal}]

By \Cref{lemma:perf_diff}, it suffices to prove that $I_s^+ = \emptyset$ for all $s \in \cS$.
%\cpfn{Why is it related to \Cref{lemma:sum of Is+ and Is- goes to zero}? \updatecomment{You are right, it is not related to Lemma \Cref{lemma:sum of Is+ and Is- goes to zero}.}}
We prove this by contradiction.
Suppose there exists at least one
state $s\in \cS$ with a non-empty $I_s^+$.
%\footnote{\cpcomment{Need to
%	include explanation that this leads to the desired result. It is
%	also fine if you just cite the paper mentioned and say following
%their argument or so, but you need that sentence to make the proof
%rigorous.} \updatecomment{If $I_s^{+}$ is not empty, then by performance difference lemma, the limiting value function will be greater than other value function induced by any policy.}}
Consider an action $a_+\in I_s^+$. 
Recall the definitions of $\bar{T}_s$, $T_{a_+},T_{a_+}^\dagger$, and
$\tilde{T}_{a_+}$ from \cref{eq:adv I_s+}-\cref{eq:adv I_s0},
\Cref{lemma:B_s0 bar}, and \Cref{lemma:compare pi(a+) and pi(a-)}.
We define $T_{\max}:=\max\{\bar{T}_s,T_{a_+},T_{a_+}^{\dagger}, \tilde{T}_{a_+}\}$,
then we have for all {$t>T_{\max}$},
\begin{align}
    0&= \sum_{a\in B_s^0(a_+)} \pi_{\omega}^{(t)}(a\rvert
	s)A^{\pi_{\omega}^{(t)}}(s,a)+\underbrace{\sum_{a\in \bar{B}_s^0(a_+)}
	\pi_{\omega}^{(t)}(a\rvert s)A^{\pi_{\omega}^{(t)}}(s,a)}_{>-\pi_{\omega}^{(t)}(a_+\rvert
	s)\frac{\Delta_s}{16} \text{ by \Cref{lemma:B_s0 bar}}} \nonumber \\
    &\quad +\underbrace{\sum_{a\in I_s^+} \pi_{\omega}^{(t)}(a\rvert
	s)A^{\pi_{\omega}^{(t)}}(s,a)}_{\geq \pi_{\omega}^{(t)}(a_+\rvert
	s)\frac{\Delta_s}{4}}+\underbrace{\sum_{a\in I_s^-}
	\pi_{\omega}^{(t)}(a\rvert s)A^{\pi_{\omega}^{(t)}}(s,a)}_{>-\pi_{\omega}^{(t)}(a_+\rvert
	s)\frac{\Delta_s}{16} \text{by \Cref{lemma:compare pi(a+) and pi(a-)}} }\label{eq:convergeoptimal 1}\\
    &>\sum_{a\in B_s^0(a_+)} \pi_{\omega}^{(t)}(a\rvert s)A^{\pi_{\omega}^{(t)}}(s,a)+\frac{1}{8}\cdot\pi_{\omega}^{(t)}(a_+\rvert s)\Delta_s\nonumber \\
    &>\sum_{a\in B_s^0(a_+)} \pi_{\omega}^{(t)}(a\rvert s)A^{\pi_{\omega}^{(t)}}(s,a),\label{eq:convergeoptimal 3}
\end{align}
where \cref{eq:convergeoptimal 1} uses \Cref{lemma:sum_pi_A}.
By \Cref{lemma:softmax_pg}, \cref{eq:convergeoptimal 3} further implies
\begin{equation}
	\label{eq:negative}
	\sum_{a\in B_s^0(a_+)} \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial
		\theta_{s,a}}\right|_{{\theta = \omega^{(t)}}}<0, \quad \forall t> T_{\max}.
\end{equation}
Moreover, {for any $t>T_{\max} + 4$}, we have
\begin{align}
    &~\sum_{a\in
	B_s^0(a_+)}\theta_{s,a}^{(t)}-\theta_{s,a}^{(0)}\nonumber\\
	=&~\sum_{a\in B_s^0(a_+)}\sum_{t'=0}^{t-1}\Big(
	\eta^{(t'+1)}\cdot \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial
		\theta_{s,a}}\right|_{{\theta = \omega^{(t')}}}\cdot G(t',t)\Big)\label{eq:update expansion}\\
		=&~\sum_{t'=0}^{t-1} \eta^{(t'+1)}G(t',t)\cdot
		\Big(\sum_{a\in B_s^0(a_+)} \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial
		\theta_{s,a}}\right|_{{\theta = \omega^{(t')}}}\Big)\nonumber\\
    =&~\underbrace{\sum_{t'=0}^{T_{\max}} \eta^{(t'+1)}G(t',t)\cdot
	\Big(\sum_{a\in B_s^0(a_+)} \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial
		\theta_{s,a}}\right|_{{\theta = \omega^{(t')}}}\Big)}_{\text{Independent of $t$ and thus finite}}
	+ \sum_{t'=T_{\max}+1}^{t-1} \eta^{(t'+1)}G(t',t)\cdot \underbrace{\Big(\sum_{a\in B_s^0(a_+)} \left.\frac{\partial V^{\pi_{\theta}}(\mu)}{\partial
		\theta_{s,a}}\right|_{{\theta = \omega^{(t')}}}\Big)}_{<0 \text{ by \cref{eq:negative}}}\label{eq:convergeoptimal 7-2},
\end{align}
where \cref{eq:update expansion} holds due to \Cref{lemma:theta as sum of gradients} and $t > T_{\text{max}} + 4 > 4$. By taking the limit of $t$ to infinity at both sides of \cref{eq:convergeoptimal 7-2}, the left-hand side
goes to
positive infinity by \Cref{lemma:sum of Bs0 goes to 1} but the
right-hand side is bounded from above. This leads to a contradiction and hence completes the proof.
\end{proof}

\begin{corollary}
\label{cor:policy convergence}
Consider a tabular softmax parameterized policy and assume that
\Cref{assump:unique_optimal} holds.
Under the setting of \Cref{theorem:convergeoptimal},
%Under \hyperref[algorithm:APG]{APG} with $\eta^{(t)} = \frac{t}{t+1} \cdot \frac{(1-\gamma)^3}{16}$ {and $\mu$ initialized uniformly at random},
the following holds almost surely:
\begin{equation*}
   \lim_{t\rightarrow \infty}V^{\pi_{\omega}^{(t)}}(s) = V^{*}(s),\quad
    \lim_{t\rightarrow \infty} \pi_{\theta}(a^*(s) | s) = 1, \quad
	\lim_{t\rightarrow \infty} \pi_{\omega}(a^*(s) | s) = 1, \quad \forall s\in\cS.
\end{equation*}
\end{corollary}
\begin{proof}[Proof of \Cref{cor:policy convergence}]
By \Cref{lemma: monotone limits exist} and
\Cref{theorem:convergeoptimal}, we know that almost surely
\begin{equation}
	\lim_{t\rightarrow \infty}V^{\pi_{\omega}^{(t)}}(s) =
	\lim_{t\rightarrow \infty}V^{\pi_{\theta}^{(t)}}(s) =
	V^*(s),\quad \forall s\in\cS.
	\label{eq:sameV}
\end{equation}
From \Cref{assump:unique_optimal} and page 14 of \citep{szepesvari2022algorithms},
\cref{eq:sameV} then implies that the
policy weight of the optimal action $a^*(s)$ converges to $1$, proving
the desired results.
%\cpcomment{Need more explanations.
%	Currently you only have that the optimal policy $a^*(s)$ gives the largest
%	$Q^*(s,a)$, but how is that related to $V^*(s)$ or $A^*(s,a)$ is
%not explained.} \updatecomment{We refer to the textbook \citep{szepesvari2022algorithms}.}
\end{proof}




